Manipulating organic semiconductor morphology with visible light

We present a method to manipulate the final morphology of roll-to-roll slot-die coated poly(3-hexylthiophene) (P3HT) by optically exciting the p-type polymer in solution while coating. Our results provide a comprehensive picture of the entire knowledge chain, from demonstrating how to apply our method to a fundamental understanding of the changes in morphology and physical properties induced by exciting P3HT while coating. By combining results from density functional theory and molecular dynamics simulations with a variety of X-ray experiments, absorption spectroscopy, and THz spectroscopy, we demonstrate the relationship between morphology and physical properties of the thin film. Specifically, in P3HT films excited with light during deposition, we observe changes in crystallinity and texture with more face-on orientation and increased out-of-plane charge mobility.

==> myArticles.tex <==
@article{Liu2018,
    title = {{18{\%} Efficiency organic solar cells}},
    year = {2020},
    journal = {Science Bulletin},
    author = {Liu, Qishi and Jiang, Yufan and Jin, Ke and Qin, Jianqiang and Xu, Jingui and Li, Wenting and Xiong, Ji and Liu, Jinfeng and Xiao, Zuo and Sun, Kuan and Yang, Shangfeng and Zhang, Xiaotao and Ding, Liming},
    number = {4},
    month = {2},
    pages = {272--275},
    volume = {65},
    publisher = {Elsevier B.V.},
    doi = {10.1016/j.scib.2020.01.001},
    issn = {20959281}
}

@article{DPDAK,
    title = {{A customizable software for fast reduction and analysis of large X-ray scattering data sets: applications of the new DPDAK package to small-angle X-ray scattering and grazing-incidence small-angle X-ray scattering}},
    year = {2014},
    journal = {J. Appl. Cryst},
    author = {Benecke, Gunthard and Wagermaier, Wolfgang and Li, Chenghao and Schwartzkopf, Matthias and Flucke, Gero and Hoerth, Rebecca and Zizak, Ivo and Burghammer, Manfred and Metwalli, Ezzeldin and M{\"{u}}ller-Buschbaum, Peter and Trebbin, Martin and Forster, Stephan and Paris, Oskar and Roth, Stephan V. and Fratzl, Peter},
    number = {5},
    pages = {1797--1803},
    volume = {47},
    publisher = {International Union of Crystallography},
    url = {http://www.dawnsci.org/},
    doi = {10.1107/S1600576714019773},
    issn = {1600-5767},
    keywords = {computer programs, data analysis, data reduction, grazing-incidence small-angle X-ray scattering, small-angle X-ray scattering}
}

@article{Armin2021,
    title = {{A History and Perspective of Non-Fullerene Electron Acceptors for Organic Solar Cells}},
    year = {2021},
    journal = {Advanced Energy Materials},
    author = {Armin, Ardalan and Li, Wei and Sandberg, Oskar J. and Xiao, Zuo and Ding, Liming and Nelson, Jenny and Neher, Dieter and Vandewal, Koen and Shoaee, Safa and Wang, Tao and Ade, Harald and Heum{\"{u}}ller, Thomas and Brabec, Christoph and Meredith, Paul},
    number = {15},
    month = {4},
    pages = {2003570},
    volume = {11},
    publisher = {John Wiley {\&} Sons, Ltd},
    url = {https://onlinelibrary.wiley.com/doi/full/10.1002/aenm.202003570 https://onlinelibrary.wiley.com/doi/abs/10.1002/aenm.202003570 https://onlinelibrary.wiley.com/doi/10.1002/aenm.202003570},
    doi = {10.1002/AENM.202003570},
    issn = {1614-6840},
    keywords = {fullerene electron acceptors, non, organic solar cells, review and perspective}
}

@article{Grimme2013,
    title = {{A simplified Tamm-Dancoff density functional approach for the electronic excitation spectra of very large molecules}},
    year = {2013},
    journal = {The Journal of Chemical Physics},
    author = {Grimme, Stefan},
    number = {24},
    month = {6},
    pages = {244104},
    volume = {138},
    publisher = {American Institute of PhysicsAIP},
    url = {https://aip.scitation.org/doi/abs/10.1063/1.4811331},
    doi = {10.1063/1.4811331},
    issn = {0021-9606},
    keywords = {approximation theory, circular dichroism, density functional theory, dyes, excited states, polymers, ultraviolet spectra}
}

@misc{r_ruger_ams_2020,
    title = {{AMS DFTB 2021.1, SCM, Theoretical Chemistry Vrije Universiteit Amsterdam The Netherlands http://www.scm.com}},
    year = {2021}
}

@article{Pedersen1997,
    title = {{Analysis of small-angle scattering data from colloids and polymer solutions: Modeling and least-squares fitting}},
    year = {1997},
    journal = {Advances in Colloid and Interface Science},
    author = {Pedersen, Jan Skov},
    number = {1-3},
    month = {7},
    pages = {171--210},
    volume = {70},
    publisher = {Elsevier},
    doi = {10.1016/S0001-8686(97)00312-6},
    issn = {00018686}
}

@article{P3HTnfa2019,
    title = {{Blade coated P3HT:non-fullerene acceptor solar cells: a high-throughput parameter study with a focus on up-scalability}},
    year = {2019},
    journal = {Journal of Materials Chemistry A},
    author = {Pascual-San-Jos{\'{e}}, Enrique and Rodr{\'{i}}guez-Mart{\'{i}}nez, Xabier and Adel-Abdelaleim, Rana and Stella, Marco and Mart{\'{i}}nez-Ferrero, Eugenia and Campoy-Quiles, Mariano},
    number = {35},
    pages = {20369--20382},
    volume = {7},
    publisher = {Royal Society of Chemistry (RSC)},
    doi = {10.1039/c9ta07361b},
    issn = {2050-7488}
}

@article{Riccardo2017,
    title = {{Bulk Heterojunction Morphologies with Atomistic Resolution from Coarse-Grain Solvent Evaporation Simulations}},
    year = {2017},
    journal = {Journal of the American Chemical Society},
    author = {Alessandri, Riccardo and Uusitalo, Jaakko J. and De Vries, Alex H. and Havenith, Remco W.A. and Marrink, Siewert J.},
    number = {10},
    month = {3},
    pages = {3697--3705},
    volume = {139},
    publisher = {American Chemical Society},
    url = {https://pubs.acs.org/doi/full/10.1021/jacs.6b11717},
    doi = {10.1021/jacs.6b11717},
    issn = {15205126},
    pmid = {28209056}
}

@article{Cunningham2008,
    title = {{Carrier dynamics resulting from above and below gap excitation of P3HT and P3HT/ PCBM investigated by optical-pump terahertz-probe spectroscopy}},
    year = {2008},
    journal = {Journal of Physical Chemistry C},
    author = {Cunningham, Paul D and Michael Hayden, L.},
    number = {21},
    pages = {7928--7935},
    volume = {112},
    doi = {10.1021/jp711827g},
    issn = {19327447}
}

@article{Velde2001,
    title = {{Chemistry with ADF}},
    year = {2001},
    journal = {Journal of Computational Chemistry},
    author = {te Velde, G. and Bickelhaupt, F. M. and Baerends, E. J. and Fonseca Guerra, C. and van Gisbergen, S. J.A. and Snijders, J. G. and Ziegler, T.},
    number = {9},
    month = {7},
    pages = {931--967},
    volume = {22},
    doi = {10.1002/JCC.1056/FORMAT/PDF},
    issn = {01928651},
    keywords = {ADF program, Chemical bond, Density functional theory, Materials science, Reactivity}
}

@article{singH2017,
    title = {{Comparative analysis of contact resistance and photoresponse in poly(3-hexylthiophene) and poly(3-octylthiophene) based organic field-effect transistors}},
    year = {2017},
    journal = {Synthetic Metals},
    author = {Bhargava, Kshitij and Shukla, Mayoorika and Singh, Vipul},
    month = {11},
    pages = {15--21},
    volume = {233},
    publisher = {Elsevier},
    doi = {10.1016/j.synthmet.2017.08.013},
    issn = {03796779},
    keywords = {Alkyl chain, Contact resistance, OFETs, P3ATs, Photoresponse}
}

@article{RRp3ht,
    title = {{Connecting Molecular Conformation to Aggregation in P3HT Using Near Edge X-ray Absorption Fine Structure Spectroscopy}},
    year = {2017},
    journal = {J. Phys. Chem. C},
    author = {Urquhart, Stephen G and Martinson, Mercedes and Eger, Shaylin and Murcia, Victor and Ade, Harald and Collins, Brian A},
    pages = {121},
    url = {https://pubs.acs.org/sharingguidelines},
    doi = {10.1021/acs.jpcc.7b07143}
}

@article{Tobias2017,
    title = {{Controlled Molecular Orientation of Inkjet Printed Semiconducting Polymer Fibers by Crystallization Templating}},
    year = {2017},
    journal = {Chem. Mater.},
    author = {Ro, Tobias and Marszalek, Tomasz and Held, Martin and Beck, Sebastian and Mu, Christian and Eckstein, Ralph and Morfa, Anthony J and Lovrincic, Robert and Pucci, Annemarie and Lemmer, Uli and Zaumseil, Jana and Pisula, Wojciech and Hernandez-Sosa, Gerardo},
    url = {https://pubs.acs.org/sharingguidelines},
    doi = {10.1021/acs.chemmater.7b03948}
}

@article{tobias2017b,
    title = {{Controlled Molecular Orientation of Inkjet Printed Semiconducting Polymer Fibers by Crystallization Templating}},
    year = {2017},
    journal = {Chemistry of Materials},
    author = {R{\"{o}}dlmeier, Tobias and Marszalek, Tomasz and Held, Martin and Beck, Sebastian and M{\"{u}}ller, Christian and Eckstein, Ralph and Morfa, Anthony J. and Lovrincic, Robert and Pucci, Annemarie and Lemmer, Uli and Zaumseil, Jana and Pisula, Wojciech and Hernandez-Sosa, Gerardo},
    number = {23},
    month = {12},
    pages = {10150--10158},
    volume = {29},
    publisher = {American Chemical Society},
    url = {https://pubs.acs.org/doi/full/10.1021/acs.chemmater.7b03948},
    doi = {10.1021/ACS.CHEMMATER.7B03948/SUPPL{\_}FILE/CM7B03948{\_}SI{\_}002.AVI},
    issn = {15205002}
}

@article{JClark2009,
    title = {{Determining exciton bandwidth and film microstructure in polythiophene films using linear absorption spectroscopy}},
    year = {2009},
    journal = {Applied Physics Letters},
    author = {Clark, Jenny and Chang, Jui Fen and Spano, Frank C and Friend, Richard H and Silva, Carlos},
    number = {16},
    volume = {94},
    doi = {10.1063/1.3110904},
    issn = {00036951},
    arxivId = {0903.1670}
}

@article{kunlun2017,
    title = {{Deuteration as a Means to Tune Crystallinity of Conducting Polymers}},
    year = {2017},
    journal = {The Journal of Physical Chemistry Letters},
    author = {Jakowski, Jacek and Huang, Jingsong and Garashchuk, Sophya and Luo, Yingdong and Hong, Kunlun and Keum, Jong and Sumpter, Bobby G.},
    number = {18},
    month = {9},
    pages = {4333--4340},
    volume = {8},
    url = {https://pubs.acs.org/doi/10.1021/acs.jpclett.7b01803},
    doi = {10.1021/acs.jpclett.7b01803},
    issn = {1948-7185}
}

@article{Cooke2012,
    title = {{Direct observation of sub-100 fs mobile charge generation in a polymer-fullerene film}},
    year = {2012},
    journal = {Physical Review Letters},
    author = {Cooke, D. G. and Krebs, F. C. and Jepsen, P. U.},
    number = {5},
    month = {1},
    pages = {056603},
    volume = {108},
    publisher = {American Physical Society},
    url = {https://link.aps.org/doi/10.1103/PhysRevLett.108.056603},
    doi = {10.1103/PhysRevLett.108.056603},
    issn = {00319007}
}

@article{Fogh2019,
    title = {{Dzyaloshinskii-Moriya interaction and the magnetic ground state in magnetoelectric LiCoPO 4}},
    year = {2019},
    journal = {Physical Review B},
    author = {Fogh, Ellen and Zaharko, Oksana and Schefer, Jürg and Niedermayer, Christof and Holm-Dahlin, Sonja and S{\o}rensen, Michael Korning and Kristensen, Andreas Bott and Andersen, Niels Hessel and Vaknin, David and Christensen, Niels Bech and Toft-Petersen, Rasmus and Fogh, Ellen; Zaharko, Oksana; Schefer, Jurg; Niedermayer, Christof; Holm-Dahlin, Sonja; S{\o}rensen, Michael Korning; Kristensen, Andreas Bott; Andersen, Niels Hessel; Vaknin, David; Christensen, Niels Bech},
    number = {10},
    pages = {104421},
    volume = {99},
    url = {https://doi.org/10.1103/PhysRevB.99.104421},
    doi = {10.1103/PhysRevB.99.104421},
    keywords = {doi:10.1103/PhysRevB.99.104421 url:https://doi.org}
}

@article{roth2019,
    title = {{Effect of Solvent Additives on the Morphology and Device Performance of Printed Nonfullerene Acceptor Based Organic Solar Cells}},
    year = {2019},
    journal = {ACS Applied Materials and Interfaces},
    author = {Wienhold, Kerstin S and K{\"{o}}rstgens, Volker and Grott, Sebastian and Jiang, Xinyu and Schwartzkopf, Matthias and Roth, Stephan V and M{\"{u}}ller-Buschbaum, Peter},
    pages = {42313--42321},
    volume = {11(45)},
    url = {www.acsami.org},
    doi = {10.1021/acsami.9b16784},
    issn = {19448252},
    pmid = {31644257},
    keywords = {high-efficiency organic solar cells, printed organic solar cells, slot-die coating, small molecule acceptor, solvent additives}
}

@article{p3ht_temp,
    title = {{Effect of the Polymer Chain Arrangement on Exciton and Polaron Dynamics in P3HT and P3HT:PCBM Films}},
    year = {2018},
    journal = {Journal of Physical Chemistry C},
    author = {Dimitriev, Oleg P. and Blank, David A. and Ganser, Christian and Teichert, Christian},
    number = {30},
    pages = {17096--17109},
    volume = {122},
    url = {https://pubs.acs.org/sharingguidelines},
    doi = {10.1021/acs.jpcc.8b05155},
    issn = {19327455}
}

@article{fu2015,
    title = {{Effects of thermal annealing and solvent annealing on the morphologies and properties of poly(3-hexylthiophene) nanowires}},
    year = {2015},
    journal = {Macromolecular Chemistry and Physics},
    author = {Fu, Chuan Min and Jeng, Kai Sheng and Li, Yu Hsun and Hsu, Yuan Chen and Chi, Mu Huan and Jian, Wen Bin and Chen, Jiun Tai},
    number = {1},
    month = {1},
    pages = {59--68},
    volume = {216},
    publisher = {Wiley-VCH Verlag},
    doi = {10.1002/MACP.201400315},
    keywords = {Annealing, Conjugated polymers, Nanowires, Organic field-effect transistors, Poly(3-hexylthiophene)}
}

@article{Ruger2015,
    title = {{Efficient calculation of electronic absorption spectra by means of intensity-selected time-dependent density functional tight binding}},
    year = {2015},
    journal = {Journal of Chemical Theory and Computation},
    author = {R{\"{u}}ger, Robert and Van Lenthe, Erik and Lu, You and Frenzel, Johannes and Heine, Thomas and Visscher, Lucas},
    number = {1},
    month = {1},
    pages = {157--167},
    volume = {11},
    publisher = {American Chemical Society},
    url = {https://pubs.acs.org/doi/full/10.1021/ct500838h},
    doi = {10.1021/ct500838h},
    issn = {15499626}
}

@article{jonna2017,
    title = {{Enhanced Electrical Conductivity of Molecularly p-Doped Poly(3-hexylthiophene) through Understanding the Correlation with Solid-State Order}},
    year = {2017},
    journal = {Macromolecules},
    author = {Hynynen, Jonna and Kiefer, David and Yu, Liyang and Kroon, Renee and Munir, Rahim and Amassian, Aram and Kemerink, Martijn and M{\"{u}}ller, Christian},
    number = {20},
    month = {10},
    pages = {8140--8148},
    volume = {50},
    publisher = {American Chemical Society},
    url = {https://pubs.acs.org/doi/full/10.1021/acs.macromol.7b00968},
    doi = {10.1021/ACS.MACROMOL.7B00968}
}

@misc{jenny2012,
    title = {{Environmental and economic assessment of ITO-free electrodes for organic solar cells}},
    year = {2012},
    booktitle = {Solar Energy Materials and Solar Cells},
    author = {Emmott, Christopher J.M. M and Urbina, Antonio and Nelson, Jenny},
    month = {2},
    pages = {14--21},
    volume = {97},
    url = {www.elsevier.com/locate/solmat},
    doi = {10.1016/j.solmat.2011.09.024},
    issn = {09270248},
    keywords = {Economic analysis, ITO-free, Life cycle analysis, Organic photovoltaics, Polymer solar cells, Transparent conductors}
}

@article{krebs2014,
    title = {{Environmentally printing efficient organic tandem solar cells with high fill factors: A guideline towards 20{\%} power conversion efficiency}},
    year = {2014},
    journal = {Advanced Energy Materials},
    author = {Li, Ning and Baran, Derya and Spyropoulos, George D. and Zhang, Hong and Berny, Stephane and Turbiez, Mathieu and Ameri, Tayebeh and Krebs, Frederik C. and Brabec, Christoph J.},
    number = {11},
    month = {8},
    volume = {4},
    publisher = {Wiley-VCH Verlag},
    doi = {10.1002/AENM.201400084},
    keywords = {flexible electronics, large-scale production, organic photovoltaics, organic solar cells, solution processing}
}

@article{p3ht_temp_2,
    title = {{Excited-State Dynamics and Self-Organization of Poly(3-hexylthiophene) (P3HT) in Solution and Thin Films}},
    year = {2012},
    journal = {The Journal of Physical Chemistry B},
    author = {Ferreira, Bruno and da Silva, Palmira Ferreira and Seixas de Melo, J. Sérgio and Pina, João and Ma{\c{c}}anita, António},
    number = {8},
    month = {3},
    pages = {2347--2355},
    volume = {116},
    publisher = {American Chemical Society},
    url = {https://pubs.acs.org/doi/10.1021/jp207418q},
    doi = {10.1021/jp207418q},
    issn = {1520-6106}
}

@article{Hestand2018,
    title = {{Expanded Theory of H- and J-Molecular Aggregates: The Effects of Vibronic Coupling and Intermolecular Charge Transfer}},
    year = {2018},
    journal = {Chemical Reviews},
    author = {Hestand, Nicholas J. and Spano, Frank C.},
    number = {15},
    month = {8},
    pages = {7069--7163},
    volume = {118},
    publisher = {American Chemical Society},
    url = {https://pubs.acs.org/doi/full/10.1021/acs.chemrev.7b00581},
    doi = {10.1021/ACS.CHEMREV.7B00581},
    issn = {15206890},
    pmid = {29664617}
}

@article{marcial2020,
    title = {{Flexible ITO-Free Roll-Processed Large-Area Nonfullerene Organic Solar Cells Based on P3HT:O-IDTBR}},
    year = {2020},
    journal = {Physical Review Applied},
    author = {Castro, Marcial Fernández and Mazzolini, Eva and Sondergaard, Roar R. and Espindola-Rodriguez, Moises and Andreasen, Jens Wenzel},
    number = {3},
    month = {9},
    pages = {034067},
    volume = {14},
    publisher = {American Physical Society},
    url = {https://journals.aps.org/prapplied/abstract/10.1103/PhysRevApplied.14.034067},
    doi = {10.1103/PhysRevApplied.14.034067}
}

@article{chen2010,
    title = {{Formation and Thermally-Induced Disruption of Nanowhiskers in Poly(3-hexylthiophene)/Xylene Gel Studied by Small-Angle X-ray Scattering}},
    year = {2010},
    journal = {Macromolecules},
    author = {Chen, Chun-Yu and Chan, Shu-Hua and Li, Jian-Yi and Wu, Kuan-Han and Chen, Hsin-Lung and Chen, Jean-Hong and Huang, Wen-Yao and Chen, Show-An},
    number = {17},
    month = {9},
    pages = {7305--7311},
    volume = {43},
    publisher = {American Chemical Society},
    url = {https://pubs.acs.org/doi/full/10.1021/ma1008034},
    doi = {10.1021/MA1008034}
}

@misc{g16,
    title = {{Gaussian16 Revision C.01}},
    year = {2016},
    author = {M. J. Frisch and G. W. Trucks and H. B. Schlegel and G. E. Scuseria and M. A. Robb and J. R. Cheeseman and G. Scalmani and V. Barone and G. A. Petersson and H. Nakatsuji and X. Li and M. Caricato and A. V. Marenich and J. Bloino and B. G. Janesko and R. G, J. A. and J. E. Peralta and F. Ogliaro and M. J. Bearpark and J. J. Heyd and E. N. Brothers and K. N. Kudin and V. N. Staroverov and T. A. Keith and R. Kobayashi and J. Normand and K. Raghavachari and A. P. Rendell and J. C. Burant and S. S. Iyengar and J}
}

@article{Wassenaar2014,
    title = {{Going backward: A flexible geometric approach to reverse transformation from coarse grained to atomistic models}},
    year = {2014},
    journal = {Journal of Chemical Theory and Computation},
    author = {Wassenaar, Tsjerk A. and Pluhackova, Kristyna and B{\"{o}}ckmann, Rainer A. and Marrink, Siewert J. and Tieleman, D. Peter},
    number = {2},
    month = {2},
    pages = {676--690},
    volume = {10},
    publisher = {American Chemical Society},
    url = {https://pubs.acs.org/doi/full/10.1021/ct400617g},
    doi = {10.1021/CT400617G/SUPPL{\_}FILE/CT400617G{\_}SI{\_}002.TXT},
    issn = {15499618}
}

@article{Papadakis2008,
    title = {{Grazing-incidence small-angle X-ray scattering from thin polymer films with lamellar structures - The scattering cross section in the distorted-wave Born approximation}},
    year = {2006},
    journal = {Journal of Applied Crystallography},
    author = {Busch, P. and Rauscher, M. and Smilgies, D. M. and Posselt, D. and Papadakis, C. M.},
    number = {3},
    pages = {433--442},
    volume = {39},
    publisher = {International Union of Crystallography},
    doi = {10.1107/S0021889806012337},
    issn = {00218898}
}

@article{Spano2014,
    title = {{H- and J-aggregate behavior in polymeric semiconductors}},
    year = {2014},
    journal = {Annual Review of Physical Chemistry},
    author = {Spano, Frank C. and Silva, Carlos},
    month = {4},
    pages = {477--500},
    volume = {65},
    publisher = {Annual Reviews},
    url = {https://www.annualreviews.org/doi/abs/10.1146/annurev-physchem-040513-103639},
    doi = {10.1146/annurev-physchem-040513-103639},
    issn = {0066426X},
    pmid = {24423378},
    keywords = {H-aggregates, J-aggregates, conjugated polymers}
}

@article{holiday2016,
    title = {{High-efficiency and air-stable P3HT-based polymer solar cells with a new non-fullerene acceptor}},
    year = {2016},
    journal = {Nature Communications},
    author = {Holliday, Sarah and Ashraf, Raja Shahid and Wadsworth, Andrew and Baran, Derya and Yousaf, Syeda Amber and Nielsen, Christian B. and Tan, Ching Hong and Dimitrov, Stoichko D. and Shang, Zhengrong and Gasparini, Nicola and Alamoudi, Maha and Laquai, Frédéric and Brabec, Christoph J. and Salleo, Alberto and Durrant, James R. and McCulloch, Iain},
    pages = {1--11},
    volume = {7},
    doi = {10.1038/ncomms11585},
    issn = {20411723}
}

@article{jo2020,
    title = {{Impacts of secondary solvents on morphology and charge transport of conjugated polymer thin films}},
    year = {2020},
    journal = {Organic Electronics 81 (2020) 105688 Contents},
    author = {Jo, Gyounglyul and Cho, Hyun and Kim, Hyungwoo and Yoon, Hyeonseok and Han, Sangil and Chang, Mincheol},
    url = {https://doi.org/10.1016/j.orgel.2020.105688 https://reader.elsevier.com/reader/sd/pii/S1566119920300744?token=9D359EFDA5C9636D3AA42D3554DBA844BEDA707463DD4E5B3479C59FC2DD03407387DA2A272646D78A88C737CA522B89&originRegion=eu-west-1&originCreation=2021090909},
    doi = {10.1016/j.orgel.2020.105688},
    keywords = {Charge carrier mobility, Molecular ordering, Morphology, Secondary solvents, Solvent properties poly(3-hexylthiophene)}
}

@article{mksJove,
    title = {{In situ grazing incidence small angle x-ray scattering on roll-to-roll coating of organic solar cells with laboratory x-ray instrumentation}},
    year = {2021},
    journal = {Journal of Visualized Experiments},
    author = {S{\o}rensen, Michael Korning and Rodriguez, Moises Espindola and Castro, Marcial Fernández and Nambi, Ashwin and Kuhn, Luise Theil and Andreasen, Jens Wenzel},
    number = {169},
    month = {3},
    pages = {1--22},
    volume = {2021},
    publisher = {Journal of Visualized Experiments},
    url = {https://www.jove.com/v/61374/in-situ-grazing-incidence-small-angle-x-ray-scattering-on-roll-to},
    doi = {10.3791/61374},
    issn = {1940087X},
    pmid = {33749681},
    keywords = {Issue 169, Teubner-Strey, This Month in JoVE, drying kinetics, in situ GISAXS, non-fullerene acceptor, organic solar cells, roll-to-roll coating, scientific video journal}
}

@article{THz2012,
    title = {{Insights into the charge carrier terahertz mobility in polyfluorenes from large-scale atomistic simulations and time-resolved terahertz spectroscopy}},
    year = {2012},
    journal = {Journal of Physical Chemistry C},
    author = {Vukmirovi{\'{c}}, Nenad and Ponseca, Carlito S and N{\v{e}}mec, Hynek and Yartsev, Arkady and Sundstr{\"{o}}m, Villy},
    number = {37},
    pages = {19665--19672},
    volume = {116},
    url = {https://pubs.acs.org/sharingguidelines},
    isbn = {19665−19672},
    doi = {10.1021/jp3055262},
    issn = {19327447}
}

@article{p3htGold2016,
    title = {{Investigation of Gold and Poly(3-Alkylthiophene) interface in top and bottom contact structures}},
    year = {2016},
    journal = {Synthetic Metals},
    author = {Bhargava, Kshitij and Singh, Vipul},
    month = {1},
    pages = {49--57},
    volume = {211},
    publisher = {Elsevier},
    doi = {10.1016/j.synthmet.2015.11.003},
    issn = {03796779},
    keywords = {Au diffusion, Conjugation length, Energetic disorder, Raman shift, {$\pi$}-conjugated polymer}
}

@article{edward2012,
    title = {{J-Aggregate Behavior in Poly-3-hexylthiophene Nanofibers}},
    year = {2012},
    journal = {J. Phys. Chem. Lett},
    author = {Niles, Edwards T and Roehling, John D and Yamagata, Hajime and Wise, Adam J and Spano, Frank C and Moule, Adam J Moule and Grey, John K},
    volume = {3},
    url = {https://pubs.acs.org/sharingguidelines},
    doi = {10.1021/jz201509h}
}

@article{Sangmin2018,
    title = {{Laser-induced orientation transformation of a conjugated polymer thin film with enhanced vertical charge transport}},
    year = {2018},
    journal = {Journal of Materials Chemistry C},
    author = {Chae, Sangmin and Yi, Ahra and Lee, Hyun Hwi and Choi, Jiyeon and Kim, Hyo Jung},
    number = {35},
    month = {9},
    pages = {9374--9382},
    volume = {6},
    publisher = {The Royal Society of Chemistry},
    url = {https://pubs.rsc.org/en/content/articlehtml/2018/tc/c8tc02393j https://pubs.rsc.org/en/content/articlelanding/2018/tc/c8tc02393j},
    doi = {10.1039/C8TC02393J},
    issn = {2050-7534}
}

@article{Rahimi2014,
    title = {{Light absorption of poly(3-hexylthiophene) single crystals †}},
    year = {2014},
    journal = {Open Access Article. Published on},
    author = {Rahimi, Khosrow and Botiz, Ioan and Agumba, John O and Motamen, Sajedeh and Stingelin, Natalie and ¨ Unter Reiter, G},
    pages = {11121--11123},
    volume = {4},
    url = {www.rsc.org/advances},
    isbn = {1112111123},
    doi = {10.1039/c3ra47064d}
}

@article{Fogh2020,
    title = {{Magnetic structures and quadratic magnetoelectric effect in LiNiPO 4 beyond 30 T}},
    year = {2020},
    journal = {Physical Review B},
    author = {Fogh, E and Kihara, T and Toft-Petersen, R and Bartkowiak, M and Narumi, Y and Prokhnenko, O and Miyake, A and Tokunaga, M and Oikawa, K and S{\o}rensen, M K and Dyrnum, J C and Grimmer, H and Nojiri, H and Christensen, N B},
    number = {2},
    pages = {24403},
    volume = {101},
    publisher = {APA},
    url = {https://doi.org/10.1103/physrevb.101.024403},
    doi = {10.1103/physrevb.101.024403},
    keywords = {Bartkowiak, Maciej, Kihara, Takumi, Miyake, Atsushi, Narumi, Yasuo, Oikawa, Kenichi, Prokhnenko, Oleksandr, S{\o}rensen, Michael Korning, Toft-Petersen, Rasmus, Tokunaga, Masashi}
}

@article{MARIAinstrument,
    title = {{MARIA: Magnetic reflectometer with high incident angle}},
    year = {2015},
    journal = {Journal of large-scale research facilities JLSRF},
    author = {Mattauch, Stefan and Koutsioubas, Alexandros and P{\"{u}}tter, Sabine},
    number = {0},
    month = {8},
    pages = {8},
    volume = {1},
    publisher = {Forschungszentrum Julich, Zentralbibliothek},
    url = {https://jlsrf.org/index.php/lsf/article/view/29},
    doi = {10.17815/JLSRF-1-29},
    issn = {2364-091X}
}

@article{Souza2021,
    title = {{Martini 3: a general purpose force field for coarse-grained molecular dynamics}},
    year = {2021},
    journal = {Nature Methods},
    author = {Souza, Paulo C.T. and Alessandri, Riccardo and Barnoud, Jonathan and Thallmair, Sebastian and Faustino, Ignacio and Gr{\"{u}}newald, Fabian and Patmanidis, Ilias and Abdizadeh, Haleh and Bruininks, Bart M.H. and Wassenaar, Tsjerk A and Kroon, Peter C and Melcr, Josef and Nieto, Vincent and Corradi, Valentina and Khan, Hanif M and Doma{\'{n}}ski, Jan and Javanainen, Matti and Martinez-Seara, Hector and Reuter, Nathalie and Best, Robert B and Vattulainen, Ilpo and Monticelli, Luca and Periole, Xavier and Tieleman, D Peter and de Vries, Alex H. and Marrink, Siewert J},
    number = {4},
    pages = {382--388},
    volume = {18},
    url = {https://doi.org/10.1038/s41592-021-01098-3},
    doi = {10.1038/s41592-021-01098-3},
    issn = {15487105},
    pmid = {33782607}
}

@article{sava2014,
    title = {{Mechanical properties of conjugated polymers and polymer-fullerene composites as a function of molecular structure}},
    year = {2014},
    journal = {Advanced Functional Materials},
    author = {Savagatrup, Suchol and Makaram, Aditya S. and Burke, Daniel J. and Lipomi, Darren J.},
    number = {8},
    month = {2},
    pages = {1169--1181},
    volume = {24},
    publisher = {Wiley-VCH Verlag},
    doi = {10.1002/ADFM.201302646},
    keywords = {conjugated polymers, mechanical properties, organic photovoltaics, polythiophene, stretchable electronics, stretchable solar cells}
}

@misc{asg2021,
    title = {{Molecular dynamics force fields for organic solar cell materials}},
    year = {2021},
    author = {Gertsen, Anders S.},
    doi = {https://doi.org/10.11583/DTU.c.5254236.v1}
}

@article{dag2006,
    title = {{Molecular-weight dependence of interchain polaron delocalization and exciton bandwidth in high-mobility conjugated polymers}},
    year = {2006},
    journal = {Physical Review B - Condensed Matter and Materials Physics},
    author = {Chang, Jui Fen and Clark, Jenny and Zhao, Ni and Sirringhaus, Henning and Breiby, Dag W and Andreasen, Jens W and Nielsen, Martin M and Giles, Mark and Heeney, Martin and McCulloch, Iain},
    number = {11},
    volume = {74},
    doi = {10.1103/PhysRevB.74.115318},
    issn = {10980121},
    keywords = {7280Le, 7361Ph, numbers: 7340Qv}
}

@article{p3ht_temp3,
    title = {{Moving through the phase diagram: Morphology formation in solution cast polymer-fullerene blend films for organic solar cells}},
    year = {2011},
    journal = {ACS Nano},
    author = {Schmidt-Hansberg, Benjamin and Sanyal, Monamie and Klein, Michael F.G. and Pfaff, Marina and Schnabel, Natalie and Jaiser, Stefan and Vorobiev, Alexei and M{\"{u}}ller, Erich and Colsmann, Alexander and Scharfer, Philip and Gerthsen, Dagmar and Lemmer, Uli and Barrena, Esther and Schabel, Wilhelm},
    number = {11},
    pages = {8579--8590},
    volume = {5},
    url = {www.acsnano.org},
    doi = {10.1021/nn2036279},
    issn = {19360851},
    keywords = {P3HT:PCBM, doctor blade, drying kinetics, in situ grazing incidence X-ray diffraction (GIXD), self-assembly, solubility, solvent mixture}
}

@phdthesis{AndersPHD,
    title = {{Multiscale Modelling of Organic Solar Cell Materials}},
    year = {2020},
    author = {Gertsen, Anders S},
    pages = {185},
    school = {Technical University of Denmark},
    isbn = {0000000000000}
}

@article{Lee2014,
    title = {{Nanomorphology evolution of p3ht/pcbm blends during solution-processing from coarse-grained molecular simulations}},
    year = {2014},
    journal = {Journal of Physical Chemistry C},
    author = {Lee, Cheng Kuang and Pao, Chun Wei},
    number = {21},
    month = {5},
    pages = {11224--11233},
    volume = {118},
    publisher = {American Chemical Society},
    url = {https://pubs.acs.org/doi/full/10.1021/jp501323p},
    doi = {10.1021/JP501323P/SUPPL{\_}FILE/JP501323P{\_}SI{\_}001.PDF},
    issn = {19327455}
}

@article{Gertsen2020,
    title = {{Nanostructure of organic semiconductor thin films: Molecular dynamics modeling with solvent evaporation}},
    year = {2020},
    journal = {Physical Review Materials},
    author = {Gertsen, Anders S and S{\o}rensen, Michael Korning and Andreasen, Jens W},
    number = {7},
    volume = {4},
    doi = {10.1103/PhysRevMaterials.4.075405},
    issn = {24759953},
    keywords = {doi:10.1103/PhysRevMaterials.4.075405 url:https://}
}

@article{elsa2016,
    title = {{Ordering of Poly(3-hexylthiophene) in Solutions and Films: Effects of Fiber Length and Grain Boundaries on Anisotropy and Mobility}},
    year = {2016},
    author = {Kleinhenz, Nabil and Persson, Nils and Xue, Zongzhe and Chu, Ping Hsun and Wang, Gang and Yuan, Zhibo and Mcbride, Michael A and Choi, Dalsu and Grover, Martha A and Reichmanis, Elsa},
    url = {https://pubs.acs.org/sharingguidelines},
    doi = {10.1021/acs.chemmater.6b01163}
}

@article{Moritz2021,
    title = {{Organic Solar Cells—The Path to Commercial Success}},
    year = {2021},
    journal = {Advanced Energy Materials},
    author = {Riede, Moritz and Spoltore, Donato and Leo, Karl},
    number = {1},
    month = {1},
    volume = {11},
    publisher = {Wiley-VCH Verlag},
    doi = {10.1002/AENM.202002653},
    keywords = {commercialization, markets, organic photovoltaics, organic solar cells}
}

@article{Roseli2017,
    title = {{Origin of the Excited-State Absorption Spectrum of Polythiophene}},
    year = {2017},
    journal = {Journal of Physical Chemistry Letters},
    author = {Roseli, Ras Baizureen and Tapping, Patrick C. and Kee, Tak W.},
    number = {13},
    month = {7},
    pages = {2806--2811},
    volume = {8},
    publisher = {American Chemical Society},
    url = {https://pubs.acs.org/doi/full/10.1021/acs.jpclett.7b01053},
    doi = {10.1021/ACS.JPCLETT.7B01053/SUPPL{\_}FILE/JZ7B01053{\_}SI{\_}001.PDF},
    issn = {19487185},
    pmid = {28590132}
}

@article{P03Micro,
    title = {{P03, the microfocus and nanofocus X-ray scattering (MiNaXS) beamline of the PETRA III storage ring: The microfocus endstation}},
    year = {2012},
    journal = {Journal of Synchrotron Radiation},
    author = {Buffet, Adeline and Rothkirch, André and D{\"{o}}hrmann, Ralph and K{\"{o}}rstgens, Volker and Abul Kashem, Mottakin M. and Perlich, Jan and Herzog, Gerd and Schwartzkopf, Matthias and Gehrke, Rainer and M{\"{u}}ller-Buschbaum, Peter and Roth, Stephan V},
    number = {4},
    pages = {647--653},
    volume = {19},
    url = {http://www.seso.com/pub/X},
    doi = {10.1107/S0909049512016895},
    issn = {09090495},
    keywords = {X-ray scattering, kinetic studies, microfocus, nanocomposites}
}

@article{P3HT_MW,
    title = {{P3HT Molecular Weight Determines the Performance of P3HT:O-IDTBR Solar Cells}},
    year = {2019},
    journal = {Solar RRL},
    author = {Khan, Jafar Iqbal and Ashraf, Raja Shahid and Alamoudi, Maha A. and Nabi, Mohammed N. and Mohammed, Hamza N. and Wadsworth, Andrew and Firdaus, Yuliar and Zhang, Weimin and Anthopoulos, Thomas D. and McCulloch, Iain and Laquai, Frédéric},
    number = {8},
    month = {8},
    pages = {1900023},
    volume = {3},
    publisher = {John Wiley {\&} Sons, Ltd},
    url = {https://onlinelibrary.wiley.com/doi/full/10.1002/solr.201900023 https://onlinelibrary.wiley.com/doi/abs/10.1002/solr.201900023 https://onlinelibrary.wiley.com/doi/10.1002/solr.201900023},
    doi = {10.1002/solr.201900023},
    issn = {2367198X},
    keywords = {O-IDTBR, molecular weights, nonfullerene acceptors, poly(3-hexylthiophene) (P3HT), transient absorption}
}

@book{ludwigs2014,
    title = {{P3HT Revisited-from Molecular Scale to Solar Cell Devices}},
    year = {2014},
    author = {Ludwigs, Sabine},
    pages = {232},
    publisher = {Springer, Berlin, Heidelberg},
    url = {http://www.springer.com/series/12},
    isbn = {978-3-662-51105-3},
    doi = {https://doi.org/10.1007/978-3-662-45145-8}
}

@article{Gaus2014,
    title = {{Parameterization of DFTB3/3OB for sulfur and phosphorus for chemical and biological applications}},
    year = {2014},
    journal = {Journal of Chemical Theory and Computation},
    author = {Gaus, Michael and Lu, Xiya and Elstner, Marcus and Cui, Qiang},
    number = {4},
    pages = {1518--1537},
    volume = {10},
    url = {https://pubs.acs.org/sharingguidelines},
    doi = {10.1021/ct401002w},
    issn = {15499626}
}

@article{Gaus2013,
    title = {{Parametrization and benchmark of DFTB3 for organic molecules}},
    year = {2013},
    journal = {Journal of Chemical Theory and Computation},
    author = {Gaus, Michael and Goez, Albrecht and Elstner, Marcus},
    number = {1},
    pages = {338--354},
    volume = {9},
    url = {https://pubs.acs.org/sharingguidelines},
    doi = {10.1021/ct300849w},
    issn = {15499618},
    pmid = {26589037}
}

@article{Edberg2016,
    title = {{Patterning and Conductivity Modulation of Conductive Polymers by UV Light Exposure}},
    year = {2016},
    journal = {Advanced Functional Materials},
    author = {Edberg, Jesper and Iandolo, Donata and Brooke, Robert and Liu, Xianjie and Musumeci, Chiara and Andreasen, Jens Wenzel and Simon, Daniel T. and Evans, Drew and Engquist, Isak and Berggren, Magnus},
    number = {38},
    month = {10},
    pages = {6950--6960},
    volume = {26},
    publisher = {John Wiley {\&} Sons, Ltd},
    url = {https://onlinelibrary-wiley-com.proxy.findit.dtu.dk/doi/full/10.1002/adfm.201601794 https://onlinelibrary-wiley-com.proxy.findit.dtu.dk/doi/abs/10.1002/adfm.201601794 https://onlinelibrary-wiley-com.proxy.findit.dtu.dk/doi/10.1002/adfm.201601794},
    doi = {10.1002/adfm.201601794},
    issn = {16163028},
    keywords = {4-ethylenedioxythiophene), conductive polymers, conductivity, organic electronics, patterning, poly(3, vapor phase polymerization}
}

@article{lipomi2017,
    title = {{Poly(3-hexylthiophene) (P3HT): fruit fly or outlier in organic solar cell research?}},
    year = {2017},
    journal = {Journal of Materials Chemistry A},
    author = {T. Kleinschmidt, Andrew and E. Root, Samuel and J. Lipomi, Darren},
    number = {23},
    month = {6},
    pages = {11396--11400},
    volume = {5},
    publisher = {Royal Society of Chemistry},
    url = {https://pubs.rsc.org/en/content/articlehtml/2017/ta/c6ta08317j https://pubs.rsc.org/en/content/articlelanding/2017/ta/c6ta08317j},
    doi = {10.1039/C6TA08317J}
}

@article{Hexemer2011,
    title = {{Polymer crystallization of partially miscible polythiophene/fullerene mixtures controls morphology}},
    year = {2011},
    journal = {Macromolecules},
    author = {Kozub, Derek R. and Vakhshouri, Kiarash and Orme, Lisa M. and Wang, Cheng and Hexemer, Alexander and Gomez, Enrique D.},
    number = {14},
    pages = {5722--5726},
    volume = {44},
    url = {https://pubs.acs.org/sharingguidelines},
    doi = {10.1021/ma200855r},
    issn = {00249297}
}

@article{DanYe2020,
    title = {{Preferred crystallographic orientation of cellulose in plant primary cell walls}},
    year = {2020},
    journal = {Nature Communications},
    author = {Ye, Dan and Rongpipi, Sintu and Kiemle, Sarah N and Barnes, William J and Chaves, Arielle M and Zhu, Chenhui and Norman, Victoria A and Liebman-Pel{\'{a}}ez, Alexander and Hexemer, Alexander and Toney, Michael F and Roberts, Alison W and Anderson, Charles T and Cosgrove, Daniel J and Gomez, Esther W. and Gomez, Enrique D},
    number = {1},
    volume = {11},
    url = {https://doi.org/10.1038/s41467-020-18449-x},
    doi = {10.1038/s41467-020-18449-x},
    issn = {20411723},
    pmid = {32948753}
}

@article{dag2019,
    title = {{Probing Organic Thin Films by Coherent X-ray Imaging and X-ray Scattering}},
    year = {2019},
    journal = {ACS Applied Polymer Materials},
    author = {Patil, Nilesh and Narayanan, Theyencheri and Michels, Leander and Skj{\o}nsfjell, Eirik Torbjørn Bakken and {Bakken} and Guizar-Sicairos, Manuel and Brande, Niko Van den and Claessens, Raf and Mele, Bruno Van and Breiby, Dag Werner and Van den Brande, Niko and Claessens, Raf and Van Mele, Bruno and Breiby, Dag Werner and Torbj{\o}rn, Eirik and Skj{\o}nsfjell, Bakken and Guizar-Sicairos, Manuel and Van den Brande, Niko and Claessens, Raf and Bruno, ⊥ and Mele, Van and Breiby, Dag Werner and Skj{\o}nsfjell, Eirik Torbjørn Bakken and Guizar-Sicairos, Manuel and Van den Brande, Niko and Claessens, Raf and Van Mele, Bruno and Breiby, Dag Werner},
    number = {7},
    month = {7},
    pages = {1787--1797},
    volume = {1},
    publisher = {American Chemical Society},
    url = {https://pubs.acs.org/sharingguidelines https://pubs.acs.org/doi/full/10.1021/acsapm.9b00324},
    doi = {10.1021/acsapm.9b00324},
    issn = {2637-6105},
    keywords = {P3HT, PCBM, SAXS, USAXS, X-ray ptychography, morphology, p3ht, pcbm, saxs, usaxs, x-ray ptychography}
}

@article{nied2013,
    title = {{Probing the relation between charge transport and supramolecular organization down to {\AA}ngstr{\"{o}}m resolution in a benzothiadiazole- cyclopentadithiophene copolymer}},
    year = {2013},
    journal = {Advanced Materials},
    author = {Niedzialek, Dorota and Lemaur, Vincent and Dudenko, Dmytro and Shu, Jie and Hansen, Michael Ryan and Andreasen, Jens Wenzel and Pisula, Wojciech and M{\"{u}}llen, Klaus and Cornil, Jérôme and Beljonne, David},
    number = {13},
    month = {4},
    pages = {1939--1947},
    volume = {25},
    doi = {10.1002/ADMA.201201058},
    keywords = {atomistic modeling, charge transport, conjugated polymer, supramolecular organization}
}

@article{pulseLaser,
    title = {{Pulsed laser annealing of P3HT/PCBM organic solar cells}},
    year = {2010},
    journal = {Solar Energy Materials and Solar Cells},
    author = {Okraku, E. W. and Gupta, M. C. and Wright, K. D.},
    number = {12},
    month = {12},
    pages = {2013--2017},
    volume = {94},
    doi = {10.1016/j.solmat.2010.06.004},
    issn = {09270248},
    keywords = {Laser annealing, Organic solar cells, P3HT, PCBM}
}

@article{Baran2017,
    title = {{Reducing the efficiency-stability-cost gap of organic photovoltaics with highly efficient and stable small molecule acceptor ternary solar cells}},
    year = {2017},
    journal = {Nature Materials},
    author = {Baran, Derya and Ashraf, Raja Shahid and Hanifi, David A and Abdelsamie, Maged and Gasparini, Nicola and R{\"{o}}hr, Jason A and Holliday, Sarah and Wadsworth, Andrew and Lockett, Sarah and Neophytou, Marios and Emmott, Christopher J.M. and Nelson, Jenny and Brabec, Christoph J and Amassian, Aram and Salleo, Alberto and Kirchartz, Thomas and Durrant, James R and McCulloch, Iain},
    number = {3},
    pages = {363--369},
    volume = {16},
    url = {www.nature.com/naturematerials},
    doi = {10.1038/nmat4797},
    issn = {14764660},
    pmid = {27869824}
}

@article{GertCastro2020,
    title = {{Scalable fabrication of organic solar cells based on non-fullerene acceptors}},
    year = {2020},
    journal = {Flexible and Printed Electronics},
    author = {Gertsen, Anders S. and Castro, Marcial Fernández and S{\o}ndergaard, Roar R. and Andreasen, Jens W.},
    number = {1},
    month = {1},
    pages = {014004},
    volume = {5},
    publisher = {IOP Publishing},
    url = {https://iopscience.iop.org/article/10.1088/2058-8585/ab5f57 https://iopscience.iop.org/article/10.1088/2058-8585/ab5f57/meta},
    doi = {10.1088/2058-8585/AB5F57},
    issn = {2058-8585},
    keywords = {non-fullerene acceptors, organic photovoltaics, polymer solar cells, printing and coating, scalable fabrication}
}

@article{DagBrei2008,
    title = {{Simulating X-ray diffraction of textured films}},
    year = {2008},
    journal = {J. Appl. Cryst},
    author = {Breiby, Dag W and Bunk, Oliver and Andreasen, Jens W and Lemke, Henrik T and Nielsen, Martin M},
    pages = {262--271},
    volume = {41},
    doi = {10.1107/S0021889808001064},
    issn = {0021-8898}
}

@article{Green2021,
    title = {{Solar cell efficiency tables (Version 58)}},
    year = {2021},
    journal = {Progress in Photovoltaics: Research and Applications},
    author = {Green, Martin A. and Dunlop, Ewan D. and Hohl-Ebinger, Jochen and Yoshita, Masahiro and Kopidakis, Nikos and Hao, Xiaojing},
    number = {7},
    month = {7},
    pages = {657--667},
    volume = {29},
    publisher = {John Wiley {\&} Sons, Ltd},
    url = {https://onlinelibrary.wiley.com/doi/full/10.1002/pip.3444 https://onlinelibrary.wiley.com/doi/abs/10.1002/pip.3444 https://onlinelibrary.wiley.com/doi/10.1002/pip.3444},
    doi = {10.1002/PIP.3444},
    issn = {1099-159X},
    keywords = {energy conversion efficiency, photovoltaic efficiency, solar cell efficiency}
}

@article{krebs_oneDay,
    title = {{Solar cells with one-day energy payback for the factories of the future}},
    year = {2012},
    journal = {Energy and Environmental Science},
    author = {Espinosa, Nieves and H{\"{o}}sel, Markus and Angmo, Dechan and Krebs, Frederik C.},
    number = {1},
    month = {1},
    pages = {5117--5132},
    volume = {5},
    doi = {10.1039/c1ee02728j},
    issn = {17545692}
}

@article{natalie2015,
    title = {{Solution processing of polymer semiconductor: Insulator blends—Tailored optical properties through liquid–liquid phase separation control}},
    year = {2015},
    journal = {Journal of Polymer Science Part B: Polymer Physics},
    author = {Hellmann, Christoph and Treat, Neil D. and Scaccabarozzi, Alberto D. and Hollis, Joseph Razzell and Fleischli, Franziska D. and Bannock, James H. and Mello, John de and Michels, Jasper J. and Kim, Ji-Seon and Stingelin, Natalie},
    number = {4},
    month = {2},
    pages = {304--310},
    volume = {53},
    publisher = {John Wiley {\&} Sons, Ltd},
    url = {https://www.onlinelibrary.wiley.com/doi/full/10.1002/polb.23656 https://www.onlinelibrary.wiley.com/doi/abs/10.1002/polb.23656 https://onlinelibrary.wiley.com/doi/10.1002/polb.23656},
    doi = {10.1002/POLB.23656},
    issn = {1099-0488},
    keywords = {Spano Model, blends, conjugated polymers, liquid, liquid phase separation, photophysics}
}

@article{dale2013,
    title = {{Solvent quality-induced nucleation and growth of parallelepiped nanorods in dilute poly(3-hexylthiophene) (P3HT) solution and the impact on the crystalline morphology of solution-cast thin film}},
    year = {2013},
    journal = {CrystEngComm},
    author = {Keum, Jong K. and Xiao, Kai and Ivanov, Ilia N. and Hong, Kunlun and Browning, James F. and Smith, Gregory S. and Shao, Ming and Littrell, Kenneth C. and Rondinone, Adam J. and Payzant, E. Andrew and Chen, Jihua and Hensley, Dale K.},
    number = {6},
    month = {1},
    pages = {1114--1124},
    volume = {15},
    publisher = {The Royal Society of Chemistry},
    url = {https://pubs.rsc.org/en/content/articlehtml/2013/ce/c2ce26666k https://pubs.rsc.org/en/content/articlelanding/2013/ce/c2ce26666k},
    doi = {10.1039/C2CE26666K},
    issn = {1466-8033},
    keywords = {dag2019}
}

@article{lipomi2017b,
    title = {{Stretchable and ultraflexible organic electronics}},
    year = {2017},
    journal = {MRS Bulletin 2017 42:2},
    author = {Lipomi, Darren J. and Bao, Zhenan},
    number = {2},
    month = {2},
    pages = {93--97},
    volume = {42},
    publisher = {Springer},
    url = {https://link.springer.com/article/10.1557/mrs.2016.325},
    doi = {10.1557/MRS.2016.325},
    issn = {1938-1425},
    keywords = {Applied and Technical Physics, Characterization and Evaluation of Materials, Energy Materials, Materials Engineering, Materials Science, Nanotechnology, general}
}

@article{YuanYuan2015,
    title = {{Study on {$\pi$}-{$\pi$} Interaction in H- and J-Aggregates of Poly(3-hexylthiophene) Nanowires by Multiple Techniques}},
    year = {2015},
    journal = {Journal of Physical Chemistry B},
    author = {Yuan, Yuan and Shu, Jie and Liu, Ping and Zhang, Yinping and Duan, Yongxin and Zhang, Jianming},
    number = {26},
    month = {7},
    pages = {8446--8456},
    volume = {119},
    publisher = {American Chemical Society},
    url = {https://pubs.acs.org/sharingguidelines},
    doi = {10.1021/acs.jpcb.5b02805},
    issn = {15205207}
}

@article{chu2016,
    title = {{Synergistic Effect of Regioregular and Regiorandom Poly(3-hexylthiophene) Blends for High Performance Flexible Organic Field Effect Transistors}},
    year = {2016},
    journal = {Advanced Electronic Materials},
    author = {Chu, Ping-Hsun and Wang, Gang and Fu, Boyi and Choi, Dalsu and Park, Jung Ok and Srinivasarao, Mohan and Reichmanis, Elsa},
    number = {2},
    month = {2},
    pages = {1500384},
    volume = {2},
    publisher = {John Wiley {\&} Sons, Ltd},
    url = {https://onlinelibrary.wiley.com/doi/full/10.1002/aelm.201500384 https://onlinelibrary.wiley.com/doi/abs/10.1002/aelm.201500384 https://onlinelibrary.wiley.com/doi/10.1002/aelm.201500384},
    doi = {10.1002/AELM.201500384},
    issn = {2199-160X},
    keywords = {hexylthiophene), organic field effect transistor, poly(3, regiorandom, regioregular}
}

@article{Wang2020,
    title = {{Synergistic Optimization Enables Large-Area Flexible Organic Solar Cells to Maintain over 98{\%} PCE of the Small-Area Rigid Devices}},
    year = {2020},
    journal = {Advanced Materials},
    author = {Wang, Guodong and Zhang, Jianqi and Yang, Chen and Wang, Yuheng and Xing, Yi and Adil, Muhammad Abdullah and Yang, Yang and Tian, Lijun and Su, Ming and Shang, Wuqiang and Lu, Kun and Shuai, Zhigang and Wei, Zhixiang},
    number = {49},
    month = {12},
    pages = {2005153},
    volume = {32},
    publisher = {John Wiley {\&} Sons, Ltd},
    url = {https://onlinelibrary.wiley.com/doi/full/10.1002/adma.202005153 https://onlinelibrary.wiley.com/doi/abs/10.1002/adma.202005153 https://onlinelibrary.wiley.com/doi/10.1002/adma.202005153},
    doi = {10.1002/adma.202005153},
    issn = {15214095},
    pmid = {33150635},
    keywords = {flexibility, large-area modules, organic solar cells, shelf stability, slot-die coating}
}

@article{binbin2019,
    title = {{Terahertz time-domain spectroscopy of zone-folded acoustic phonons in 4H and 6H silicon carbide}},
    year = {2019},
    journal = {Optics Express},
    author = {Tarekegne, Abebe T. and Zhou, Binbin and Kaltenecker, Korbinian and Iwaszczuk, Krzysztof and Clark, Stewart and Jepsen, Peter Uhd},
    number = {3},
    month = {2},
    pages = {3618},
    volume = {27},
    publisher = {Optical Society of America},
    url = {https://www.osapublishing.org/viewmedia.cfm?uri=oe-27-3-3618&seq=0&html=true https://www.osapublishing.org/abstract.cfm?uri=oe-27-3-3618 https://www.osapublishing.org/oe/abstract.cfm?uri=oe-27-3-3618},
    doi = {10.1364/oe.27.003618},
    issn = {1094-4087},
    pmid = {30732379},
    keywords = {Femtosecond pulses, Infrared spectroscopy, Pulse generation, Raman spectroscopy, Terahertz generation, Terahertz spectroscopy}
}

@article{MariaMLZ2018,
    title = {{The high-intensity reflectometer of the j{\"{u}}lich centre for neutron science: MARIA}},
    year = {2018},
    journal = {Journal of Applied Crystallography},
    author = {Mattauch, Stefan and Koutsioubas, Alexandros and R{\"{u}}cker, Ulrich and Korolkov, Denis and Fracassi, Vicenzo and Daemen, Jos and Schmitz, Ralf and Bussmann, Klaus and Suxdorf, Frank and Wagener, Michael and K{\"{a}}mmerling, Peter and Kleines, Harald and Fleischhauer-Fu{\ss}, Lydia and Bednareck, Manfred and Ossoviy, Vladimir and Nebel, Andreas and Stronciwilk, Peter and Staringer, Simon and G{\"{o}}del, Marko and Richter, Alfred and Kusche, Harald and Kohnke, Thomas and Ioffe, Alexander and Babcock, Earl and Salhi, Zahir and Bruckel, Thomas},
    pages = {546--654},
    volume = {51},
    url = {https://doi.org/10.1107/S1600576718006994},
    doi = {10.1107/S1600576718006994},
    issn = {16005767},
    keywords = {GISANS, Grazing-incidence small-angle neutron scattering, Magnetism, Polarized neutron reflectometry}
}

@article{krebs2014anneald,
    title = {{The influence of additives on the morphology and stability of roll-to-roll processed polymer solar cells studied through ex situ and in situ X-ray scattering}},
    year = {2014},
    journal = {Journal of Materials Chemistry A},
    author = {Zawacka, Natalia K. and Andersen, Thomas R. and Andreasen, Jens W. and Rossander, Lea H. and Dam, Henrik F. and J{\o}rgensen, Mikkel and Krebs, Frederik C.},
    number = {43},
    month = {11},
    pages = {18644--18654},
    volume = {2},
    publisher = {Royal Society of Chemistry},
    doi = {10.1039/c4ta03484h},
    issn = {20507496}
}

@article{Ming2014,
    title = {{The isotopic effects of deuteration on optoelectronic properties of conducting polymers}},
    year = {2014},
    journal = {Nature Communications},
    author = {Shao, Ming and Keum, Jong and Chen, Jihua and He, Youjun and Chen, Wei and Browning, James F. and Jakowski, Jacek and Sumpter, Bobby G. and Ivanov, Ilia N. and Ma, Ying-Zhong Zhong and Rouleau, Christopher M. and Smith, Sean C. and Geohegan, David B. and Hong, Kunlun and Xiao, Kai},
    month = {1},
    volume = {5},
    url = {www.nature.com/naturecommunications},
    doi = {10.1038/ncomms4180},
    issn = {20411723}
}

@article{someya2015,
    title = {{The rise of plastic bioelectronics}},
    year = {2016},
    journal = {Nature 2016 540:7633},
    author = {Someya, Takao and Bao, Zhenan and Malliaras, George G.},
    number = {7633},
    month = {12},
    pages = {379--385},
    volume = {540},
    publisher = {Nature Publishing Group},
    url = {https://www.nature.com/articles/nature21004},
    doi = {10.1038/nature21004},
    issn = {1476-4687},
    keywords = {Engineering, Materials science}
}

@article{Spano2009,
    title = {{The Spectral Signatures of Frenkel Polarons in H- and J-Aggregates}},
    year = {2009},
    journal = {Accounts of Chemical Research},
    author = {Spano, Frank C.},
    number = {3},
    month = {3},
    pages = {429--439},
    volume = {43},
    publisher = {American Chemical Society},
    url = {https://pubs.acs.org/doi/full/10.1021/ar900233v},
    doi = {10.1021/AR900233V}
}

@article{peng2011,
    title = {{Thermal Annealing Effects on the Absorption and Structural Properties of Regioregular Poly(3-Hexylthiophene) Films}},
    year = {2011},
    journal = {Journal of Macromolecular Science, Part B.},
    author = {Peng, Ruixiang and Zhu, Jun and Pang, Wenmin and Cui, Qi and Wu, Fan and Liu, Ke and Wang, Mingtai and Pan, Guoqiang},
    number = {3},
    month = {2},
    pages = {624--636},
    volume = {50},
    publisher = {Taylor {\&} Francis Group},
    url = {https://www.tandfonline.com/doi/abs/10.1080/00222341003784741},
    doi = {10.1080/00222341003784741},
    keywords = {optical absorption, phase conversion, poly(3-hexylthiophene), thermal annealing}
}

@article{Sales2019,
    title = {{Three dimensional polarimetric neutron tomography - Beyond the phase-wrapping limit}},
    year = {2019},
    journal = {Journal of Physics D: Applied Physics},
    author = {Sales, Morten and Shinohara, Takenao and Sorensen, Michael Korning and Knudsen, Erik B. and Tremsin, Anton and Strobl, Markus and Schmidt, Soren},
    number = {20},
    volume = {51},
    url = {https://doi.org/10.1088/1361-6463/ab0aba},
    isbn = {192.38.90.123},
    doi = {10.1088/1361-6463/ab0aba},
    issn = {13616463},
    keywords = {Neutron imaging, magnetic felds, neutron polarimetry, neutron tomography}
}

@article{Sales2019a,
    title = {{Three dimensional polarimetric neutron tomography—beyond the phase-wrapping limit}},
    year = {2019},
    journal = {Journal of Physics D: Applied Physics},
    author = {Sales, Morten and Shinohara, Takenao and S{\o}rensen, Michael Korning and Knudsen, Erik B and Tremsin, Anton and Strobl, Markus and Schmidt, Søren},
    number = {20},
    month = {3},
    pages = {205001},
    volume = {52},
    publisher = {IOP Publishing},
    doi = {10.1088/1361-6463/AB0ABA},
    issn = {0022-3727}
}

@article{aiar2011,
    title = {{Tunable crystallinity in regioregular poly(3-Hexylthiophene) thin films and its impact on field effect mobility}},
    year = {2011},
    journal = {Advanced Functional Materials},
    author = {Aiyar, Avishek R. and Hong, Jung Il and Nambiar, Rakesh and Collard, David M. and Reichmanis, Elsa},
    number = {14},
    month = {7},
    pages = {2652--2659},
    volume = {21},
    doi = {10.1002/ADFM.201002729},
    keywords = {P3HT, aggregation, mobility, organic field effect transistor, ultrasound, {$\pi$} stacking}
}

@article{medom1999,
    title = {{Two-dimensional charge transport in self-organized, high-mobility conjugated polymers}},
    year = {1999},
    journal = {Nature 1999 401:6754},
    author = {Sirringhaus, H. and Brown, P. J. and Friend, R. H. and Nielsen, M. M. and Bechgaard, K. and Langeveld-Voss, B. M. W. and Spiering, A. J. H. and Janssen, R. A. J. and Meijer, E. W. and Herwig, P. and de Leeuw, D. M.},
    number = {6754},
    month = {10},
    pages = {685--688},
    volume = {401},
    publisher = {Nature Publishing Group},
    url = {https://www.nature.com/articles/44359},
    doi = {10.1038/44359},
    issn = {1476-4687},
    keywords = {Humanities and Social Sciences, Science, multidisciplinary}
}

@article{Kajiya2018,
    title = {{Ultrapure Films of Polythiophene Derivatives are Born on a Substrate by Liquid Flow}},
    year = {2018},
    journal = {ACS Applied Energy Materials},
    author = {Kajiya, Daisuke and Saitow, Ken Ichi},
    number = {12},
    pages = {6881--6889},
    volume = {1},
    doi = {10.1021/acsaem.8b01260},
    issn = {25740962},
    keywords = {aggregate, coffee ring, contact angle, soft electronics, {$\pi$}-conjugated polymer}
}

@article{GTSAXS2021,
    title = {{Uncovering the out-of-plane nanomorphology of organic photovoltaic bulk heterojunction by GTSAXS}},
    year = {2021},
    journal = {Nature Communications},
    author = {Xia, Xinxin and Lau, Tsz Ki and Guo, Xuyun and Li, Yuhao and Qin, Minchao and Liu, Kuan and Chen, Zeng and Zhan, Xiaozhi and Xiao, Yiqun and Chan, Pok Fung and Liu, Heng and Xu, Luhang and Cai, Guilong and Li, Na and Zhu, Haiming and Li, Gang and Zhu, Ye and Zhu, Tao and Zhan, Xiaowei and Wang, Xun Li and Lu, Xinhui},
    number = {1},
    volume = {12},
    url = {https://doi.org/10.1038/s41467-021-26510-6},
    doi = {10.1038/s41467-021-26510-6},
    issn = {20411723},
    pmid = {34711821}
}

@article{brabed2021highthroughput,
    title = {{Understanding the Microstructure Formation of Polymer Films by Spontaneous Solution Spreading Coating with a High-Throughput Engineering Platform}},
    year = {2021},
    journal = {ChemSusChem},
    author = {Wang, Rong and L{\"{u}}er, Larry and Langner, Stefan and Heumueller, Thomas and Forberich, Karen and Zhang, Heyi and Hauch, Jens and Li, Ning and Brabec, Christoph J.},
    number = {17},
    month = {9},
    pages = {3590--3598},
    volume = {14},
    publisher = {John Wiley and Sons Inc},
    doi = {10.1002/cssc.202100927},
    issn = {1864564X},
    pmid = {34236142},
    keywords = {Gaussian process regression, high-throughput engineering, microstructure morphology, organic photovoltaics, spontaneous film spreading}
}

@article{rpm2005,
    title = {{Variations in Semiconducting Polymer Microstructure and Hole Mobility with Spin-Coating Speed}},
    year = {2005},
    journal = {Chemistry of Materials},
    author = {M. DeLongchamp, Dean and M. Vogel, Brandon and Jung, Youngsuk and C. Gurau, Marc and A. Richter, Curt and A. Kirillov, Oleg and Obrzut, Jan and A. Fischer, Daniel and Sambasivan, Sharadha and J. Richter, Lee and K. Lin, Eric},
    number = {23},
    month = {10},
    pages = {5610--5612},
    volume = {17},
    doi = {10.1021/cm0513637}
}

@article{ruger2016,
    title = {{Vibrationally resolved UV/Vis spectroscopy with time-dependent density functional based tight binding}},
    year = {2016},
    journal = {Journal of Chemical Physics},
    author = {R{\"{u}}ger, Robert and Niehaus, Thomas and Van Lenthe, Erik and Heine, Thomas and Visscher, Lucas},
    number = {18},
    month = {11},
    pages = {184102},
    volume = {145},
    publisher = {AIP Publishing LLCAIP Publishing},
    url = {https://aip.scitation.org/doi/abs/10.1063/1.4966918},
    doi = {10.1063/1.4966918},
    issn = {00219606},
    arxivId = {1606.06145},
    keywords = {Franck-Condon factors, Hessian matrices, density functional theory, excited states, tight-binding calculations, ultraviolet spectra, vibrational states, visible spectra, wave functions}
}

@article{rothBA2006,
    title = {{{$\mu$}-GISAXS experiment and simulation of a highly ordered model monolayer of PMMA-beads}},
    year = {2006},
    journal = {Journal of Physical Chemistry B},
    author = {Fr{\"{o}}msdorf, Andreas and {\v{C}}apek, Richard and Roth, Stephan Volkher},
    number = {31},
    pages = {15166--15171},
    volume = {110},
    url = {https://pubs.acs.org/sharingguidelines},
    doi = {10.1021/jp0621880},
    issn = {15206106}
}

@techreport{Pauw2011TheMeasurement,
    title = {{"The Impossible Project"-How to do a perfect SAXS measurement}},
    year = {2011},
    author = {Pauw, Brian R}
}

@misc{NoTitle,
    title = {{(No Title)}},
    url = {https://www.nature.com/articles/ncomms2108.pdf}
}

@article{Krebs201425thParks,
    title = {{25th Anniversary Article: Rise to Power - OPV-Based Solar Parks}},
    year = {2014},
    journal = {Advanced Materials},
    author = {Krebs, Frederik C. and Espinosa, Nieves and H{\"{o}}sel, Markus and S{\o}ndergaard, Roar R. and J{\o}rgensen, Mikkel},
    number = {1},
    month = {1},
    pages = {29--39},
    volume = {26},
    url = {http://doi.wiley.com/10.1002/adma.201302031},
    doi = {10.1002/adma.201302031},
    issn = {09359648},
    keywords = {fast installation, life-cycle analysis, polymer solar cells, roll-to-roll processing, solar parks}
}

@article{Babonneau2010iFitGISAXS/iPro,
    title = {{<i>FitGISAXS</i> : software package for modelling and analysis of GISAXS data using IGOR Pro}},
    year = {2010},
    journal = {Journal of Applied Crystallography},
    author = {Babonneau, David},
    number = {4},
    month = {8},
    pages = {929--936},
    volume = {43},
    url = {http://scripts.iucr.org/cgi-bin/paper?S0021889810020352},
    doi = {10.1107/S0021889810020352},
    issn = {0021-8898},
    keywords = {X-ray scattering, distorted-wave Born approximation}
}

@article{Muller-Buschbaum2009AScattering,
    title = {{A basic introduction to grazing incidence small-angle X-ray scattering}},
    year = {2009},
    journal = {Lecture Notes in Physics},
    author = {M{\"{u}}ller-Buschbaum, P.},
    pages = {61--89},
    volume = {776},
    publisher = {Springer, Berlin, Heidelberg},
    isbn = {9783540959670},
    doi = {10.1007/978-3-540-95968-7{\_}3},
    issn = {00758450}
}

@article{Agbolaghi2017AApplications,
    title = {{A comprehensive review on poly(3-alkylthiophene)-based crystalline structures, protocols and electronic applications}},
    year = {2017},
    author = {Agbolaghi, Samira and Zenoozi, Sahar},
    url = {www.elsevier.com/locate/orgel},
    doi = {10.1016/j.orgel.2017.09.038},
    keywords = {Crystalline structure, Electronic device, P3AT P3HT}
}

@article{Ghasemi2021AStability,
    title = {{A molecular interaction–diffusion framework for predicting organic solar cell stability}},
    year = {2021},
    journal = {Nature Materials},
    author = {Ghasemi, Masoud and Balar, Nrup and Peng, Zhengxing and Hu, Huawei and Qin, Yunpeng and Kim, Taesoo and Rech, Jeromy J. and Bidwell, Matthew and Mask, Walker and McCulloch, Iain and You, Wei and Amassian, Aram and Risko, Chad and O’Connor, Brendan T. and Ade, Harald},
    month = {1},
    pages = {1--8},
    publisher = {Nature Publishing Group},
    url = {http://www.nature.com/articles/s41563-020-00872-6},
    doi = {10.1038/s41563-020-00872-6},
    issn = {1476-1122},
    keywords = {Electronic devices, Organic molecules in materials science, Polymers, Solar cells}
}

@article{Venkatakrishnan2016AScattering,
    title = {{A multi-slice simulation algorithm for grazing-incidence small-angle X-ray scattering}},
    year = {2016},
    journal = {Journal of Applied Crystallography},
    author = {Venkatakrishnan, S. V. and Donatelli, Jeffrey and Kumar, Dinesh and Sarje, Abhinav and Sinha, Sunil K. and Li, Xiaoye S. and Hexemer, Alexander},
    number = {6},
    pages = {1876--1884},
    volume = {49},
    doi = {10.1107/S1600576716013273},
    issn = {16005767},
    keywords = {GISAXS, distorted-wave Born approximation, grazing-incidence small-angle X-ray scattering, multi-slice algorithm}
}

@article{Mahmood2020ACells,
    title = {{A Review of Grazing Incidence Small‐ and Wide‐Angle X‐ray Scattering Techniques for exploring the Film Morphology of Organic Solar Cells}},
    year = {2020},
    journal = {Solar RRL},
    author = {Mahmood, Asif and Wang, Jin-Liang},
    month = {7},
    pages = {solr.202000337},
    url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/solr.202000337},
    doi = {10.1002/solr.202000337},
    issn = {2367-198X}
}

@article{Gurney2019AControl,
    title = {{A review of non-fullerene polymer solar cells: From device physics to morphology control}},
    year = {2019},
    journal = {Reports on Progress in Physics},
    author = {Gurney, Robert S. and Lidzey, David G. and Wang, Tao},
    number = {3},
    volume = {82},
    publisher = {IOP Publishing},
    doi = {10.1088/1361-6633/ab0530},
    issn = {00344885},
    keywords = {efficiency, morphology, non-fullerene, organic photovoltaics, polymer solar cells}
}

@article{Saurel2019AStorage,
    title = {{A SAXS outlook on disordered carbonaceous materials for electrochemical energy storage}},
    year = {2019},
    journal = {Energy Storage Materials},
    author = {Saurel, Damien and Segalini, Julie and Jauregui, María and Pendashteh, Afshin and Daffos, Barbara and Simon, Patrice and Casas-Cabanas, Montse},
    month = {9},
    pages = {162--173},
    volume = {21},
    publisher = {Elsevier B.V.},
    doi = {10.1016/j.ensm.2019.05.007},
    issn = {24058297},
    keywords = {Battery, Disordered carbons, Pore structure, Small angle X-ray scattering, Supercapacitor}
}

@article{Chen2017ALoss,
    title = {{A Wide-Bandgap Donor Polymer for Highly Efficient Non-fullerene Organic Solar Cells with a Small Voltage Loss}},
    year = {2017},
    journal = {Journal of the American Chemical Society},
    author = {Chen, Shangshang and Liu, Yuhang and Zhang, Lin and Chow, Philip C.Y. and Wang, Zheng and Zhang, Guangye and Ma, Wei and Yan, He},
    number = {18},
    pages = {6298--6301},
    volume = {139},
    doi = {10.1021/jacs.7b01606},
    issn = {15205126}
}

@article{Cser2001AboutPolymers,
    title = {{About the Lorentz correction used in the interpretation of small angle X-ray scattering data of semicrystalline polymers}},
    year = {2001},
    journal = {Journal of Applied Polymer Science},
    author = {Cser, F.},
    number = {12},
    pages = {2300--2308},
    volume = {80},
    doi = {10.1002/app.1335},
    issn = {00218995},
    keywords = {Diffraction, Lorentz correction, Poly-ethylene, Semicrystalline polymers, Small angle X-ray scattering}
}

@article{Li2018AchievingRecombination,
    title = {{Achieving over 11{\%} power conversion efficiency in PffBT4T-2OD-based ternary polymer solar cells with enhanced open-circuit-voltage and suppressed charge recombination}},
    year = {2018},
    journal = {Nano Energy},
    author = {Li, Wei and Cai, Jinlong and Cai, Feilong and Yan, Yu and Yi, Hunan and Gurney, Robert S. and Liu, Dan and Iraqi, Ahmed and Wang, Tao},
    month = {2},
    pages = {155--163},
    volume = {44},
    publisher = {Elsevier Ltd},
    doi = {10.1016/j.nanoen.2017.12.005},
    issn = {22112855},
    keywords = {Device physics, Morphology, Polymer solar cells, Ternary solar cells}
}

@article{Fan2019AchievingCells,
    title = {{Achieving over 16{\%} efficiency for single-junction organic solar cells}},
    year = {2019},
    journal = {Science China Chemistry},
    author = {Fan, Baobing and Zhang, Difei and Li, Meijing and Zhong, Wenkai and Zeng, Zhaomiyi and Ying, Lei and Huang, Fei and Cao, Yong},
    publisher = {Science in China Press},
    doi = {10.1007/s11426-019-9457-5},
    issn = {18691870},
    keywords = {high performance, non-fullerene acceptor, organic solar cells, wide bandgap polymer}
}

@article{Hexemer2015AdvancedAnalysis,
    title = {{Advanced grazing-incidence techniques for modern soft-matter materials analysis}},
    year = {2015},
    journal = {IUCrJ},
    author = {Hexemer, Alexander and M{\"{u}}ller-Buschbaum, Peter},
    number = {1},
    month = {1},
    pages = {106--125},
    volume = {2},
    publisher = {International Union of Crystallography},
    doi = {10.1107/S2052252514024178},
    keywords = {GISANS, GISAXS, GIWAXS, grazing-incidence techniques, morphology, resonant soft X-ray scattering, soft matter}
}

@article{Liu2014AggregationCells,
    title = {{Aggregation and morphology control enables multiple cases of high-efficiency polymer solar cells}},
    year = {2014},
    journal = {Nature Communications},
    author = {Liu, Yuhang and Zhao, Jingbo and Li, Zhengke and Mu, Cheng and Ma, Wei and Hu, Huawei and Jiang, Kui and Lin, Haoran and Ade, Harald and Yan, He},
    number = {1},
    month = {11},
    pages = {1--8},
    volume = {5},
    publisher = {Nature Publishing Group},
    url = {www.nature.com/naturecommunications},
    doi = {10.1038/ncomms6293},
    issn = {20411723},
    keywords = {Carbon nanotubes and fullerenes, Polymers, Solar cells}
}

@article{Larsen-Olsen2012AllVacuum,
    title = {{All printed transparent electrodes through an electrical switching mechanism: A convincing alternative to indium-tin-oxide, silver and vacuum}},
    year = {2012},
    journal = {Energy and Environmental Science},
    author = {Larsen-Olsen, Thue T. and Sondergaard, Roar R. and Norrman, Kion and Jorgensen, Mikkel and Krebs, Frederik C.},
    number = {11},
    month = {11},
    pages = {9467--9471},
    volume = {5},
    doi = {10.1039/c2ee23244h},
    issn = {17545692}
}

@article{Abdullah2019All-small-moleculeMorphologies,
    title = {{All-small-molecule organic solar cells with over 14{\%} efficiency by optimizing hierarchical morphologies}},
    year = {2019},
    journal = {Nature Communications},
    author = {Abdullah, Muhammad},
    volume = {10},
    url = {https://doi.org/10.1038/s41467-019-13292-1},
    doi = {10.1038/s41467-019-13292-1}
}

@article{Amonoo2015AnCells,
    title = {{An all-conjugated gradient copolymer approach for morphological control of polymer solar cells}},
    year = {2015},
    journal = {Journal of Materials Chemistry A},
    author = {Amonoo, Jojo A. and Li, Anton and Purdum, Geoffrey E. and Sykes, Matthew E. and Huang, Bingyuan and Palermo, Edmund F. and McNeil, Anne J. and Shtein, Max and Loo, Yueh Lin and Green, Peter F.},
    number = {40},
    pages = {20174--20184},
    volume = {3},
    publisher = {Royal Society of Chemistry},
    doi = {10.1039/c5ta04752h},
    issn = {20507496}
}

@article{Howells2009AnMicroscopy,
    title = {{An assessment of the resolution limitation due to radiation-damage in X-ray diffraction microscopy}},
    year = {2009},
    journal = {Journal of Electron Spectroscopy and Related Phenomena},
    author = {Howells, M.R. and Beetz, T. and Chapman, H.N. and Cui, C. and Holton, J.M. and Jacobsen, C.J. and Kirz, J. and Lima, E. and Marchesini, S. and Miao, H. and Sayre, D. and Shapiro, D.A. and Spence, J.C.H. and Starodub, D.},
    number = {1-3},
    month = {3},
    pages = {4--12},
    volume = {170},
    url = {https://linkinghub.elsevier.com/retrieve/pii/S0368204808001424},
    doi = {10.1016/j.elspec.2008.10.008},
    issn = {03682048},
    keywords = {Coherent X-rays, Diffraction imaging, Dose fractionation, Frozen-hydrated samples, Radiation damage}
}

@article{Cha2017AnAcceptor,
    title = {{An Efficient, “Burn in” Free Organic Solar Cell Employing a Nonfullerene Electron Acceptor}},
    year = {2017},
    journal = {Advanced Materials},
    author = {Cha, Hyojung and Wu, Jiaying and Wadsworth, Andrew and Nagitta, Jade and Limbu, Saurav and Pont, Sebastian and Li, Zhe and Searle, Justin and Wyatt, Mark F. and Baran, Derya and Kim, Ji-Seon Seon and McCulloch, Iain and Durrant, James R.},
    number = {33},
    month = {9},
    pages = {1--8},
    volume = {29},
    url = {http://doi.wiley.com/10.1002/adma.201701156},
    doi = {10.1002/adma.201701156},
    issn = {15214095},
    keywords = {charge separation, nonfullerene acceptors, organic solar cells, trap assisted recombination}
}

@article{Lin2015AnCells,
    title = {{An Electron Acceptor Challenging Fullerenes for Efficient Polymer Solar Cells}},
    year = {2015},
    journal = {Advanced Materials},
    author = {Lin, Yuze and Wang, Jiayu and Zhang, Zhi-Guo and Bai, Huitao and Li, Yongfang and Zhu, Daoben and Zhan, Xiaowei},
    number = {7},
    month = {2},
    pages = {1170--1174},
    volume = {27},
    url = {http://doi.wiley.com/10.1002/adma.201404317},
    doi = {10.1002/adma.201404317},
    issn = {09359648}
}

@article{Cook2008AnalysisP3HT,
    title = {{Analysis of the excited states of regioregular polythiophene P3HT}},
    year = {2008},
    journal = {Energy and Environmental Science},
    author = {Cook, Steffan and Furube, Akihiro and Katoh, Ryuzi},
    number = {2},
    month = {7},
    pages = {294--299},
    volume = {1},
    publisher = {The Royal Society of Chemistry},
    url = {www.rsc.org/ees},
    doi = {10.1039/b805643a},
    issn = {17545692}
}

@article{Li2018AnalyzingMerit,
    title = {{Analyzing the efficiency, stability and cost potential for fullerene-free organic photovoltaics in one figure of merit}},
    year = {2018},
    journal = {Energy and Environmental Science},
    author = {Li, Ning and McCulloch, Iain and Brabec, Christoph J.},
    number = {6},
    month = {6},
    pages = {1355--1361},
    volume = {11},
    publisher = {Royal Society of Chemistry},
    doi = {10.1039/c8ee00151k},
    issn = {17545706}
}

@techreport{ReviEw1963AnomalousRays,
    title = {{Anomalous Surface Reflection of X Rays}},
    year = {1963},
    author = {Revi Ew, Ysicai},
    number = {5},
    volume = {131}
}

@article{Yoneda1963AnomalousRays,
    title = {{Anomalous surface reflection of X rays}},
    year = {1963},
    journal = {Physical Review},
    author = {Yoneda, Y.},
    number = {5},
    month = {9},
    pages = {2010--2013},
    volume = {131},
    publisher = {American Physical Society},
    doi = {10.1103/PhysRev.131.2010},
    issn = {0031899X}
}

@misc{Pescitelli2014ApplicationSystems,
    title = {{Application of electronic circular dichroism in the study of supramolecular systems}},
    year = {2014},
    booktitle = {Chemical Society Reviews},
    author = {Pescitelli, Gennaro and Di Bari, Lorenzo and Berova, Nina},
    number = {15},
    month = {8},
    pages = {5211--5233},
    volume = {43},
    publisher = {Royal Society of Chemistry},
    url = {www.rsc.org/csr},
    doi = {10.1039/c4cs00104d},
    issn = {14604744}
}

@incollection{Riekel2009ApplicationsSciences,
    title = {{Applications of Synchrotron Light to Scattering and Diffraction in Materials and Life Sciences}},
    year = {2009},
    booktitle = {Lecture Notes in Physics},
    author = {Riekel, C and Burghammer, M and Davies, R and Gebhardt, Ronald and Popov, Dmitry},
    editor = {Ezquerra, T.A. and Garcia-Gutierrez, M.C. and Nogales, A. and Gomez, M.},
    number = {2009},
    pages = {91--104},
    volume = {776},
    publisher = {Springer},
    url = {http://www.scopus.com/inward/record.url?eid=2-s2.0-67649446294&partnerID=tZOtx3y1},
    isbn = {978-3-540-95967-0},
    doi = {10.1007/978-3-540-95968-7},
    issn = {00758450}
}

@article{Wang2018ARTICLEGlasses,
    title = {{ARTICLE Spatial correlation of elastic heterogeneity tunes the deformation behavior of metallic glasses}},
    year = {2018},
    journal = {npj Computational Materials},
    author = {Wang, Neng and Ding, Jun and Yan, Feng and Asta, Mark and Ritchie, Robert O and Li, Lin},
    number = {},
    pages = {19},
    volume = {4},
    doi = {10.1038/s41524-018-0077-8}
}

@article{QianArtificialLight,
    title = {{Artificial phototropism for omnidirectional tracking and harvesting of light}},
    author = {Qian, Xiaoshi and Zhao, Yusen and Alsaid, Yousif and Wang, Xu and Hua, Mutian and Galy, Tiphaine and Gopalakrishna, Hamsini and Yang, Yunyun and Cui, Jinsong and Liu, Ning and Marszewski, Michal and Pilon, Laurent and Jiang, Hanqing and He, Ximin},
    url = {https://doi.org/10.1038/s41565-019-0562-3},
    doi = {10.1038/s41565-019-0562-3}
}

@article{Alonzo2013AssemblyPhotovoltaics,
    title = {{Assembly and organization of poly(3-hexylthiophene) brushes and their potential use as novel anode buffer layers for organic photovoltaics}},
    year = {2013},
    journal = {Nanoscale},
    author = {Alonzo, José and Kochemba, W. Michael and Pickel, Deanna L. and Ramanathan, Muruganathan and Sun, Zhenzhong and Li, Dawen and Chen, Jihua and Sumpter, Bobby G. and Heller, William T. and Kilbey, S. Michael},
    number = {19},
    month = {10},
    pages = {9357--9364},
    volume = {5},
    publisher = {The Royal Society of Chemistry},
    url = {www.rsc.org/nanoscale},
    doi = {10.1039/c3nr02226a},
    issn = {20403364},
    pmid = {23955069}
}

@article{Mamusa2019AssociativeWater,
    title = {{Associative properties of poly(ethylene glycol)-poly(vinyl acetate) comb-like graft copolymers in water}},
    year = {2019},
    journal = {Nanoscale},
    author = {Mamusa, Marianna and Tempesti, Paolo and Bartolini, Arianna and Carretti, Emiliano and Ghobadi, Ahmad F. and Smets, Johan and Aouad, Yousef G. and Baglioni, Piero},
    number = {14},
    month = {4},
    pages = {6635--6643},
    volume = {11},
    publisher = {Royal Society of Chemistry},
    doi = {10.1039/c8nr10453k},
    issn = {20403372}
}

@article{Chen2020AsymmetricCells,
    title = {{Asymmetric Alkoxy and Alkyl Substitution on Nonfullerene Acceptors Enabling High‐Performance Organic Solar Cells}},
    year = {2020},
    journal = {Advanced Energy Materials},
    author = {Chen, Yuzhong and Bai, Fujin and Peng, Zhengxing and Zhu, Lei and Zhang, Jianquan and Zou, Xinhui and Qin, Yunpeng and Kim, Ha Kyung and Yuan, Jun and Ma, Lik‐Kuen and Zhang, Jie and Yu, Han and Chow, Philip C. Y. and Huang, Fei and Zou, Yingping and Ade, Harald and Liu, Feng and Yan, He},
    month = {11},
    pages = {2003141},
    volume = {2003141},
    publisher = {John Wiley {\&} Sons, Ltd},
    url = {https://onlinelibrary.wiley.com/doi/10.1002/aenm.202003141},
    doi = {10.1002/aenm.202003141},
    issn = {1614-6832},
    keywords = {Y‐series acceptors, asymmetric alkoxy substitution, morphology, organic solar cells, solubility}
}

@article{Lin2020BalancingLosses,
    title = {{Balancing the pre-aggregation and crystallization kinetics enables high efficiency slot-die coated organic solar cells with reduced non-radiative recombination losses}},
    year = {2020},
    journal = {Energy and Environmental Science},
    author = {Lin, Baojun and Zhou, Xiaobo and Zhao, Heng and Yuan, Jian and Zhou, Ke and Chen, Kai and Wu, Hongbo and Guo, Renjun and Scheel, Manuel A. and Chumakov, Andrei and Roth, Stephan V. and Mao, Yimin and Wang, Laili and Tang, Zheng and M{\"{u}}ller-Buschbaum, Peter and Ma, Wei and Yimin Mao, ef and Wang, Laili and Tang, Zheng and M{\"{u}} ller-Buschbaum, Peter and Ma, Wei},
    number = {8},
    month = {8},
    pages = {2467--2479},
    volume = {13},
    publisher = {Royal Society of Chemistry},
    url = {https://pubs.rsc.org/en/content/articlehtml/2020/ee/d0ee00774a https://pubs.rsc.org/en/content/articlelanding/2020/ee/d0ee00774a},
    doi = {10.1039/d0ee00774a},
    issn = {17545706}
}

@article{Tu2020Barrier-FreeCells,
    title = {{Barrier-Free Charge Separation Enabled by Electronic Polarization in High-Efficiency Non-fullerene Organic Solar Cells}},
    year = {2020},
    journal = {Journal of Physical Chemistry Letters},
    author = {Tu, Zeyi and Han, Guangchao and Yi, Yuanping},
    number = {7},
    month = {4},
    pages = {2585--2591},
    volume = {11},
    publisher = {American Chemical Society},
    doi = {10.1021/acs.jpclett.0c00405},
    issn = {19487185},
    pmid = {32163716}
}

@misc{BenchmarkReader,
    title = {{Benchmark problems for numerical implementations of phase field models | Elsevier Enhanced Reader}},
    url = {https://reader.elsevier.com/reader/sd/pii/S0927025616304712?token=F9A73822EE1CC4A60959161B278D2CD062635858D687E488DB4BA86F5E90F0A0046A33D9A7079CD9BB960DF453CE50F2}
}

@article{Ekimoto2019BiophysicsExperiments,
    title = {{Biophysics and Physicobiology Combination of coarse-grained molecular dynamics simulations and small-angle X-ray scattering experiments}},
    year = {2019},
    author = {Ekimoto, Toru and Kokabu, Yuichi and Oroguchi, Tomotaka and Ikeguchi, Mitsunori},
    pages = {377--390},
    volume = {16},
    url = {https://www.jstage.jst.go.jp/browse/biophysico/},
    doi = {10.2142/biophysico.16.0{\_}377},
    keywords = {MD simulation, SAXS, nucleosome, protein solution structure, structural ensemble}
}

@article{Henemann2008BIPV:Energy,
    title = {{BIPV: Built-in solar energy}},
    year = {2008},
    journal = {Renewable Energy Focus},
    author = {Henemann, Andreas},
    number = {6 SUPPL.},
    month = {11},
    volume = {9},
    doi = {10.1016/S1471-0846(08)70179-3},
    issn = {17550084}
}

@article{Pospelov2020BornAgain:Scattering,
    title = {{BornAgain: software for simulating and fitting grazing-incidence small-angle scattering}},
    year = {2020},
    journal = {J. Appl. Cryst},
    author = {Pospelov, Gennady and Herck, Walter Van and Burle, Jan and Carmona Loaiza, Juan M and Durniak, Céline and Fisher, Jonathan M and Ganeva, Marina and Yurov, Dmitry and Wuttke, Joachim},
    pages = {262--276},
    volume = {53},
    url = {https://doi.org/10.1107/S1600576719016789},
    doi = {10.1107/S1600576719016789},
    keywords = {X-ray scattering, grazing-incidence small-angle scattering (GISAS), neutron scattering, simulation, software}
}

@article{Gasparini2017Burn-inCells,
    title = {{Burn-in Free Nonfullerene-Based Organic Solar Cells}},
    year = {2017},
    journal = {Advanced Energy Materials},
    author = {Gasparini, Nicola and Salvador, Michael and Strohm, Sebastian and Heumueller, Thomas and Levchuk, Ievgen and Wadsworth, Andrew and Bannock, James H. and de Mello, John C. and Egelhaaf, Hans-Joachim Joachim and Baran, Derya and McCulloch, Iain and Brabec, Christoph J.},
    number = {19},
    month = {10},
    pages = {1700770},
    volume = {7},
    publisher = {Wiley-VCH Verlag},
    url = {http://doi.wiley.com/10.1002/aenm.201700770},
    doi = {10.1002/aenm.201700770},
    keywords = {P3HT, degradation, light-soaking stability, nonfullerene acceptor, organic solar cells}
}

@article{Bockmann2015CanP3HT,
    title = {{Can excited electronic states of macromolecules with extended pi-systems be reliably predicted? A case study on P3HT}},
    year = {2015},
    journal = {Frontiers in Materials},
    author = {B{\"{o}}ckmann, Marcus and Doltsinis, Nikos L.},
    month = {4},
    volume = {2},
    publisher = {Frontiers Media S.A.},
    doi = {10.3389/fmats.2015.00025},
    issn = {22968016},
    keywords = {Exchange-correlation functionals, Excited states, Multiscale modeling, Polymers, TDDFT}
}

@article{Chowdhury2001CharacterizationSpectroscopies,
    title = {{Characterization of chiral H and J aggregates of cyanine dyes formed by DNA templating using stark and fluorescence spectroscopies}},
    year = {2001},
    journal = {Journal of Physical Chemistry B},
    author = {Chowdhury, Arindam and Wachsmann-Hogiu, Sebastian and Bangal, Prakriti R. and Raheem, Izzat and Peteanu, Linda A.},
    number = {48},
    pages = {12196--12201},
    volume = {105},
    doi = {10.1021/jp012825g},
    issn = {15206106}
}

@article{Liu2013CharacterizationPhotovoltaics,
    title = {{Characterization of the morphology of solution-processed bulk heterojunction organic photovoltaics}},
    year = {2013},
    journal = {Progress in Polymer Science},
    author = {Liu, Feng and Gu, Yu and Shen, Xiaobo and Ferdous, Sunzida and Wang, Hsin-Wei and Russell, Thomas P.},
    number = {12},
    month = {12},
    pages = {1990--2052},
    volume = {38},
    url = {https://linkinghub.elsevier.com/retrieve/pii/S0079670013000907},
    doi = {10.1016/j.progpolymsci.2013.07.010},
    issn = {00796700},
    keywords = {Bulk heterojunction, Conjugated polymers, Morphology, Organic photovoltaics, Structure}
}

@article{Tiwari2009ChargeSemiconductors,
    title = {{Charge mobility measurement techniques in organic semiconductors}},
    year = {2009},
    journal = {Optical and Quantum Electronics},
    author = {Tiwari, Sanjay and Greenham, N. C.},
    number = {2},
    pages = {69--89},
    volume = {41},
    doi = {10.1007/s11082-009-9323-0},
    issn = {03068919},
    keywords = {Charge transport, Conjugated polymers, Mobility, Organic electronics, Polymeric field-effect transistor, Polymeric light-emitting diode}
}

@article{Clark2009CiteAs,
    title = {{Cite as}},
    year = {2009},
    journal = {The Journal of Chemical Physics},
    author = {Clark, Jenny and Chang, Jui-Fen and Spano, Frank C and Friend, Richard H and Silva, Carlos},
    pages = {184901},
    volume = {94},
    url = {https://doi.org/10.1063/1.3110904},
    doi = {10.1063/1.3110904}
}

@article{Bo2861CiteThis,
    title = {{Cite this}},
    year = {2861},
    journal = {Phys. Chem. Chem. Phys},
    author = {B{\"{o}}, Marcus and Schemme, Thomas and De Jong, Djurre H and Denz, Cornelia and Heuer, Andreas and Doltsinis, Nikos L},
    pages = {28616},
    volume = {17},
    url = {www.rsc.org/pccp},
    doi = {10.1039/c5cp03665h}
}

@article{Rainville2015Co-GISAXSDynamics,
    title = {{Co-GISAXS technique for investigating surface growth dynamics}},
    year = {2015},
    journal = {Physical Review B - Condensed Matter and Materials Physics},
    author = {Rainville, Meliha G. and Wagenbach, Christa and Ulbrandt, Jeffrey G. and Narayanan, Suresh and Sandy, Alec R. and Zhou, Hua and Headrick, Randall L. and Ludwig, Karl F.},
    number = {21},
    pages = {1--8},
    volume = {92},
    doi = {10.1103/PhysRevB.92.214102},
    issn = {1550235X}
}

@article{Queralto2021CombinatorialPrinting,
    title = {{Combinatorial Screening of Cuprate Superconductors by Drop-On-Demand Inkjet Printing}},
    year = {2021},
    journal = {ACS Appl. Mater. Interfaces},
    author = {Queralt{\'{o}}, Albert and Banchewski, Juri and Pacheco, Adrià and Gupta, Kapil and Saltarelli, Lavinia and Garcia, Diana and Alcalde, Núria and Mocuta, Cristian and Ricart, Susagna and Pino, Flavio and Obradors, Xavier and Puig, Teresa},
    pages = {39},
    volume = {13},
    publisher = {UTC},
    url = {www.acsami.org},
    doi = {10.1021/acsami.0c18014},
    keywords = {chemical solution deposition, combinatorial chemistry, cuprate superconductors, high-throughput experimentation, inkjet printing, superconducting materials, transient liquid-assisted growth}
}

@article{Schottl2019CombinedHydrotrope,
    title = {{Combined molecular dynamics (MD) and small angle scattering (SAS) analysis of organization on a nanometer-scale in ternary solvent solutions containing a hydrotrope}},
    year = {2019},
    journal = {Journal of Colloid and Interface Science},
    author = {Sch{\"{o}}ttl, Sebastian and Lopian, Tobias and Pr{\'{e}}vost, Sylvain and Touraud, Didier and Grillo, Isabelle and Diat, Olivier and Zemb, Thomas and Horinek, Dominik},
    month = {3},
    pages = {623--633},
    volume = {540},
    publisher = {Academic Press Inc.},
    doi = {10.1016/j.jcis.2019.01.037},
    issn = {10957103},
    keywords = {Detergentless microemulsion, Molecular dynamics, Pre-Ouzo, Small angle scattering, Surfactant-free microemulsion, Ternary mixtures, Ultraflexible microemulsion}
}

@article{Meng2019CommuniCationCells,
    title = {{CommuniCation A General Approach for Lab-to-Manufacturing Translation on Flexible Organic Solar Cells}},
    year = {2019},
    journal = {Adv. Mater},
    author = {Meng, Xiangchuan and Zhang, Lin and Xie, Yuanpeng P and Hu, Xiaotian and Xing, Zhi and Huang, Zengqi and Liu, Cong and Tan, Licheng and Zhou, Weihua and Sun, Yanming and Ma, Wei and Chen, Yiwang and Meng, Xiangchuan and Hu, Xiaotian and Xing, Zhi and Huang, Zengqi and Liu, Cong and Tan, Licheng and Zhou, Weihua and Chen, Yiwang and Zhang, Lin and Ma, Wei and Xie, Yuanpeng P and Sun, Yanming},
    number = {41},
    pages = {1903649},
    volume = {31},
    url = {https://doi.org/10.1002/adma.201903649.},
    doi = {10.1002/adma.201903649},
    issn = {15214095},
    pmid = {31423693},
    keywords = {flexibility, impulse calculation, modules, organic solar cells, slot-die printing}
}

@article{Gu2016CompactPrinting,
    title = {{Compact Roll-to-Roll Coater for in Situ X-ray Diffraction Characterization of Organic Electronics Printing}},
    year = {2016},
    journal = {ACS Applied Materials {\&} Interfaces},
    author = {Gu, Xiaodan and Reinspach, Julia and Worfolk, Brian J. and Diao, Ying and Zhou, Yan and Yan, Hongping and Gu, Kevin and Mannsfeld, Stefan and Toney, Michael F. and Bao, Zhenan},
    number = {3},
    month = {1},
    pages = {1687--1694},
    volume = {8},
    url = {https://pubs.acs.org/doi/10.1021/acsami.5b09174},
    doi = {10.1021/acsami.5b09174},
    issn = {1944-8244},
    keywords = {X-ray scattering, organic electronics, roll-to-roll process, solar cell, synchrotron radiation}
}

@article{Jones2017ComputationallyMorphology,
    title = {{Computationally connecting organic photovoltaic performance to atomistic arrangements and bulk morphology}},
    year = {2017},
    journal = {Molecular Simulation},
    author = {Jones, Matthew L. and Jankowski, Eric},
    number = {10-11},
    pages = {756--773},
    volume = {43},
    publisher = {Taylor {\&} Francis},
    url = {http://dx.doi.org/10.1080/08927022.2017.1296958},
    doi = {10.1080/08927022.2017.1296958},
    issn = {10290435},
    keywords = {Organic photovoltaics, atomistic backmapping, charge mobility, coarse-grained, diffraction, fine-graining, molecular dynamics}
}

@article{Jankowski2013ComputationallyMorphology,
    title = {{Computationally linking molecular features of conjugated polymers and fullerene derivatives to bulk heterojunction morphology}},
    year = {2013},
    journal = {Macromolecules},
    author = {Jankowski, Eric and Marsh, Hilary S. and Jayaraman, Arthi},
    number = {14},
    pages = {5775--5785},
    volume = {46},
    doi = {10.1021/ma400724e},
    issn = {00249297}
}

@book{Reynolds2019ConjugatedApplications,
    title = {{Conjugated Polymers: Properties, Processing, and Applications}},
    year = {2019},
    author = {Reynolds, John R. and Thompson, Barry C. and Skotheim, Terje A.},
    editor = {Reynolds, John R. and Thompson, Barry C. and Skotheim, Terje A.},
    month = {3},
    publisher = {CRC Press},
    url = {https://www.taylorfrancis.com/books/9781315159294},
    isbn = {9780429190520},
    doi = {10.1201/9780429190520}
}

@article{Hajizadeh2018ConsensusData,
    title = {{Consensus Bayesian assessment of protein molecular mass from solution X-ray scattering data}},
    year = {2018},
    journal = {Scientific Reports},
    author = {Hajizadeh, Nelly R. and Franke, Daniel and Jeffries, Cy M. and Svergun, Dmitri I.},
    number = {1},
    month = {12},
    volume = {8},
    publisher = {Nature Publishing Group},
    doi = {10.1038/s41598-018-25355-2},
    issn = {20452322}
}

@article{Song2018ControllingCells,
    title = {{Controlling Blend Morphology for Ultrahigh Current Density in Nonfullerene Acceptor-Based Organic Solar Cells}},
    year = {2018},
    journal = {ACS Energy Letters},
    author = {Song, Xin and Gasparini, Nicola and Ye, Long and Yao, Huifeng and Hou, Jianhui and Ade, Harald and Baran, Derya},
    number = {3},
    pages = {669--676},
    volume = {3},
    doi = {10.1021/acsenergylett.7b01266},
    issn = {23808195}
}

@article{Leng2022CorrelatingCells,
    title = {{Correlating Electronic Structure and Device Physics with Mixing Region Morphology in High‐Efficiency Organic Solar Cells}},
    year = {2022},
    journal = {Advanced Science},
    author = {Leng, Shifeng and Hao, Tianyu and Zhou, Guanqing and Zhu, Lei and Zhong, Wenkai and Yang, Yankang and Zhang, Ming and Xu, Jinqiu and Zhan, Junzhe and Zhou, Zichun and Chen, Jiajun and Lu, Shirong and Tang, Zheng and Shi, Zhiwen and Zhu, Haiming and Zhang, Yongming and Liu, Feng},
    pages = {2104613},
    url = {https://doi.org/10.1002/advs.202104613},
    doi = {10.1002/advs.202104613},
    issn = {2198-3844}
}

@article{Richards2014CorrelatingMicroscopy,
    title = {{Correlating Structure and Photocurrent for Composite Semiconducting Nanoparticles with Contrast Variation Small-Angle Neutron Scattering and Photoconductive Atomic Force Microscopy}},
    year = {2014},
    journal = {ACS Nano},
    author = {Richards, Jeffrey J. and Whittle, Curtis L. and Shao, Guozheng and Pozzo, Lilo D.},
    number = {5},
    month = {5},
    pages = {4313--4324},
    volume = {8},
    url = {https://pubs.acs.org/doi/10.1021/nn405914g},
    doi = {10.1021/nn405914g},
    issn = {1936-0851}
}

@article{Pauw2013Corrigendum.,
    title = {{Corrigendum : Everything SAXS : small-angle scattering pattern collection and correction ( 2013 J . Phys .: Condens .}},
    year = {2013},
    author = {Pauw, Brian Richard},
    doi = {10.1088/0953-8984/26/23/239501}
}

@article{Wadsworth2019CriticalCells,
    title = {{Critical review of the molecular design progress in non-fullerene electron acceptors towards commercially viable organic solar cells}},
    year = {2019},
    journal = {Chemical Society Reviews},
    author = {Wadsworth, Andrew and Moser, Maximilian and Marks, Adam and Little, Mark S. and Gasparini, Nicola and Brabec, Christoph J. and Baran, Derya and McCulloch, Iain},
    number = {6},
    pages = {1596--1625},
    volume = {48},
    publisher = {Royal Society of Chemistry},
    doi = {10.1039/c7cs00892a},
    issn = {14604744}
}

@misc{CriticalV2.pdf,
    title = {{Critical review of the molecular design progress in nonfullerene v2.pdf}}
}

@misc{Dadsad.pdf,
    title = {{dadsad.pdf}}
}

@article{Harkin2016DecouplingSemiconductor,
    title = {{Decoupling Charge Transport and Electroluminescence in a High Mobility Polymer Semiconductor}},
    year = {2016},
    journal = {Advanced Materials},
    author = {Harkin, David J. and Broch, Katharina and Schreck, Maximilian and Ceymann, Harald and Stoy, Andreas and Yong, Chaw Keong and Nikolka, Mark and McCulloch, Iain and Stingelin, Natalie and Lambert, Christoph and Sirringhaus, Henning},
    pages = {6378--6385},
    publisher = {Wiley-VCH Verlag},
    doi = {10.1002/adma.201600851},
    issn = {15214095},
    keywords = {NIR, energy transfer, fluorescence, organic LEDs}
}

@article{Sim2014DependencePolymers,
    title = {{Dependence of Exciton Diffusion Length on Crystalline Order in Conjugated Polymers}},
    year = {2014},
    journal = {The Journal of Physical Chemistry C},
    author = {Sim, Myungsun and Shin, Jisoo and Shim, Chiyeoung and Kim, Min and Byeok Jo, Sae and Kim, Joo-Hyun and Cho, Kilwon},
    number = {2},
    month = {1},
    pages = {760--766},
    volume = {118},
    doi = {10.1021/jp409776s}
}

@article{Hu2017DesignPhotovoltaics,
    title = {{Design of Donor Polymers with Strong Temperature-Dependent Aggregation Property for Efficient Organic Photovoltaics}},
    year = {2017},
    journal = {Accounts of Chemical Research},
    author = {Hu, Huawei and Chow, Philip C.Y. and Zhang, Guangye and Ma, Tingxuan and Liu, Jing and Yang, Guofang and Yan, He},
    number = {10},
    month = {10},
    pages = {2519--2528},
    volume = {50},
    publisher = {American Chemical Society},
    doi = {10.1021/acs.accounts.7b00293},
    issn = {15204898}
}

@techreport{2020DetectingIndustry,
    title = {{detecting the future Maximum resolution with minimal dimensions laboratory and industry}},
    year = {2020},
    url = {www.dectris.com}
}

@article{Cho2012DeterminationCells,
    title = {{Determination Via Computational Modeling of the Structure-Properties Relationships in Interclated Polymer : Fullerene Blends Found in Bulk-Heterojunction Solar Cells}},
    year = {2012},
    journal = {Georgia Institute of Technology},
    author = {Cho, Eunkyung},
    number = {December}
}

@article{Xiang2017DiameterNanotubes,
    title = {{Diameter and thermal treatment dependent structure and optical properties of poly(3-hexylthiophene) nanotubes}},
    year = {2017},
    journal = {Journal of Materials Chemistry C},
    author = {Xiang, Weizhong and Sun, Xiaoli and Ren, Zhongjie and Zhang, Jianming and Li, Huihui and Yan, Shouke},
    number = {32},
    month = {8},
    pages = {8315--8322},
    volume = {5},
    publisher = {Royal Society of Chemistry},
    url = {https://pubs.rsc.org/en/content/articlehtml/2017/tc/c7tc00947j https://pubs.rsc.org/en/content/articlelanding/2017/tc/c7tc00947j},
    doi = {10.1039/c7tc00947j},
    issn = {20507526}
}

@article{Gann2018DiffractiveFilms,
    title = {{Diffractive X-ray Waveguiding Reveals Orthogonal Crystalline Stratification in Conjugated Polymer Thin Films}},
    year = {2018},
    journal = {Macromolecules},
    author = {Gann, Eliot and Caironi, Mario and Noh, Yong Young and Kim, Yun Hi and McNeill, Christopher R.},
    number = {8},
    pages = {2979--2987},
    volume = {51},
    doi = {10.1021/acs.macromol.8b00168},
    issn = {15205835}
}

@article{Lebert2018DirectingPolymerization,
    title = {{Directing the Aggregation of Native Polythiophene during in Situ Polymerization}},
    year = {2018},
    author = {Lebert, Jenny and Kratzer, Eva M and Bourdick, Axel and Coric, Mihael and Gekle, Stephan and Herzig, Eva M},
    url = {https://pubs.acs.org/sharingguidelines},
    doi = {10.1021/acsomega.8b00684}
}

@article{Darko2019DownloadedDec,
    title = {{Downloaded from orbit.dtu.dk on: dec}},
    year = {2019},
    author = {Darko, C ; and Botiz, I ; and Reiter, G ; and Breiby, D W ; and Andreasen, Jens and Wenzel, ; and Roth, S V ; and Smilgies, D.-M ; and Metwalli, E ; and Papadakis, C M and Darko, C and Botiz, I and Reiter, G and Breiby, D W and Andreasen, J W and Roth, S},
    volume = {19},
    url = {https://doi.org/10.1103/PhysRevE.79.041802},
    doi = {10.1103/PhysRevE.79.041802}
}

@article{Lee2020Eco-FriendlyDesign,
    title = {{Eco-Friendly Polymer Solar Cells: Advances in Green-Solvent Processing and Material Design}},
    year = {2020},
    journal = {ACS Nano},
    author = {Lee, Seungjin and Jeong, Dahyun and Kim, Changkyun and Lee, Changyeon and Kang, Hyunbum and Woo, Han Young and Kim, Bumjoon J.},
    number = {11},
    month = {11},
    pages = {14493--14527},
    volume = {14},
    publisher = {American Chemical Society},
    url = {https://pubs.acs.org/doi/full/10.1021/acsnano.0c07488 https://dx.doi.org/10.1021/acsnano.0c07488},
    issn = {1936086X},
    pmid = {33103903},
    keywords = {eco-friendly polymer solar cells, eco-friendly processing, green solvents, large-area solar cells, long-term stability, non-halogenated solvents, organic solar cells, water/alcohol-based processing}
}

@article{Endo2001EffectMixtures,
    title = {{Effect of amphiphilic block copolymers on the structure and phase behavior of oil-water-surfactant mixtures}},
    year = {2001},
    journal = {Journal of Chemical Physics},
    author = {Endo, H. and Mihailescu, M. and Monkenbusch, M. and Allgaier, J. and Gompper, G. and Richter, D. and Jakobs, B. and Sottmann, T. and Strey, R. and Grillo, I.},
    number = {1},
    month = {7},
    pages = {580--600},
    volume = {115},
    doi = {10.1063/1.1377881},
    issn = {00219606}
}

@article{Bernal2012EffectFoams,
    title = {{Effect of hard segment content and carbon-based nanostructures on the kinetics of flexible polyurethane nanocomposite foams}},
    year = {2012},
    journal = {Polymer},
    author = {Bernal, M. Mar and Martin-Gallego, Mario and Romasanta, Laura J. and Mortamet, Anne-Cecile and L{\'{o}}pez-Manchado, Miguel A. and Ryan, Anthony J. and Verdejo, Raquel},
    number = {19},
    month = {8},
    pages = {4025--4032},
    volume = {53},
    publisher = {Elsevier Ltd},
    url = {https://linkinghub.elsevier.com/retrieve/pii/S0032386112005848},
    doi = {10.1016/j.polymer.2012.07.017},
    issn = {00323861},
    keywords = {Foaming, Kinetics, Polyurethane}
}

@article{Sanyal2011EffectDiffraction,
    title = {{Effect of photovoltaic polymer/fullerene blend composition ratio on microstructure evolution during film solidification investigated in real time by X-ray diffraction}},
    year = {2011},
    journal = {Macromolecules},
    author = {Sanyal, Monamie and Schmidt-Hansberg, Benjamin and Klein, Michael F.G. and Munuera, Carmen and Vorobiev, Alexei and Colsmann, Alexander and Scharfer, Philip and Lemmer, Uli and Schabel, Wilhelm and Dosch, Helmut and Barrena, Esther},
    number = {10},
    month = {5},
    pages = {3795--3800},
    volume = {44},
    publisher = {American Chemical Society},
    doi = {10.1021/ma2000338},
    issn = {00249297}
}

@article{Baghgar2014EffectNanofibers,
    title = {{Effect of Polymer Chain Folding on the Transition from H-to J-Aggregate Behavior in P3HT Nanofibers}},
    year = {2014},
    journal = {J. Phys. Chem. C},
    author = {Baghgar, Mina and Labastide, Joelle A and Bokel, Felicia and Hayward, Ryan C and Barnes, Michael D},
    volume = {118},
    url = {https://pubs.acs.org/sharingguidelines},
    doi = {10.1021/jp411668g}
}

@article{Ruegg2007EffectInteractions,
    title = {{Effect of Pressure on a Multicomponent A/B/A−C Polymer Blend with Attractive and Repulsive Interactions}},
    year = {2007},
    journal = {Macromolecules},
    author = {Ruegg, Megan L. and Reynolds, Benedict J. and Lin, Min Y. and Lohse, David J. and Krishnamoorti, Ramanan and Balsara, Nitash P.},
    number = {2},
    month = {1},
    pages = {355--365},
    volume = {40},
    url = {https://pubs.acs.org/doi/10.1021/ma061894w},
    doi = {10.1021/ma061894w},
    issn = {0024-9297}
}

@article{Chen2018EfficientTransfer,
    title = {{Efficient Nonfullerene Organic Solar Cells with Small Driving Forces for Both Hole and Electron Transfer}},
    year = {2018},
    journal = {Advanced Materials},
    author = {Chen, Shangshang and Wang, Yuming and Zhang, Lin and Zhao, Jingbo and Chen, Yuzhong and Zhu, Danlei and Yao, Huatong and Zhang, Guangye and Ma, Wei and Friend, Richard H. and Chow, Philip C.Y. and Gao, Feng and Yan, He},
    number = {45},
    volume = {30},
    doi = {10.1002/adma.201804215},
    issn = {15214095},
    keywords = {charge transfer, organic solar cells, small-molecular acceptors, voltage loss}
}

@article{Zhao2016EfficientSolvents,
    title = {{Efficient organic solar cells processed from hydrocarbon solvents}},
    year = {2016},
    journal = {Nature Energy},
    author = {Zhao, Jingbo and Li, Yunke and Yang, Guofang and Jiang, Kui and Lin, Haoran and Ade, Harald and Ma, Wei and Yan, He},
    number = {2},
    pages = {15027},
    volume = {1},
    url = {www.nature.com/natureenergy},
    doi = {10.1038/NENERGY.2015.27},
    issn = {20587546}
}

@article{Liu2012EfficientBlends,
    title = {{Efficient Polymer Solar Cells Based on a Low Bandgap Semi-crystalline DPP Polymer-PCBM Blends}},
    year = {2012},
    journal = {Advanced Materials},
    author = {Liu, Feng and Gu, Yu and Wang, Cheng and Zhao, Wei and Chen, Dian and Briseno, Alejandro L. and Russell, Thomas P.},
    number = {29},
    month = {8},
    pages = {3947--3951},
    volume = {24},
    publisher = {John Wiley {\&} Sons, Ltd},
    url = {http://doi.wiley.com/10.1002/adma.201200902},
    doi = {10.1002/adma.201200902},
    issn = {09359648},
    keywords = {X-ray scattering, low bandgap polymers, photovoltaic devices, polymer solar cells, resonant soft X-rays}
}

@article{Stoltzfus2020ElectronicInformation,
    title = {{Electronic Supplementary Information}},
    year = {2020},
    author = {Stoltzfus, Dani M and Joshi, Gajadhar and Popli, Henna and Jamali, Shirin and Kavand, Marzieh and Milster, Sebastian and Bange, Sebastian and Nahlawi, Adnan and Teferi, Mandefro Y and Atwood, Sabastian I and Leung, Anna E and Darwish, Tamim A and Malissa, Hans and Burn, Paul L and Lupton, John M and Boehme, Christoph},
    pages = {1--15}
}

@misc{Proller2020ElectrophoresisFilms,
    title = {{Electrophoresis Assisted Printing: A Method to Control the Morphology in Organic Thin Films}},
    year = {2020},
    booktitle = {ACS Applied Materials and Interfaces},
    author = {Pr{\"{o}}ller, Stephan and Filonik, Oliver and Eller, Fabian and Mansi, Salma and Zhu, Chenhui and Schaible, Eric and Hexemer, Alexander and M{\"{u}}ller-Buschbaum, Peter and Herzig, Eva M.},
    number = {5},
    month = {2},
    pages = {5219--5225},
    volume = {12},
    publisher = {American Chemical Society},
    doi = {10.1021/acsami.9b18064},
    issn = {19448252},
    keywords = {controlling vertical segregation, electric field during printing, electrophoresis, printed solar cells, slot die coating}
}

@book{Als-Nielsen2011ElementsEdition,
    title = {{Elements of Modern X-ray Physics: Second Edition}},
    year = {2011},
    booktitle = {Elements of Modern X-ray Physics: Second Edition},
    author = {Als-Nielsen, Jens and McMorrow, Des},
    month = {4},
    publisher = {John Wiley and Sons},
    isbn = {9780470973950},
    doi = {10.1002/9781119998365}
}

@article{Hoefler2019ElucidationMobility,
    title = {{Elucidation of Donor:Acceptor Phase Separation in Nonfullerene Organic Solar Cells and Its Implications on Device Performance and Charge Carrier Mobility}},
    year = {2019},
    journal = {ACS Applied Energy Materials},
    author = {Hoefler, Sebastian F. and Haberfehlner, Georg and Rath, Thomas and Keilbach, Andreas and Hobisch, Mathias A. and Dixon, Alex and Pavlica, Egon and Bratina, Gvido and Kothleitner, Gerald and Hofer, Ferdinand and Trimmel, Gregor},
    number = {10},
    month = {10},
    pages = {7535--7545},
    volume = {2},
    url = {https://pubs.acs.org/sharingguidelines https://pubs.acs.org/doi/10.1021/acsaem.9b01534},
    doi = {10.1021/acsaem.9b01534},
    issn = {2574-0962},
    keywords = {bulk-heterojunction, charge carrier mobility, nanomorphology, organic photovoltaics, scanning transmission electron microscopy}
}

@book{DanishEnergyAgency2018EnergistatistikKort,
    title = {{Energistatistik 2017: Data, tabeller, statistikker og kort}},
    year = {2018},
    author = {{Danish Energy Agency}},
    isbn = {9788793180369}
}

@article{Ji2020EnergyProspects,
    title = {{Energy Loss in Organic Solar Cells: Mechanisms, Strategies, and Prospects}},
    year = {2020},
    journal = {Solar RRL},
    author = {Ji, Yiwen and Xu, Lingxia and Hao, Xiaotao and Gao, Kun},
    month = {5},
    pages = {2000130},
    publisher = {Wiley},
    url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/solr.202000130},
    doi = {10.1002/solr.202000130},
    issn = {2367-198X},
    keywords = {charge transfers, energy losses, nonradiative recombination, organic solar cells, power conversion efficiencies}
}

@article{He2012EnhancedStructure,
    title = {{Enhanced power-conversion efficiency in polymer solar cells using an inverted device structure}},
    year = {2012},
    journal = {Nature Photonics},
    author = {He, Zhicai and Zhong, Chengmei and Su, Shijian and Xu, Miao and Wu, Hongbin and Cao, Yong},
    number = {9},
    month = {9},
    pages = {591--595},
    volume = {6},
    publisher = {Nature Publishing Group},
    doi = {10.1038/nphoton.2012.190},
    issn = {17494885},
    keywords = {Solar energy and photovoltaic technology}
}

@article{Ko2020EnhancedNanoconfinement,
    title = {{Enhanced Vertical Charge Transport of Homo-and Blended Semiconducting Polymers by Nanoconfinement}},
    year = {2020},
    author = {Ko, Jongkuk and Kim, Youngkeol and Kang, Jin Soo and Berger, Rüdiger and Yoon, Hyunsik and Char, Kookheon and Ko, J and Kim, Y and Char, K and Kang, J S and Berger, R and Yoon, H},
    url = {https://doi.org/10.1002/adma.201908087.},
    doi = {10.1002/adma.201908087}
}

@article{Pauw2013EverythingCorrection,
    title = {{Everything SAXS: Small-angle scattering pattern collection and correction}},
    year = {2013},
    journal = {Journal of Physics Condensed Matter},
    author = {Pauw, Brian Richard},
    number = {38},
    pages = {1--2},
    volume = {25},
    doi = {10.1088/0953-8984/25/38/383201},
    issn = {09538984},
    arxivId = {arXiv:1306.0637v1}
}

@article{Dudenas2019EvolutionStudy,
    title = {{Evolution of Ionomer Morphology from Dispersion to Film: An in Situ X-ray Study}},
    year = {2019},
    author = {Dudenas, Peter J and Kusoglu, Ahmet},
    url = {https://pubs.acs.org/sharingguidelines},
    doi = {10.1021/acs.macromol.9b01024}
}

@article{Muller2012ExcitedBlends,
    title = {{Excited States in P3HT and P3HT/PCBM Blends}},
    year = {2012},
    journal = {BioNanoScience},
    author = {M{\"{u}}ller, K. and Richter, M. and Philip, S. and Kunst, M. and Schmei{\ss}er, D.},
    number = {1},
    month = {1},
    pages = {42--51},
    volume = {2},
    publisher = {Springer New York LLC},
    url = {https://link.springer.com/article/10.1007/s12668-011-0031-4},
    doi = {10.1007/s12668-011-0031-4},
    issn = {21911649},
    keywords = {Exciton dissociation, Excitons, P3HT, Polarons, TRMC, UPS, XAS}
}

@article{He2014FacilitatingGrafts,
    title = {{Facilitating hydroxide transport in anion exchange membranes via hydrophilic grafts}},
    year = {2014},
    journal = {Journal of Materials Chemistry A},
    author = {He, Steve S. and Frank, Curtis W.},
    number = {39},
    month = {10},
    pages = {16489--16497},
    volume = {2},
    publisher = {Royal Society of Chemistry},
    url = {http://dx.doi.org/10.1039/C4TA02942A},
    doi = {10.1039/c4ta02942a},
    issn = {20507496}
}

@article{Liu2015FastCoating,
    title = {{Fast printing and in situ morphology observation of organic photovoltaics using slot-die coating}},
    year = {2015},
    journal = {Advanced Materials},
    author = {Liu, Feng and Ferdous, Sunzida and Schaible, Eric and Hexemer, Alexander and Church, Matthew and Ding, Xiaodong and Wang, Cheng and Russell, Thomas P.},
    number = {5},
    month = {2},
    pages = {886--891},
    volume = {27},
    url = {http://doi.wiley.com/10.1002/adma.201404040},
    doi = {10.1002/adma.201404040},
    issn = {15214095}
}

@article{Weu2018Field-AssistedCells,
    title = {{Field-Assisted Exciton Dissociation in Highly Efficient PffBT4T-2OD:Fullerene Organic Solar Cells}},
    year = {2018},
    journal = {Chemistry of Materials},
    author = {Weu, Andreas and Hopper, Thomas R. and Lami, Vincent and Kre{\ss}, Joshua A. and Bakulin, Artem A. and Vaynzof, Yana},
    number = {8},
    month = {4},
    pages = {2660--2667},
    volume = {30},
    publisher = {American Chemical Society},
    doi = {10.1021/acs.chemmater.8b00094},
    issn = {15205002}
}

@article{Diao2015Flow-enhancedCells,
    title = {{Flow-enhanced solution printing of all-polymer solar cells}},
    year = {2015},
    journal = {Nature Communications},
    author = {Diao, Ying and Zhou, Yan and Kurosawa, Tadanori and Shaw, Leo and Wang, Cheng and Park, Steve and Guo, Yikun and Reinspach, Julia A. and Gu, Kevin and Gu, Xiaodan and Tee, Benjamin C.K. and Pang, Changhyun and Yan, Hongping and Zhao, Dahui and Toney, Michael F. and Mannsfeld, Stefan C.B. and Bao, Zhenan},
    volume = {6},
    publisher = {Nature Publishing Group},
    doi = {10.1038/ncomms8955},
    issn = {20411723}
}

@article{Proller2016FollowingCells,
    title = {{Following the Morphology Formation In Situ in Printed Active Layers for Organic Solar Cells}},
    year = {2016},
    journal = {Advanced Energy Materials},
    author = {Pr{\"{o}}ller, Stephan and Liu, Feng and Zhu, Chenhui and Wang, Cheng and Russell, Thomas P. and Hexemer, Alexander and M{\"{u}}ller-Buschbaum, Peter and Herzig, Eva M.},
    number = {1},
    month = {1},
    pages = {1501580},
    volume = {6},
    publisher = {Wiley-VCH Verlag},
    url = {http://doi.wiley.com/10.1002/aenm.201501580},
    doi = {10.1002/aenm.201501580},
    issn = {16146832},
    keywords = {crystallization, morphology, organic solar cells, printed solar cells, structure formation}
}

@article{Niebuur2018FormationJumps,
    title = {{Formation and Growth of Mesoglobules in Aqueous Poly(N-isopropylacrylamide) Solutions Revealed with Kinetic Small-Angle Neutron Scattering and Fast Pressure Jumps}},
    year = {2018},
    journal = {ACS Macro Letters},
    author = {Niebuur, Bart Jan and Chiappisi, Leonardo and Zhang, Xiaohan and Jung, Florian and Schulte, Alfons and Papadakis, Christine M.},
    number = {10},
    month = {10},
    pages = {1155--1160},
    volume = {7},
    publisher = {American Chemical Society},
    doi = {10.1021/acsmacrolett.8b00605},
    issn = {21611653}
}

@article{Ye2012FromCells,
    title = {{From Binary to Ternary Solvent: Morphology Fine-tuning of D/A Blends in PDPP3T-based Polymer Solar Cells}},
    year = {2012},
    journal = {Advanced Materials},
    author = {Ye, Long and Zhang, Shaoqing and Ma, Wei and Fan, Benhu and Guo, Xia and Huang, Ye and Ade, Harald and Hou, Jianhui},
    number = {47},
    month = {12},
    pages = {6335--6341},
    volume = {24},
    publisher = {John Wiley {\&} Sons, Ltd},
    url = {http://doi.wiley.com/10.1002/adma.201202855},
    doi = {10.1002/adma.201202855},
    issn = {09359648},
    keywords = {diketopyrrolopyrrole, domain purity, morphology, polymer solar cells, ternary mixed solvent}
}

@article{Han2018FromCells,
    title = {{From Molecular Packing Structures to Electronic Processes: Theoretical Simulations for Organic Solar Cells}},
    year = {2018},
    journal = {Advanced Energy Materials},
    author = {Han, Guangchao and Yi, Yuanping and Shuai, Zhigang},
    number = {28},
    month = {10},
    pages = {1702743},
    volume = {8},
    publisher = {Wiley-VCH Verlag},
    url = {http://doi.wiley.com/10.1002/aenm.201702743},
    doi = {10.1002/aenm.201702743},
    issn = {16146832},
    keywords = {charge transfer, molecular dynamics, molecular packing, photoelectric conversion, quantum chemistry}
}

@article{Sharma2017Ga-dopedCells,
    title = {{Ga-doped ZnO as an electron transport layer for PffBT4T-2OD: PC70BM organic solar cells}},
    year = {2017},
    journal = {Organic Electronics: physics, materials, applications},
    author = {Sharma, Ramakant and Lee, Hyunwoo and Borse, Kunal and Gupta, Vinay and Joshi, Amish G. and Yoo, Seunghyup and Gupta, Dipti},
    pages = {207--213},
    volume = {43},
    publisher = {Elsevier B.V},
    url = {http://dx.doi.org/10.1016/j.orgel.2017.01.028},
    doi = {10.1016/j.orgel.2017.01.028},
    issn = {15661199},
    keywords = {Electron transport layers, Ga-doped ZnO, Hole blocking layer, Organic solar cells, PffBT4T-2OD:PC70BM}
}

@article{Perlich2010GrazingHASYLAB,
    title = {{Grazing incidence wide angle x-ray scattering at the wiggler beamline BW4 of HASYLAB}},
    year = {2010},
    author = {Perlich, J and Rubeck, J and Botta, S and Gehrke, R and Roth, S V and Ruderer, M A and Prams, S M and Rawolle, M and Zhong, Q and K{\"{o}}rstgens, V and M{\"{u}}ller-Buschbaum, P},
    url = {http://rsi.aip.org/about/rights_and_permissions},
    doi = {10.1063/1.3488459}
}

@article{Nouhi2017Grazing-incidenceInterface,
    title = {{Grazing-incidence small-angle neutron scattering from structures below an interface}},
    year = {2017},
    journal = {Journal of Applied Crystallography},
    author = {Nouhi, Shirin and Hellsing, Maja S. and Kapaklis, Vassilios and Rennie, Adrian R.},
    pages = {1066--1074},
    volume = {50},
    publisher = {International Union of Crystallography},
    doi = {10.1107/S1600576717007518},
    issn = {16005767},
    keywords = {GISANS, colloidal particles, grazing-incidence small-angle neutron scattering, solid/liquid interfaces}
}

@article{ChukhovskiiGrazing-incidenceFormalism,
    title = {{Grazing-incidence small-angle X-ray scattering in a twofold rough-interface medium: a new theoretical approach using the q-eigenwave formalism}},
    author = {Chukhovskii, F N and Roshchin, B S},
    url = {http://dx.doi.org/10.1107/S2053273315016666},
    doi = {10.1107/S2053273315016666}
}

@article{Lucera2015GuidelinesModules,
    title = {{Guidelines for Closing the Efficiency Gap between Hero Solar Cells and Roll-To-Roll Printed Modules}},
    year = {2015},
    journal = {Energy Technology},
    author = {Lucera, Luca and Kubis, Peter and Fecher, Frank W. and Bronnbauer, Carina and Turbiez, Mathieu and Forberich, Karen and Ameri, Tayebeh and Egelhaaf, Hans-Joachim and Brabec, Christoph J.},
    number = {4},
    month = {4},
    pages = {373--384},
    volume = {3},
    url = {http://doi.wiley.com/10.1002/ente.201402192},
    doi = {10.1002/ente.201402192},
    issn = {21944288}
}

@article{Spano2014H-Semiconductors,
    title = {{H- and J-Aggregate Behavior in Polymeric Semiconductors}},
    year = {2014},
    journal = {Annual Review of Physical Chemistry},
    author = {Spano, Frank C. and Silva, Carlos},
    number = {1},
    month = {4},
    pages = {477--500},
    volume = {65},
    publisher = {Annual Reviews Inc.},
    url = {http://www.annualreviews.org/doi/10.1146/annurev-physchem-040513-103639},
    doi = {10.1146/annurev-physchem-040513-103639},
    issn = {0066-426X},
    keywords = {H-aggregates, J-aggregates, conjugated polymers}
}

@article{Mai2017HighPolymers,
    title = {{High efficiency ternary organic solar cell with morphology-compatible polymers}},
    year = {2017},
    journal = {Journal of Materials Chemistry A},
    author = {Mai, Jiangquan and Lu, Haipeng and Lau, Tsz Ki and Peng, Shih Hao and Hsu, Chain Shu and Hua, Wenqiang and Zhao, Ni and Xiao, Xudong and Lu, Xinhui},
    number = {23},
    pages = {11739--11745},
    volume = {5},
    publisher = {Royal Society of Chemistry},
    doi = {10.1039/c7ta00292k},
    issn = {20507496}
}

@article{Na2019HighCoating,
    title = {{High Performance Roll-to-Roll Produced Fullerene-Free Organic Photovoltaic Devices via Temperature-Controlled Slot Die Coating}},
    year = {2019},
    journal = {Advanced Functional Materials},
    author = {Na, Seok In and Seo, You Hyun and Nah, Yoon Chae and Kim, Seok Soon and Heo, Hyojung and Kim, Jueng Eun and Rolston, Nicholas and Dauskardt, Reinhold H. and Gao, Mei and Lee, Youngu and Vak, Doojin},
    number = {6},
    pages = {1--10},
    volume = {29},
    doi = {10.1002/adfm.201805825},
    issn = {16163028},
    keywords = {3d printer, flexible solar cells, nonfullerene acceptor, printed solar cells, roll-to-roll}
}

@article{Nikolka2019High-mobilityDiodes,
    title = {{High-mobility, trap-free charge transport in conjugated polymer diodes}},
    year = {2019},
    journal = {Nature Communications},
    author = {Nikolka, Mark and Broch, Katharina and Armitage, John and Hanifi, David and Nowack, Peer J. and Venkateshvaran, Deepak and Sadhanala, Aditya and Saska, Jan and Mascal, Mark and Jung, Seok Heon and Lee, Jin Kyun and McCulloch, Iain and Salleo, Alberto and Sirringhaus, Henning},
    number = {1},
    month = {12},
    volume = {10},
    publisher = {Nature Publishing Group},
    doi = {10.1038/s41467-019-10188-y},
    issn = {20411723}
}

@article{Fan2018High-PerformanceEfficiency,
    title = {{High-Performance As-Cast Nonfullerene Polymer Solar Cells with Thicker Active Layer and Large Area Exceeding 11{\%} Power Conversion Efficiency}},
    year = {2018},
    journal = {Advanced Materials},
    author = {Fan, Qunping and Wang, Yan and Zhang, Maojie and Wu, Bo and Guo, Xia and Jiang, Yufeng and Li, Wanbin and Guo, Bing and Ye, Chennan and Su, Wenyan and Fang, Jin and Ou, Xuemei and Liu, Feng and Wei, Zhixiang and Sum, Tze Chien and Russell, Thomas P. and Li, Yongfang},
    number = {6},
    pages = {1--7},
    volume = {30},
    doi = {10.1002/adma.201704546},
    issn = {15214095},
    keywords = {large area, nonfullerene polymer solar cells, thicker active layer, wide-bandgap polymer donor, without extra treatments}
}

@article{Donnelly2016High-resolutionPtychography,
    title = {{High-resolution hard x-ray magnetic imaging with dichroic ptychography}},
    year = {2016},
    journal = {Physical Review B},
    author = {Donnelly, Claire and Scagnoli, Valerio and Guizar-Sicairos, Manuel and Holler, Mirko and Wilhelm, Fabrice and Guillou, Francois and Rogalev, Andrei and Detlefs, Carsten and Menzel, Andreas and Raabe, Jörg and Heyderman, Laura J.},
    number = {6},
    pages = {1--10},
    volume = {94},
    doi = {10.1103/PhysRevB.94.064421},
    issn = {24699969},
    arxivId = {arXiv:1603.03588v3}
}

@article{Chumakov2019High-resolutionNanostructures,
    title = {{High-resolution SAXS setup with tuneable resolution in direct and reciprocal space: a new tool to study ordered nanostructures}},
    year = {2019},
    journal = {J. Appl. Cryst},
    author = {Chumakov, Andrei P and Napolskii, Kirill S and Petukhov, Andrei V and Snigirev, Anatoly A and Snigireva, Irina I and Roslyakov, Ilya V and Grigoriev, Sergey V},
    pages = {1095--1103},
    volume = {52},
    url = {https://doi.org/10.1107/S1600576719011221},
    doi = {10.1107/S1600576719011221},
    keywords = {anodic alumina Russian Federation, f Physics Institute, NRC Kurchatov Institute, Gatchina, Leningrad Region 188300, Russian Federation, and, compound refractive lenses, microradian diffraction, small-angle X-ray scattering}
}

@article{Bottiger2012High-throughputLayers,
    title = {{High-throughput roll-to-roll X-ray characterization of polymer solar cell active layers}},
    year = {2012},
    journal = {Journal of Materials Chemistry},
    author = {B{\"{o}}ttiger, Arvid P L and Jorgensen, Mikkel and Menzel, Andreas and Krebs, Frederik C. and Andreasen, Jens W.},
    number = {42},
    pages = {22501--22509},
    volume = {22},
    doi = {10.1039/c2jm34596j},
    issn = {09599428}
}

@article{Wadsworth2017HighlySolvents,
    title = {{Highly Efficient and Reproducible Nonfullerene Solar Cells from Hydrocarbon Solvents}},
    year = {2017},
    journal = {ACS Energy Letters},
    author = {Wadsworth, Andrew and Ashraf, Raja S. and Abdelsamie, Maged and Pont, Sebastian and Little, Mark and Moser, Maximilian and Hamid, Zeinab and Neophytou, Marios and Zhang, Weimin and Amassian, Aram and Durrant, James R. and Baran, Derya and McCulloch, Iain},
    number = {7},
    pages = {1494--1500},
    volume = {2},
    doi = {10.1021/acsenergylett.7b00390},
    issn = {23808195}
}

@article{Xu2015HomogeneousCells,
    title = {{Homogeneous phase separation in polymer:Fullerene bulk heterojunction organic solar cells}},
    year = {2015},
    journal = {Organic Electronics: physics, materials, applications},
    author = {Xu, Wei Long and Wu, Bo and Zheng, Fei and Wang, Hua Bin and Wang, Yu Zhu and Bian, Feng Gang and Hao, Xiao Tao and Zhu, Furong},
    month = {7},
    pages = {266--274},
    volume = {25},
    publisher = {Elsevier},
    doi = {10.1016/j.orgel.2015.06.042},
    issn = {15661199},
    keywords = {Bulk heterojunction, Homogeneous distribution, Organic solar cells, Phase separation}
}

@misc{HoppingMobility.pdf,
    title = {{Hopping transport electron mobility.pdf}}
}

@article{Song2018HotCells,
    title = {{Hot slot die coating for additive-free fabrication of high performance roll-to-roll processed polymer solar cells}},
    year = {2018},
    journal = {Energy and Environmental Science},
    author = {Song, Seyeong and Lee, Kang Taek and Koh, Chang Woo and Shin, Hyebeom and Gao, Mei and Woo, Han Young and Vak, Doojin and Kim, Jin Young},
    number = {11},
    pages = {3248--3255},
    volume = {11},
    publisher = {Royal Society of Chemistry},
    doi = {10.1039/c8ee02221f},
    issn = {17545706}
}

@misc{IEEEPDF:,
    title = {{IEEE Xplore Full-Text PDF:}},
    url = {https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=6925260}
}

@article{Bristow2019ImpactMobility,
    title = {{Impact of Nonfullerene Acceptor Side Chain Variation on Transistor Mobility}},
    year = {2019},
    author = {Bristow, Helen and Thorley, Karl J and White, Andrew J P and Wadsworth, Andrew and Babics, Maxime and Hamid, Zeinab and Zhang, Weimin and Paterson, Alexandra F and Kosco, Jan and Panidi, Julianna and Anthopoulos, Thomas D and Mcculloch, Iain},
    url = {https://doi.org/10.1002/aelm.201900344.},
    doi = {10.1002/aelm.201900344}
}

@article{Winkler2019ImpactAerogels,
    title = {{Impact of Solvent Structuring in Water/tert-Butanol Mixtures on the Assembly of Silica Nanoparticles to Aerogels}},
    year = {2019},
    journal = {Langmuir},
    author = {Winkler, Robert and R{\'{e}}, Elisa and Arrachart, Guilhem and Pellet-Rostaing, Stéphane},
    number = {24},
    month = {6},
    pages = {7905--7915},
    volume = {35},
    publisher = {American Chemical Society},
    doi = {10.1021/acs.langmuir.9b00655},
    issn = {15205827}
}

@article{Bi2018ImportanceCells,
    title = {{Importance of Nucleation during Morphology Evolution of the Blade-Cast PffBT4T-2OD-Based Organic Solar Cells}},
    year = {2018},
    journal = {Macromolecules},
    author = {Bi, Zhaozhao and Naveed, Hafiz Bilal and Mao, Yimin and Yan, Hongping and Ma, Wei and Hafiz, † and Naveed, Bilal and Mao, Yimin and Yan, Hongping and Ma, Wei},
    number = {17},
    month = {9},
    pages = {6682--6691},
    volume = {51},
    url = {https://pubs.acs.org/sharingguidelines https://pubs.acs.org/doi/10.1021/acs.macromol.8b01156},
    doi = {10.1021/acs.macromol.8b01156},
    issn = {0024-9297}
}

@article{Herzog2013InSilicon,
    title = {{In situ grazing incidence small-angle X-ray scattering investigation of polystyrene nanoparticle spray deposition onto silicon}},
    year = {2013},
    journal = {Langmuir},
    author = {Herzog, Gerd and Benecke, Gunthard and Buffet, Adeline and Heidmann, Berit and Perlich, Jan and Risch, Johannes F.H. and Santoro, Gonzalo and Schwartzkopf, Matthias and Yu, Shun and Wurth, Wilfried and Roth, Stephan V.},
    number = {36},
    month = {9},
    pages = {11260--11266},
    volume = {29},
    publisher = {American Chemical Society},
    doi = {10.1021/la402254q},
    issn = {07437463}
}

@article{Rossander2014InCoating,
    title = {{In situ monitoring of structure formation in the active layer of polymer solar cells during roll-to-roll coating}},
    year = {2014},
    journal = {AIP Advances},
    author = {Rossander, Lea H. and Zawacka, Natalia K. and Dam, Henrik F. and Krebs, Frederik C. and Andreasen, Jens W.},
    number = {8},
    volume = {4},
    doi = {10.1063/1.4892526},
    issn = {21583226}
}

@article{Schmidt-Hansberg2009InCells,
    title = {{In situ monitoring the drying kinetics of knife coated polymer-fullerene films for organic solar cells}},
    year = {2009},
    journal = {Journal of Applied Physics},
    author = {Schmidt-Hansberg, B. and Klein, M. F.G. and Peters, K. and Buss, F. and Pfeifer, J. and Walheim, S. and Colsmann, A. and Lemmer, U. and Scharfer, P. and Schabel, W.},
    number = {12},
    volume = {106},
    doi = {10.1063/1.3270402},
    issn = {00218979}
}

@article{Wienhold2020InAcceptor,
    title = {{In Situ Printing: Insights into the Morphology Formation and Optical Property Evolution of Slot‐Die‐Coated Active Layers Containing Low Bandgap Polymer Donor and Nonfullerene Small Molecule Acceptor}},
    year = {2020},
    journal = {Solar RRL},
    author = {Wienhold, Kerstin S. and Korstgens, Volker and Grott, Sebastian and Jiang, Xinyu and Schwartzkopf, Matthias and Roth, Stephan V. and M{\"{u}}ller-Buschbaum, Peter},
    number = {7},
    month = {7},
    pages = {2000086},
    volume = {4},
    publisher = {Wiley-VCH Verlag},
    url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/solr.202000086},
    doi = {10.1002/solr.202000086},
    issn = {2367-198X},
    keywords = {GISAXS, in situ printing, low bandgap polymers, nonfullerene acceptors, slot-die coating}
}

@article{Yang2020InCells,
    title = {{In Situ Studies of Solvent Additive Effects on the Morphology Development during Printing of Bulk Heterojunction Films for Organic Solar Cells}},
    year = {2020},
    journal = {Small Methods},
    author = {Yang, Dan and Grott, Sebastian and Jiang, Xinyu and Wienhold, Kerstin S. and Schwartzkopf, Matthias and Roth, Stephan V. and M{\"{u}}ller‐Buschbaum, Peter},
    number = {9},
    month = {8},
    pages = {2000418},
    volume = {4},
    publisher = {John Wiley and Sons Inc.},
    url = {https://onlinelibrary.wiley.com/doi/10.1002/smtd.202000418 https://onlinelibrary.wiley.com/doi/abs/10.1002/smtd.202000418},
    doi = {10.1002/smtd.202000418},
    issn = {23669608},
    keywords = {PPDT2FBT:PC71BM films, crystallinity, morphology, printing, solvent additive}
}

@article{Li2020InPrinting,
    title = {{In Situ Study of Order Formation in Mesoporous Titania Thin Films Templated by a Diblock Copolymer during Slot-Die Printing}},
    year = {2020},
    journal = {ACS Applied Materials and Interfaces},
    author = {Li, Nian and Chen, Wei and Song, Lin and Guo, Renjun and Scheel, Manuel A. and Yang, Dan and Korstgens, Volker and Schwartzkopf, Matthias and Roth, Stephan V. and M{\"{u}}ller-Buschbaum, Peter},
    pages = {57637},
    volume = {12},
    publisher = {American Chemical Society},
    url = {https://dx.doi.org/10.1021/acsami.0c18851},
    doi = {10.1021/acsami.0c18851},
    issn = {19448252},
    keywords = {hybrid films, in situ GISAXS, self-assembly, slot-die printing, titania nanostructures}
}

@article{Son2019In-depthStructures,
    title = {{In-depth optical characterization of poly(3-hexylthiophene) after formation of nanosecond laser-induced periodic surface structures}},
    year = {2019},
    journal = {Nanoscale},
    author = {Son, Sung Yun and Kang, Gyeongho and Kim, Minjun and Lee, Junwoo and Kim, Taewan and Park, Taiho and Lim, Jongchul},
    number = {16},
    month = {4},
    pages = {7567--7571},
    volume = {11},
    publisher = {Royal Society of Chemistry},
    doi = {10.1039/c8nr10075f},
    issn = {20403372}
}

@article{Rossander2017In-lineLayers,
    title = {{In-line, roll-to-roll morphology analysis of organic solar cell active layers}},
    year = {2017},
    journal = {Energy Environ. Sci.},
    author = {Rossander, Lea Hildebrandt and Dam, Henrik Friis and Carl{\'{e}}, Jon Eggert and Helgesen, Martin and Rajkovic, Ivan and Corazza, Michael and Krebs, Frederik Christian and Andreasen, Jens Wenzel},
    pages = {2411--2419},
    doi = {10.1039/C7EE01900A},
    issn = {1754-5692}
}

@article{Bhattacharyya2017In-SituSensitivity,
    title = {{In-Situ GISAXS study of supramolecular nanofibers having ultrafast humidity sensitivity}},
    year = {2017},
    journal = {Scientific Reports},
    author = {Bhattacharyya, Arpan and Sanyal, Milan K. and Mogera, Umesha and George, Subi J. and Mukhopadhyay, Mrinmay K. and Maiti, Santanu and Kulkarni, Giridhar U.},
    number = {1},
    pages = {1--11},
    volume = {7},
    publisher = {Nature Publishing Group},
    doi = {10.1038/s41598-017-00309-2},
    issn = {20452322}
}

@article{ZhangIndacenodithiopheneTransistors,
    title = {{Indacenodithiophene Semiconducting Polymers for High-Performance, Air-Stable Transistors}},
    author = {Zhang, Weimin and Smith, Jeremy and Watkins, Scott E and Gysel, Roman and Mcgehee, Michael and Salleo, Alberto and Kirkpatrick, James and Ashraf, Shahid and Anthopoulos, Thomas and Heeney, Martin and Mcculloch, Iain},
    url = {http://pubs.acs.org.},
    doi = {10.1021/ja1049324}
}

@article{Hynynen2018InfluenceF4TCNQ,
    title = {{Influence of crystallinity on the thermoelectric power factor of P3HT vapour-doped with F4TCNQ}},
    year = {2018},
    author = {Hynynen, Jonna and Kiefer, David and Uller, Christian M ¨},
    doi = {10.1039/c7ra11912g}
}

@article{Hamid2020InfluenceCells,
    title = {{Influence of Polymer Aggregation and Liquid Immiscibility on Morphology Tuning by Varying Composition in PffBT4T-2DT / Nonfullerene Organic Solar Cells}},
    year = {2020},
    journal = {Advanced Energy Materials},
    author = {Hamid, Zeinab and Wadsworth, Andrew and Rezasoltani, Elham and Holliday, Sarah and Azzouzi, Mohammed and Neophytou, Marios and Guilbert, Anne A. Y. and Dong, Yifan and Little, Mark S. and Mukherjee, Subhrangsu and Herzing, Andrew A. and Bristow, Helen and Kline, R. Joseph and Delongchamp, Dean M. and Bakulin, Artem A. and Durrant, James R. and Nelson, Jenny and McCulloch, Iain},
    number = {8},
    month = {2},
    pages = {1--13},
    volume = {1903248},
    publisher = {Wiley-VCH Verlag},
    url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/aenm.201903248},
    doi = {10.1002/aenm.201903248},
    issn = {1614-6832},
    keywords = {calorimetry, morphology, nonfullerene, organic photovoltaics, phase behavior}
}

@article{Otalora2014InfluenceSolution,
    title = {{Influence of solvent on the molecular ordering of thin films of P3HT:PCBM blends and precursor solution}},
    year = {2014},
    journal = {2014 IEEE 40th Photovoltaic Specialist Conference, PVSC 2014},
    author = {Otalora, Camilo A. and Loaiza, Andres F. and Gordillo, Gerardo},
    pages = {1754--1757},
    isbn = {9781479943982},
    doi = {10.1109/PVSC.2014.6925260},
    keywords = {P3HT:PCBM thin films, molecular ordering, optical and structural properties, solvent effect}
}

@article{Busch2007InnerScattering,
    title = {{Inner structure of thin films of lamellar poly(styrene-b-butadiene) diblock copolymers as revealed by grazing-incidence small-angle scattering}},
    year = {2007},
    journal = {Macromolecules},
    author = {Busch, P. and Posselt, D. and Smilgies, D. M. and Rauscher, M. and Papadakis, C. M.},
    number = {3},
    pages = {630--640},
    volume = {40},
    doi = {10.1021/ma061695c},
    issn = {00249297}
}

@article{Salleo2004IntrinsicPolythiophene,
    title = {{Intrinsic hole mobility and trapping in a regioregular poly(thiophene)}},
    year = {2004},
    journal = {Physical Review B - Condensed Matter and Materials Physics},
    author = {Salleo, A. and Chen, T. W. and V{\"{o}}lkel, A. R. and Wu, Y. and Liu, P. and Ong, B. S. and Street, R. A.},
    number = {11},
    pages = {1--10},
    volume = {70},
    doi = {10.1103/PhysRevB.70.115311},
    issn = {01631829}
}

@article{Schwartzkopf2016InvestigatingStudies,
    title = {{Investigating Polymer–Metal Interfaces by Grazing Incidence Small-Angle X-Ray Scattering from Gradients to Real-Time Studies}},
    year = {2016},
    journal = {Nanomaterials},
    author = {Schwartzkopf, Matthias and Roth, Stephan V.},
    number = {12},
    month = {12},
    pages = {239},
    volume = {6},
    publisher = {MDPI AG},
    url = {http://www.mdpi.com/2079-4991/6/12/239},
    doi = {10.3390/nano6120239},
    issn = {2079-4991},
    keywords = {Grazing incidence X-ray scattering, Growth kinetics, In situ, Nanocomposites, Nanostructure formation, Polymer template, Polymer–metal interfaces, Sputter deposition, X-ray scattering}
}

@article{Vegso2017KineticsScattering,
    title = {{Kinetics of Polymer-Fullerene Phase Separation during Solvent Annealing Studied by Table-Top X-ray Scattering}},
    year = {2017},
    journal = {ACS Applied Materials and Interfaces},
    author = {Vegso, Karol and Siffalovic, Peter and Jergel, Matej and Nadazdy, Peter and Nadazdy, Vojtech and Majkova, Eva},
    number = {9},
    pages = {8241--8247},
    volume = {9},
    doi = {10.1021/acsami.6b15167},
    issn = {19448252},
    keywords = {GI-SAXS, GI-WAXS, P3HT:PCBM, solar cell, solvent annealing}
}

@article{Wang2019LargeAreaMethods,
    title = {{Large‐Area Organic Solar Cells: Material Requirements, Modular Designs, and Printing Methods}},
    year = {2019},
    journal = {Advanced Materials},
    author = {Wang, Guodong and Adil, Muhammad Abdullah and Zhang, Jianqi and Wei, Zhixiang},
    number = {45},
    month = {11},
    pages = {1805089},
    volume = {31},
    publisher = {Wiley-VCH Verlag},
    url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/adma.201805089},
    doi = {10.1002/adma.201805089},
    issn = {0935-9648},
    keywords = {large-area devices, modular design, organic solar cells, printing, thick film}
}

@article{Feng2017Laser-inducedOf,
    title = {{Laser-induced crystallization and conformation control of poly ( 3- hexylthiophene ) for improving the performance of organic solar cells Laser-induced crystallization and conformation control of poly ( 3- hexylthiophene ) for improving the performance of}},
    year = {2017},
    journal = {Organic Electronics},
    author = {Feng, Lin and Zheng, Fei and Bi, Peng-qing and Yang, Xiao-yu and Niu, Meng-si and Wang, Fei},
    number = {June},
    pages = {157--164},
    volume = {49},
    publisher = {Elsevier B.V},
    url = {http://dx.doi.org/10.1016/j.orgel.2017.06.053},
    doi = {10.1016/j.orgel.2017.06.053},
    issn = {1566-1199}
}

@article{Cui2016Laser-InducedBM,
    title = {{Laser-Induced Periodic Surface Structures on P3HT and on Its Photovoltaic Blend with PC 71 BM}},
    year = {2016},
    author = {Cui, Jing and Lvaro Rodr{\'{i}}guez-Rodr{\'{i}}guez, A ́ and Hernándezhernández, Margarita and Garc{\'{i}}a-Gutiérrezgutiérrez, Mari-Cruz and Nogales, Aurora and Castillejo, Marta and Mosegu{\'{i}} Gonza{\'{i}}ez, Daniel and Mü Ller-Buschbaum, Peter and Ezquerra, Tiberio A and Rebollar, Esther},
    url = {www.acsami.org},
    doi = {10.1021/acsami.6b09053},
    keywords = {grazing incidence X-ray scattering, laser-induced periodic surface structures, organic photovoltaics, polymer films, semiconductor polymers}
}

@techreport{EditorsLecturePhysics,
    title = {{Lecture Notes in Physics}},
    author = {Editors, Founding and Beiglb{\"{o}}ck, W and Ehlers, J and Hepp, K and Weidenm{\"{u}}ller, H and L{\"{o}}hneysen, H and Mangano, Germany M and J-M Raimond, Switzerland and Sornette, France D}
}

@misc{LinZhang.pdf,
    title = {{lin Zhang.pdf}}
}

@article{Bundgaard2007LowPhotovoltaics,
    title = {{Low band gap polymers for organic photovoltaics}},
    year = {2007},
    journal = {Solar Energy Materials and Solar Cells},
    author = {Bundgaard, Eva and Krebs, Frederik C.},
    number = {11},
    pages = {954--985},
    volume = {91},
    doi = {10.1016/j.solmat.2007.01.015},
    issn = {09270248},
    keywords = {Low band gap polymers, Organic photovoltaics (OPV), Synthesis}
}

@article{Fogh2020MagneticT,
    title = {{Magnetic structures and quadratic magnetoelectric effect in {\$}{\{}{\textbackslash}rm LiNiPO{\}}{\_}4{\$} beyond 30 T}},
    year = {2020},
    journal = {Physical Review B},
    author = {Fogh, Ellen and Kihara, Takumi and Toft-Petersen, Rasmus and Bartkowiak, Maciej and Narumi, Yasuo and Prokhnenko, Oleksandr and Miyake, Atsushi and Tokunaga, Masashi and Oikawa, Kenichi and S{\o}rensen, Michael Korning and Dyrnum, Julia Cathrine and Grimmer, Hans and Nojiri, Hiroyuki and Christensen, Niels Bech},
    pages = {24403},
    volume = {101},
    doi = {10.1103/PhysRevB.101.024403},
    keywords = {doi:10.1103/PhysRevB.101.024403 url:https://doi.org/10.1103/PhysRevB.101.024403}
}

@article{Grant2015MainObjectives,
    title = {{Main Objectives}},
    year = {2015},
    author = {Grant, E R C Consolidator and Part, Seewhi and Smalley, Richard and Challenge, The Terawatt},
    pages = {1--15}
}

@article{Zhang2018MaterialAcceptors,
    title = {{Material insights and challenges for non-fullerene organic solar cells based on small molecular acceptors}},
    year = {2018},
    journal = {Nature Energy},
    author = {Zhang, Jianquan and Tan, Huei Shuan and Guo, Xugang and Facchetti, Antonio and Yan, He},
    number = {9},
    pages = {720--731},
    volume = {3},
    publisher = {Springer US},
    url = {http://dx.doi.org/10.1038/s41560-018-0181-5},
    doi = {10.1038/s41560-018-0181-5},
    issn = {20587546}
}

@article{Finn2018MechanicalTorsion,
    title = {{Mechanical stability of roll-to-roll printed solar cells under cyclic bending and torsion}},
    year = {2018},
    journal = {Solar Energy Materials and Solar Cells},
    author = {Finn, Mickey and Martens, Christian James and Zaretski, Aliaksandr V. and Roth, Bérenger and S{\o}ndergaard, Roar R. and Krebs, Frederik C. and Lipomi, Darren J.},
    number = {June 2017},
    pages = {7--15},
    volume = {174},
    publisher = {Elsevier B.V.},
    url = {http://dx.doi.org/10.1016/j.solmat.2017.08.015},
    doi = {10.1016/j.solmat.2017.08.015},
    issn = {09270248},
    keywords = {Barrier encapsulation, Conjugated polymer, Cyclic fatigue testing, Flexible electronics, Mechanical stability, Organic solar cell}
}

@article{Collins2011MiscibilityStability,
    title = {{Miscibility, Crystallinity, and Phase Development in P3HT/PCBM Solar Cells: Toward an Enlightened Understanding of Device Morphology and Stability}},
    year = {2011},
    journal = {J. Phys. Chem.Lett},
    author = {Collins, Brian A and Tumbleston, John R and Ade, Harald},
    pages = {3145},
    volume = {2},
    url = {https://pubs.acs.org/sharingguidelines},
    doi = {10.1021/jz2014902}
}

@article{Spano2005ModelingFilms,
    title = {{Modeling disorder in polymer aggregates: The optical spectroscopy of regioregular poly(3-hexylthiophene) thin films}},
    year = {2005},
    journal = {Journal of Chemical Physics},
    author = {Spano, Frank C.},
    number = {23},
    month = {6},
    pages = {234701},
    volume = {122},
    publisher = {American Institute of PhysicsAIP},
    url = {https://aip.scitation.org/doi/abs/10.1063/1.1914768},
    doi = {10.1063/1.1914768},
    issn = {00219606},
    keywords = {Gaussian distribution, aggregation, infrared spectra, phonon-exciton interactions, photoluminescence, polymer films, spectral line breadth, spectral line intensity, ultraviolet spectra, visible spectra}
}

@techreport{Wodo2012ModelingCells,
    title = {{Modeling morphology evolution during solvent-based fabrication of organic solar cells}},
    year = {2012},
    booktitle = {Computational Materials Science},
    author = {Wodo, Olga and Ganapathysubramanian, Baskar},
    month = {4},
    pages = {113--126},
    volume = {55},
    publisher = {Elsevier},
    doi = {10.1016/j.commatsci.2011.12.012},
    issn = {09270256},
    arxivId = {1109.3239v2},
    keywords = {Cahn-Hilliard equation, Evaporation, Morphology evolution, Organic solar cells, Phase separation, Substrate patterning, evaporation, morphology evolution *, organic solar cells, phase separation, substrate patterning}
}

@article{Few2015ModelsCells,
    title = {{Models of charge pair generation in organic solar cells}},
    year = {2015},
    journal = {Physical Chemistry Chemical Physics},
    author = {Few, Sheridan and Frost, Jarvist M. and Nelson, Jenny},
    number = {4},
    pages = {2311--2325},
    volume = {17},
    publisher = {Royal Society of Chemistry},
    url = {http://dx.doi.org/10.1039/C4CP03663H},
    doi = {10.1039/c4cp03663h},
    issn = {14639076}
}

@article{Li2019MolecularCells,
    title = {{Molecular Order Control of Non-fullerene Acceptors for High-Efficiency Polymer Solar Cells}},
    year = {2019},
    journal = {Joule},
    author = {Li, Wei and Chen, Mengxue and Cai, Jinlong and Spooner, Emma L.K. and Zhang, Huijun and Gurney, Robert S. and Liu, Dan and Xiao, Zuo and Lidzey, David G. and Ding, Liming and Wang, Tao},
    number = {3},
    month = {3},
    pages = {819--833},
    volume = {3},
    publisher = {Cell Press},
    url = {https://linkinghub.elsevier.com/retrieve/pii/S2542435118305725},
    doi = {10.1016/j.joule.2018.11.023},
    issn = {25424351},
    keywords = {molecular order, morphology, non-fullerene, organic photovoltaics, polymer solar cells, power-conversion efficiency}
}

@article{Zhang2013MolecularCopolymer,
    title = {{Molecular origin of high field-effect mobility in an indacenodithiophene- benzothiadiazole copolymer}},
    year = {2013},
    journal = {Nature Communications},
    author = {Zhang, Xinran and Bronstein, Hugo and Kronemeijer, Auke J. and Smith, Jeremy and Kim, Youngju and Kline, R. Joseph and Richter, Lee J. and Anthopoulos, Thomas D. and Sirringhaus, Henning and Song, Kigook and Heeney, Martin and Zhang, Weimin and McCulloch, Iain and Delongchamp, Dean M.},
    pages = {1--9},
    volume = {4},
    publisher = {Nature Publishing Group},
    url = {http://dx.doi.org/10.1038/ncomms3238},
    doi = {10.1038/ncomms3238},
    issn = {20411723}
}

@article{Bredas2009MolecularChallenges,
    title = {{Molecular Understanding of Organic Solar Cells: The Challenges}},
    year = {2009},
    author = {Br{\'{e}}das, Jean-Luc and Br{\'{e}}das, Br´ and Norton, Joseph E and Cornil, Jérôme and Coropceanu, Veaceslav},
    url = {https://pubs.acs.org/sharingguidelines},
    doi = {10.1021/ar900099h}
}

@article{Ohm1998MorphologicalFilms,
    title = {{Morphological properties of airbrush spray-deposited enzymatic cellulose thin films}},
    year = {1998},
    journal = {J. Coat. Technol. Res},
    author = {Ohm, Wiebke and Rothkirch, André and Pandit, Pallavi and K{\"{o}}, Volker and M{\"{u}} Ller-Buschbaum, Peter and Rojas, Ramiro and Yu, Shun and Brett, Calvin J and S{\"{o}}, Daniel L and Roth, Stephan V and Roth, Stephan V and K{\"{o}}, Volker and M{\"{u}} Ller-Buschbaum, Peter and Rojas, Ramiro and Yu, Shun and Brett, Calvin J and S{\"{o}}, Daniel L},
    number = {4},
    pages = {759--769},
    volume = {15},
    url = {https://doi.org/10.1007/s11998-018-0089-9},
    doi = {10.1007/s11998-018-0089-9},
    keywords = {Cellulose, Grazing incidence X-ray scattering, Spray coating, Thin films}
}

@article{Ro2016Morphology,
    title = {{Morphology changes upon scaling a high-efficiency, solution-processed solar cell †}},
    year = {2016},
    author = {Ro, Hyun Wook and Downing, Jonathan M and Engmann, Sebastian and Herzing, Andrew A and Delongchamp, Dean M and Richter, Lee J and Mukherjee, Subhrangsu and Ade, Harald and Abdelsamie, Maged and Jagadamma, Lethy K and Amassian, Aram and Liu, Yuhang and Yan, He},
    url = {www.rsc.org/ees},
    doi = {10.1039/c6ee01623e}
}

@misc{Zhao2018MorphologyCells,
    title = {{Morphology Control in Organic Solar Cells}},
    year = {2018},
    booktitle = {Advanced Energy Materials},
    author = {Zhao, Fuwen and Wang, Chunru and Zhan, Xiaowei},
    number = {28},
    month = {10},
    pages = {1703147},
    volume = {8},
    publisher = {Wiley-VCH Verlag},
    url = {http://doi.wiley.com/10.1002/aenm.201703147},
    doi = {10.1002/aenm.201703147},
    keywords = {morphology characterization, morphology control, organic solar cells}
}

@article{Richter2017MorphologyViewpoint,
    title = {{Morphology Development in Solution-Processed Functional Organic Blend Films: An in Situ Viewpoint}},
    year = {2017},
    journal = {Chemical Reviews},
    author = {Richter, Lee J. and Delongchamp, Dean M. and Amassian, Aram},
    number = {9},
    pages = {6332--6366},
    volume = {117},
    doi = {10.1021/acs.chemrev.6b00618},
    issn = {15206890}
}

@article{Freychet2020MorphologyScattering,
    title = {{Morphology of poly(lactide)-block-poly(dimethylsiloxane)-block-polylactide high-{$\chi$} triblock copolymer film studied by grazing incidence small-angle X-ray scattering}},
    year = {2020},
    author = {Freychet, Guillaume and Maret, Mireille and Fernandez-Regulez, Marta and Tiron, Raluca and Gharbi, | Ahmed and Nicolet, Celia and Gergaud, Patrice},
    doi = {10.1002/pol.20200196}
}

@article{Ruderer2011MorphologyPhotovoltaics,
    title = {{Morphology of polymer-based bulk heterojunction films for organic photovoltaics}},
    year = {2011},
    journal = {Soft Matter},
    author = {Ruderer, Matthias A. and M{\"{u}}ller-Buschbaum, Peter},
    number = {12},
    pages = {5482--5493},
    volume = {7},
    doi = {10.1039/c0sm01502d},
    issn = {1744683X}
}

@article{Hoppe2006MorphologyCells,
    title = {{Morphology of polymer/fullerene bulk heterojunction solar cells}},
    year = {2006},
    journal = {Journal of Materials Chemistry},
    author = {Hoppe, Harald and Sariciftci, Niyazi Serdar},
    number = {1},
    pages = {45--61},
    volume = {16},
    doi = {10.1039/b510618b},
    issn = {09599428}
}

@article{Li2019MorphologyStability,
    title = {{Morphology optimization via molecular weight tuning of donor polymer enables all-polymer solar cells with simultaneously improved performance and stability}},
    year = {2019},
    journal = {Nano Energy},
    author = {Li, Zhenye and Zhong, Wenkai and Ying, Lei and Liu, Feng and Li, Ning and Huang, Fei and Cao, Yong},
    month = {10},
    pages = {103931},
    volume = {64},
    publisher = {Elsevier BV},
    doi = {10.1016/j.nanoen.2019.103931},
    issn = {22112855}
}

@article{Haase2017MultifunctionalSeparation,
    title = {{Multifunctional nanocomposite hollow fiber membranes by solvent transfer induced phase separation}},
    year = {2017},
    journal = {Nature Communications},
    author = {Haase, Martin F. and Jeon, Harim and Hough, Noah and Kim, Jong Hak and Stebe, Kathleen J. and Lee, Daeyeon},
    number = {1},
    volume = {8},
    publisher = {Springer US},
    url = {www.nature.com/naturecommunications http://dx.doi.org/10.1038/s41467-017-01409-3},
    doi = {10.1038/s41467-017-01409-3},
    issn = {20411723}
}

@article{Tlf2019NadjaNielsen,
    title = {{Nadja Curdt og Camilla Munch Nielsen}},
    year = {2019},
    author = {Tlf, Slangerup and Reg, Handelsbanken and Iban, Handdkkk},
    pages = {8--10}
}

@article{Liu2019NanomorphologyCells,
    title = {{Nanomorphology in A–D–A type small molecular acceptors-based bulk heterojunction polymer solar cells}},
    year = {2019},
    journal = {Journal of Energy Chemistry},
    author = {Liu, Delong and Zhang, Ying and Li, Gang},
    pages = {104--123},
    volume = {35},
    publisher = {Elsevier B.V. and Science Press},
    url = {https://doi.org/10.1016/j.jechem.2018.11.001},
    doi = {10.1016/j.jechem.2018.11.001},
    issn = {20954956},
    keywords = {A–D–A type small molecules, Bulk heterojunction, Nanomorphology, Non-fullerene acceptor, Polymer solar cells}
}

@techreport{GuoNanostructuresPhotovoltaics,
    title = {{Nanostructures for polymer-based organic photovoltaics}},
    author = {Guo, Shuai},
    keywords = {()}
}

@article{Anctil2020NetApplications,
    title = {{Net energy and cost benefit of transparent organic solar cells in building-integrated applications}},
    year = {2020},
    journal = {Applied Energy},
    author = {Anctil, Annick and Lee, Eunsang and Lunt, Richard R.},
    month = {3},
    volume = {261},
    publisher = {Elsevier Ltd},
    doi = {10.1016/j.apenergy.2019.114429},
    issn = {03062619},
    keywords = {Building energy simulation, Building integrated photovoltaics (BIPV), Life cycle assessment, Transparent photovoltaics}
}

@article{Cheng2018Next-generationAcceptors,
    title = {{Next-generation organic photovoltaics based on non-fullerene acceptors}},
    year = {2018},
    author = {Cheng, Pei and Li, Gang and Zhan, Xiaowei and Yang, Yang},
    url = {https://doi.org/10.1038/s41566-018-0104-9},
    doi = {10.1038/s41566-018-0104-9}
}

@misc{Schwartzkopf2016NoTitle,
    title = {{No Title}},
    year = {2016},
    booktitle = {Nanomaterials},
    author = {Schwartzkopf, Matthias and Roth, Stephan V.},
    number = {12},
    month = {12},
    pages = {239},
    volume = {6},
    publisher = {MDPI AG},
    url = {http://www.mdpi.com/2079-4991/6/12/239},
    doi = {10.3390/nano6120239},
    keywords = {Grazing incidence X-ray scattering, Growth kinetics, In situ, Nanocomposites, Nanostructure formation, Polymer template, Polymer–metal interfaces, Sputter deposition, X-ray scattering}
}

@article{Pedersen2015NoTitle,
    title = {{No Title}},
    year = {2015},
    journal = {Journal of Materials Chemistry A},
    author = {Pedersen, E. B.L. L and Pedersen, M. C. and Simonsen, S. B. and Brandt, R. G. and Andersen, T. R. and Jiang, W. and Xie, Z. Y. and Krebs, F. C. and Arleth, L. and Andreasen, J. W. and B{\"{o}}ttiger, A. P.L. and Andersen, T. R. and Jiang, W. and Xie, Z. Y. and Krebs, F. C. and Arleth, L. and Andreasen, J. W.},
    number = {33},
    month = {7},
    pages = {17022--17031},
    volume = {3},
    publisher = {Royal Society of Chemistry},
    url = {www.rsc.org/MaterialsA},
    doi = {10.1039/c5ta04980f},
    issn = {20507496}
}

@article{Pascual-San-Jose2019NoTitle,
    title = {{No Title}},
    year = {2019},
    journal = {Journal of Materials Chemistry A},
    author = {Pascual-San-Jos{\'{e}}, Enrique and Rodr{\'{i}}guez-Mart{\'{i}}nez, Xabier and Adel-Abdelaleim, Rana and Stella, Marco and Mart{\'{i}}nez-Ferrero, Eugenia and Campoy-Quiles, Mariano and Jos{\'{e}}, Jos´ and Rodr{\'{i}}guezrodr{\'{i}}guez-Mart{\'{i}}nezmart{\'{i}}nez, Xabier and Adel-Abdelaleim, Rana and Stella, Marco and Mart{\'{i}}nezmart{\'{i}}nez-Ferrero, Eugenia and Campoy-Quiles, Mariano},
    number = {35},
    pages = {20369--20382},
    volume = {7},
    publisher = {Royal Society of Chemistry (RSC)},
    url = {http://xlink.rsc.org/?DOI=C9TA07361B},
    issn = {2050-7488}
}

@article{Rossander2017NoTitle,
    title = {{No Title}},
    year = {2017},
    author = {Rossander, Lea Hildebrandt and Dam, Henrik Friis and Carl{\'{e}}, Jon Eggert and Helgesen, Martin and Rajkovic, Ivan and Corazza, Michael and Krebs, Frederik Christian and Andreasen, Jens Wenzel},
    volume = {10},
    issn = {1754-5692}
}

@misc{Kroon2016NoTitle,
    title = {{No Title}},
    year = {2016},
    author = {Kroon, Renee and Mengistie, Desalegn Alemu and Kiefer, David and Hynynen, Jonna and Ryan, Jason D. and Yu, Liyang and M{\"{u}}ller, Christian},
    number = {22},
    month = {11},
    pages = {6147--6164},
    volume = {45},
    publisher = {Royal Society of Chemistry},
    url = {http://www.ncbi.nlm.nih.gov/pubmed/27385496 http://www.pubmedcentral.nih.gov/articlerender.fcgi?artid=PMC5123640},
    doi = {10.1039/c6cs00149a},
    pmid = {27385496}
}

@misc{Lin2014Non-fullereneHorizon,
    title = {{Non-fullerene acceptors for organic photovoltaics: An emerging horizon}},
    year = {2014},
    booktitle = {Materials Horizons},
    author = {Lin, Yuze and Zhan, Xiaowei},
    number = {5},
    month = {9},
    pages = {470--488},
    volume = {1},
    publisher = {Royal Society of Chemistry},
    doi = {10.1039/c4mh00042k},
    issn = {20516355}
}

@article{Yan2018Non-fullereneProject,
    title = {{Non-fullerene acceptors for organic solar cells High Energy Density Nanocomposites Based on Surface-Modified BaTiO3 and a Ferroelectric Polymer View project Organic Solar Cells View project}},
    year = {2018},
    journal = {Nature Publishing Group},
    author = {Yan, Cenqi and Barlow, Stephen and Jen, Alex K-Y and Marder, Seth},
    pages = {1--19},
    volume = {3},
    publisher = {Macmillan Publishers Limited},
    url = {https://www.researchgate.net/publication/323149045},
    doi = {10.1038/natrevmats.2018.3}
}

@article{Zhang2018NonfullereneCells,
    title = {{Nonfullerene Acceptor Molecules for Bulk Heterojunction Organic Solar Cells}},
    year = {2018},
    journal = {Chemical Reviews},
    author = {Zhang, Guangye and Zhao, Jingbo and Chow, Philip C. Y. and Jiang, Kui and Zhang, Jianquan and Zhu, Zonglong and Zhang, Jie and Huang, Fei and Yan, He},
    number = {7},
    month = {4},
    pages = {3447--3507},
    volume = {118},
    url = {https://pubs.acs.org/doi/10.1021/acs.chemrev.7b00535},
    doi = {10.1021/acs.chemrev.7b00535},
    issn = {0009-2665}
}

@article{Proller2017Note:Films,
    title = {{Note: Setup for chemical atmospheric control during in situ grazing incidence X-ray scattering of printed thin films}},
    year = {2017},
    journal = {Review of Scientific Instruments},
    author = {Pr{\"{o}}ller, Stephan and Mosegu{\'{i}} Gonz{\'{a}}lez, Daniel and Zhu, Chenhuii and Schaible, Eric and Wang, Cheng and M{\"{u}}ller-Buschbaum, Peter and Hexemer, Alexander and Herzig, Eva M.},
    number = {6},
    volume = {88},
    url = {http://dx.doi.org/10.1063/1.4984130},
    doi = {10.1063/1.4984130},
    issn = {10897623}
}

@article{Jao2014NovelElectrospinning,
    title = {{Novel elastic nanofibers of syndiotactic polypropylene obtained from electrospinning}},
    year = {2014},
    journal = {European Polymer Journal},
    author = {Jao, Cheng Shin and Wang, Yu and Wang, Chi},
    number = {1},
    pages = {181--189},
    volume = {54},
    publisher = {Elsevier Ltd},
    url = {http://dx.doi.org/10.1016/j.eurpolymj.2014.03.006},
    doi = {10.1016/j.eurpolymj.2014.03.006},
    issn = {00143057},
    keywords = {Aligned nanofibers, High-temperature electrospinning, Mesophase, Microstructure, Syndiotactic polypropylene, Tensile hysteresis}
}

@article{Liu2012OnPhotovoltaics,
    title = {{On the Morphology of Polymer-Based Photovoltaics}},
    year = {2012},
    journal = {J Polym Sci Part B: Polym Phys},
    author = {Liu, Feng and Gu, Yu and Jung, Jae Woong and Jo, Won Ho and Russell, Thomas P.},
    number = {15},
    month = {8},
    pages = {1018--1044},
    volume = {50},
    publisher = {Wiley Periodicals, Inc},
    doi = {10.1002/polb.23063},
    issn = {08876266},
    keywords = {X-ray scattering, conjugated polymers, diffusion, miscibility, morphol-ogy, morphology, neutron scattering, organic photovoltaics, phase separation}
}

@article{Elumalai2016OpenReview,
    title = {{Open circuit voltage of organic solar cells: An in-depth review}},
    year = {2016},
    journal = {Energy and Environmental Science},
    author = {Elumalai, Naveen Kumar and Uddin, Ashraf},
    number = {2},
    pages = {391--410},
    volume = {9},
    publisher = {Royal Society of Chemistry},
    doi = {10.1039/c5ee02871j},
    issn = {17545706}
}

@article{Wang2018OpticalLosses,
    title = {{Optical Gaps of Organic Solar Cells as a Reference for Comparing Voltage Losses}},
    year = {2018},
    journal = {Advanced Energy Materials},
    author = {Wang, Yuming and Qian, Deping and Cui, Yong and Zhang, Huotian and Hou, Jianhui and Vandewal, Koen and Kirchartz, Thomas and Gao, Feng},
    number = {28},
    month = {10},
    pages = {1801352},
    volume = {8},
    publisher = {John Wiley {\&} Sons, Ltd},
    doi = {10.1002/aenm.201801352},
    issn = {1614-6832}
}

@article{Wang2016OpticalInvestigations,
    title = {{Optical properties of regioregular poly(3-hexylthiophene) aggregates from fully atomistic investigations}},
    year = {2016},
    journal = {CrystEngComm},
    author = {Wang, Linjun and Beljonne, David},
    number = {38},
    pages = {7297--7304},
    volume = {18},
    publisher = {Royal Society of Chemistry},
    doi = {10.1039/c6ce00645k},
    issn = {14668033}
}

@article{Hou2018OrganicAcceptors,
    title = {{Organic solar cells based on non-fullerene acceptors}},
    year = {2018},
    journal = {Nature Materials},
    author = {Hou, Jianhui and Inganas, Olle and Friend, Richard H. and Gao, Feng and Ingan{\"{a}}s, Olle and Friend, Richard H. and Gao, Feng},
    number = {2},
    pages = {119--128},
    volume = {17},
    publisher = {Nature Publishing Group},
    url = {www.nature.com/naturematerials http://dx.doi.org/10.1038/nmat5063},
    doi = {10.1038/NMAT5063},
    issn = {14764660}
}

@article{Chen2017OrganicCopolymers,
    title = {{Organic Solar Cells with Controlled Nanostructures Based on Microphase Separation of Fullerene-Attached Thiophene-Selenophene Heteroblock Copolymers}},
    year = {2017},
    journal = {ACS Applied Materials and Interfaces},
    author = {Chen, Peihong and Nakano, Kyohei and Suzuki, Kaori and Hashimoto, Kazuhito and Kikitsu, Tomoka and Hashizume, Daisuke and Koganezawa, Tomoyuki and Tajima, Keisuke},
    number = {5},
    month = {2},
    pages = {4758--4768},
    volume = {9},
    publisher = {American Chemical Society},
    doi = {10.1021/acsami.6b14629},
    issn = {19448252},
    keywords = {block copolymers, energy cascade, microphase separation, organic solar cells, self-organization, semiconducting polymers, thin films}
}

@article{Verploegen2010OrganicMorphology,
    title = {{Organic Solar Cells: How X-ray Scattering Has Improved Our Understanding of Morphology}},
    year = {2010},
    journal = {Synchrotron Radiation News},
    author = {Verploegen, Eric and Miller, Chad E. and Toney, Michael F.},
    number = {4},
    month = {8},
    pages = {16--21},
    volume = {23},
    publisher = { Taylor {\&} Francis Group },
    url = {http://www.tandfonline.com/doi/abs/10.1080/08940886.2010.501491},
    doi = {10.1080/08940886.2010.501491},
    issn = {0894-0886}
}

@article{Yano2012OrientationStretching,
    title = {{Orientation of poly(vinyl alcohol) nanofiber and crystallites in non-woven electrospun nanofiber mats under uniaxial stretching}},
    year = {2012},
    journal = {Polymer},
    author = {Yano, Takahiro and Higaki, Yuji and Tao, Di and Murakami, Daiki and Kobayashi, Motoyasu and Ohta, Noboru and Koike, Jun Ichiro and Horigome, Misao and Masunaga, Hiroyasu and Ogawa, Hiroki and Ikemoto, Yuka and Moriwaki, Taro and Takahara, Atsushi},
    number = {21},
    pages = {4702--4708},
    volume = {53},
    publisher = {Elsevier Ltd},
    url = {http://dx.doi.org/10.1016/j.polymer.2012.07.067},
    doi = {10.1016/j.polymer.2012.07.067},
    issn = {00323861},
    keywords = {Electrospinning, Orientation, Poly(vinyl alcohol)}
}

@article{Teubner1987OriginMicroemulsions,
    title = {{Origin of the scattering peak in microemulsions}},
    year = {1987},
    journal = {The Journal of Chemical Physics},
    author = {Teubner, M. and Strey, R.},
    number = {5},
    pages = {3195--3200},
    volume = {87},
    doi = {10.1063/1.453006},
    issn = {00219606}
}

@article{Cui2019OverVoltages,
    title = {{Over 16{\%} efficiency organic photovoltaic cells enabled by a chlorinated acceptor with increased open-circuit voltages}},
    year = {2019},
    journal = {Nature Communications},
    author = {Cui, Yong and Yao, Huifeng and Zhang, Jianqi and Zhang, Tao and Wang, Yuming and Hong, Ling and Xian, Kaihu and Xu, Bowei and Zhang, Shaoqing and Peng, Jing and Wei, Zhixiang and Gao, Feng and Hou, Jianhui},
    number = {1},
    month = {12},
    pages = {2515},
    volume = {10},
    publisher = {Nature Publishing Group},
    url = {http://www.nature.com/articles/s41467-019-10351-5},
    doi = {10.1038/s41467-019-10351-5},
    issn = {2041-1723}
}

@article{Xie2018OvercomingDefects,
    title = {{Overcoming efficiency and stability limits in water-processing nanoparticular organic photovoltaics by minimizing microstructure defects}},
    year = {2018},
    journal = {Nature Communications},
    author = {Xie, Chen and Heum{\"{u}}ller, Thomas and Gruber, Wolfgang and Tang, Xiaofeng and Classen, Andrej and Schuldes, Isabel and Bidwell, Matthew and Sp{\"{a}}th, Andreas and Fink, Rainer H. and Unruh, Tobias and McCulloch, Iain and Li, Ning and Brabec, Christoph J.},
    number = {1},
    pages = {1--11},
    volume = {9},
    publisher = {Springer US},
    url = {http://dx.doi.org/10.1038/s41467-018-07807-5},
    doi = {10.1038/s41467-018-07807-5},
    issn = {20411723}
}

@article{Carle2017OvercomingCells,
    title = {{Overcoming the Scaling Lag for Polymer Solar Cells}},
    year = {2017},
    journal = {Joule},
    author = {Carl{\'{e}}, Jon E. and Helgesen, Martin and Hagemann, Ole and H{\"{o}}sel, Markus and Heckler, Ilona M. and Bundgaard, Eva and Gevorgyan, Suren A. and S{\o}ndergaard, Roar R. and J{\o}rgensen, Mikkel and Garc{\'{i}}a-Valverde, Rafael and Chaouki-Almagro, Samir and Villarejo, José A. and Krebs, Frederik C.},
    number = {2},
    month = {10},
    pages = {274--289},
    volume = {1},
    url = {https://linkinghub.elsevier.com/retrieve/pii/S2542435117300272},
    doi = {10.1016/j.joule.2017.08.002},
    issn = {25424351},
    keywords = {OPV, high voltage, operation, printed solar cells, scaling, scaling gap, scaling lag, solar foil, solar park, stability}
}

@article{Strohm2018P3HT:Methods,
    title = {{P3HT: Non-fullerene acceptor based large area, semi-transparent PV modules with power conversion efficiencies of 5{\%}, processed by industrially scalable methods}},
    year = {2018},
    journal = {Energy and Environmental Science},
    author = {Strohm, S. and Machui, F. and Langner, S. and Kubis, P. and Gasparini, N. and Salvador, M. and Mcculloch, I. and Egelhaaf, H.-J J. and Brabec, C. J.},
    number = {8},
    pages = {2225--2234},
    volume = {11},
    publisher = {Royal Society of Chemistry},
    url = {http://dx.doi.org/10.1039/C8EE01150H},
    doi = {10.1039/c8ee01150h},
    issn = {17545706}
}

@article{Segre2010ParrattsMethod,
    title = {{Parratt's Recursive Method}},
    year = {2010},
    author = {Segre, C}
}

@article{Perlich2012PatternStudy,
    title = {{Pattern formation of colloidal suspensions by dip-coating: An in situ grazing incidence X-ray scattering study}},
    year = {2012},
    journal = {physica status solidi (RRL) - Rapid Research Letters},
    author = {Perlich, J. and Schwartzkopf, M. and K{\"{o}}rstgens, V. and Erb, D. and Risch, J. F. H. and M{\"{u}}ller-Buschbaum, P. and R{\"{o}}hlsberger, R. and Roth, S. V. and Gehrke, R.},
    number = {6},
    month = {6},
    pages = {253--255},
    volume = {6},
    url = {http://doi.wiley.com/10.1002/pssr.201206114},
    doi = {10.1002/pssr.201206114},
    issn = {18626254},
    keywords = {Colloids, Dip-coating, GISAXS, Nanoparticles, Polymers, X-ray scattering}
}

@article{Gill2015Performance,
    title = {{Performance enhancement of fullerene based solar cells upon NIR laser irradiation †}},
    year = {2015},
    author = {Gill, Hardeep Singh and Thota, Sammaiah and Li, Lian and Kokil, Akshay and Mosurkal, Ravi and Kumar, Jayant},
    url = {www.rsc.org/advances},
    doi = {10.1039/c5ra05640c}
}

@article{Liu2009PhaseFilms,
    title = {{Phase behavior and dimensional scaling of symmetric block copolymer-homopolymer ternary blends in thin films}},
    year = {2009},
    journal = {Macromolecules},
    author = {Liu, Guoliang and Stoykovich, Mark P. and Ji, Shengxiang and Stuen, Karl O. and Craig, Gordon S.W. and Nealey, Paul F.},
    number = {8},
    month = {4},
    pages = {3063--3072},
    volume = {42},
    publisher = { American Chemical Society},
    doi = {10.1021/ma802773h},
    issn = {00249297}
}

@article{Ruderer2012PhaseFilms,
    title = {{Phase separation and molecular intermixing in polymer-fullerene bulk heterojunction thin films}},
    year = {2012},
    journal = {Journal of Physical Chemistry Letters},
    author = {Ruderer, Matthias A. and Meier, Robert and Porcar, Lionel and Cubitt, Robert and M{\"{u}}ller-Buschbaum, Peter},
    number = {6},
    month = {3},
    pages = {683--688},
    volume = {3},
    url = {https://pubs.acs.org/doi/10.1021/jz300039h},
    doi = {10.1021/jz300039h},
    issn = {19487185}
}

@article{Ishiguro2018Phase-fieldAlloys,
    title = {{Phase-field simulation of spinodal decomposition and its effect on stress-induced martensitic transformation in Ti–Nb–O alloys}},
    year = {2018},
    journal = {Computational Materials Science},
    author = {Ishiguro, Yuya and Tsukada, Yuhki and Koyama, Toshiyuki},
    month = {8},
    pages = {222--230},
    volume = {151},
    publisher = {Elsevier B.V.},
    doi = {10.1016/j.commatsci.2018.05.003},
    issn = {09270256},
    keywords = {Phase-field method, Spinodal decomposition, Stress-induced martensitic transformation, Ti-based alloys}
}

@article{Li2012Phase-fieldBlends,
    title = {{Phase-field simulation of thermally induced spinodal decomposition in polymer blends}},
    year = {2012},
    journal = {Modelling and Simulation in Materials Science and Engineering},
    author = {Li, Y. C. and Shi, R. P. and Wang, C. P. and Liu, X. J. and Wang, Y.},
    number = {7},
    volume = {20},
    doi = {10.1088/0965-0393/20/7/075002},
    issn = {09650393}
}

@article{ChenPHYSICALComplexes,
    title = {{PHYSICAL REVIEW LETTERS Structure and Fractal Dimension of Protein-Detergent Complexes}},
    author = {Chen, Sow-Hsin and Teixeira, Jose}
}

@article{Hjlund-Nielsen2015Polarization-dependentNm,
    title = {{Polarization-dependent aluminum metasurface operating at 450 nm}},
    year = {2015},
    journal = {Optics Express},
    author = {H{\o}jlund-Nielsen, Emil and Zhu, Xiaolong and Carstensen, Marcus S. and S{\o}rensen, Michael K. and Vannahme, Christoph and Asger Mortensen, N. and Kristensen, Anders},
    number = {22},
    month = {11},
    pages = {28829},
    volume = {23},
    publisher = {The Optical Society},
    url = {https://www.osapublishing.org/viewmedia.cfm?uri=oe-23-22-28829&seq=0&html=true https://www.osapublishing.org/abstract.cfm?uri=oe-23-22-28829 https://www.osapublishing.org/oe/abstract.cfm?uri=oe-23-22-28829},
    doi = {10.1364/oe.23.028829},
    issn = {1094-4087},
    keywords = {(0506624) Subwavelength structures, (2200220) Optical design and fabrication, (2406680) Surface plasmons, OCIS codes: (1305440) Polarization-selective devices}
}

@article{Zheng2017Poly3-hexylthiopheneCells,
    title = {{Poly(3-hexylthiophene) coated graphene oxide for improved performance of bulk heterojunction polymer solar cells}},
    year = {2017},
    journal = {Organic Electronics: physics, materials, applications},
    author = {Zheng, Fei and Yang, Xiao Yu and Bi, Peng Qing and Niu, Meng Si and Lv, Cheng Kun and Feng, Lin and Qin, Wei and Wang, Yu Zhu and Hao, Xiao Tao and Ghiggino, Kenneth P.},
    number = {February 2018},
    pages = {149--158},
    volume = {44},
    publisher = {Elsevier B.V},
    url = {http://dx.doi.org/10.1016/j.orgel.2017.02.021},
    doi = {10.1016/j.orgel.2017.02.021},
    issn = {15661199},
    keywords = {Coating, Graphene oxide, Organic solar cells, Phase separation, Poly(3-hexylthiophene)}
}

@article{Dennler2009PolymerReview.pdf,
    title = {{Polymer fullerene bulk heterojunction solar cells 3 - review.pdf}},
    year = {2009},
    journal = {Advanced Materials},
    author = {Dennler, G and Scharber, MC and Brabec, CJ},
    url = {http://onlinelibrary.wiley.com/doi/10.1002/adma.200801283/full},
    doi = {10.1088/0034-4885/73/9/096401}
}

@article{Michels2021PredictiveCoating,
    title = {{Predictive modelling of structure formation in semiconductor films produced by meniscus-guided coating}},
    year = {2021},
    journal = {Nature Materials},
    author = {Michels, Jasper J. and Zhang, Ke and Wucher, Philipp and Beaujuge, Pierre M. and Pisula, Wojciech and Marszalek, Tomasz},
    number = {1},
    month = {8},
    pages = {68--75},
    volume = {20},
    publisher = {Nature Research},
    url = {https://doi.org/10.1038/s41563-020-0760-2},
    doi = {10.1038/s41563-020-0760-2},
    issn = {14764660},
    pmid = {32778811},
    keywords = {Condensed, Materials for devices, Soft materials, Theory and computation, matter physics}
}

@article{Onder2018PreparationMorphology,
    title = {{Preparation of monolithic polycaprolactone foams with controlled morphology}},
    year = {2018},
    journal = {Polymer},
    author = {Onder, Ozgun Can and Yilgor, Emel and Yilgor, Iskender},
    number = {December},
    pages = {166--178},
    volume = {136},
    publisher = {Elsevier Ltd},
    url = {https://doi.org/10.1016/j.polymer.2017.12.054},
    doi = {10.1016/j.polymer.2017.12.054},
    issn = {00323861},
    keywords = {Foam, Polycaprolactone, Thermally induced phase separation}
}

@article{Lin2018Printed9.5,
    title = {{Printed Nonfullerene Organic Solar Cells with the Highest Efficiency of 9.5{\%}}},
    year = {2018},
    journal = {Advanced Energy Materials},
    author = {Lin, Yuanbao and Jin, Yingzhi and Dong, Sheng and Zheng, Wenhao and Yang, Junyu and Liu, Alei and Liu, Feng and Jiang, Yufeng and Russell, Thomas P. and Zhang, Fengling and Huang, Fei and Hou, Lintao},
    number = {13},
    month = {5},
    pages = {1701942},
    volume = {8},
    publisher = {Wiley-VCH Verlag},
    url = {http://doi.wiley.com/10.1002/aenm.201701942},
    doi = {10.1002/aenm.201701942},
    issn = {16146832},
    keywords = {doctor-blading nonfullerene organic solar cells, highest efficiency, large-area ITO-free flexible structures, morphology, processing additives}
}

@article{Liu2017PrintingCharacterization,
    title = {{Printing Fabrication of Bulk Heterojunction Solar Cells and In Situ Morphology Characterization}},
    year = {2017},
    journal = {J. Vis. Exp},
    author = {Liu, Feng and Ferdous, Sunzida and Wan, Xianjian and Zhu, Chenhui and Schaible, Eric and Hexemer, Alexander and Wang, Cheng and Russell, Thomas P.},
    number = {119},
    month = {1},
    pages = {53710},
    volume = {2017},
    publisher = {Journal of Visualized Experiments},
    url = {www.jove.comurl:https://www.jove.com/video/53710},
    doi = {10.3791/53710},
    issn = {1940087X},
    keywords = {Conjugated polymer, Engineering, Issue 119, Morphology, Organic photovoltaics, Slot die coating, Thin film device, X-ray diffraction, conjugated polymer, morphology, organic photovoltaics, slot die coating Date, thin film device}
}

@article{Pelse2021ProbingAcceptors,
    title = {{Probing Crystallization Effects when Processing Bulk-Heterojunction Active Layers: Comparing Fullerene and Nonfullerene Acceptors}},
    year = {2021},
    journal = {Chemistry of Materials},
    author = {Pelse, Ian and Jones, Austin L. and Richter, Lee J. and Reynolds, John R.},
    doi = {10.1021/acs.chemmater.0c03971},
    issn = {0897-4756}
}

@article{Renaud2009ProbingScattering,
    title = {{Probing surface and interface morphology with Grazing Incidence Small Angle X-Ray Scattering}},
    year = {2009},
    journal = {Surface Science Reports},
    author = {Renaud, Gilles and Lazzari, Rémi and Leroy, Frédéric},
    number = {8},
    pages = {255--380},
    volume = {64},
    publisher = {Elsevier B.V.},
    url = {https://reader.elsevier.com/reader/sd/pii/S0167572909000399?token=97DDF4F72B4E01A2D29C81AA236603A1E0EBEB8DC9A6DF5F4B6622FF139180320AC4FFAA476F51A775C84CDB6C2C4901 http://dx.doi.org/10.1016/j.surfrep.2009.07.002},
    doi = {10.1016/j.surfrep.2009.07.002},
    issn = {01675729},
    keywords = {Assemblies of nanoparticles, Catalysis, DWBA, Decoupling Approximation, Distorted Wave Born Approximation, Form factor, GISAXS, Grazing Incidence Small Angle X-Ray Scattering, Grazing incidence, Growth laws, Growth modes, In situ, Interference function, Local Monodispersed Approximation, Metal on oxide surfaces, Metal surfaces, Molecular beam epitaxy, Nano-particles, Nano-structures, Patterned substrates, Polymers, Quantum dots, Reconstructions, Scaling Approximation, Self- organized growth, Semi-conductors, Size-Spacing Correlation Approximation, Synchrotron X-rays, Theory of X-ray scattering, Ultra-high-vacuum, X-ray scattering}
}

@article{Wang2017ProbingFilms,
    title = {{Probing the intrinsic charge transport in indacenodithiophene-co-benzothiadiazole thin films}},
    year = {2017},
    journal = {AIP Advances},
    author = {Wang, Wenhe and Tang, Wei and Zhao, Jiaqing and Bao, Bei and Xing, Hui and Guo, Xiaojun and Wang, Shun and Liu, Ying},
    number = {12},
    volume = {7},
    doi = {10.1063/1.5001986},
    issn = {21583226}
}

@article{Zhao2019Processing-FriendlyMorphology,
    title = {{Processing-Friendly Slot-Die-Cast Nonfullerene Organic Solar Cells with Optimized Morphology}},
    year = {2019},
    journal = {ACS Appl. Mater. Interfaces},
    author = {Zhao, Heng and Zhang, Lin and Bilal Naveed, Hafiz and Lin, Baojun and Zhao, Baofeng and Zhou, Ke and Gao, Chao and Zhang, Cankun and Wang, Cheng and Ma, Wei},
    pages = {42392--42402},
    volume = {11},
    url = {www.acsami.org},
    doi = {10.1021/acsami.9b12522},
    keywords = {high efficiency, organic solar cells ■ INTRODUCTION, processing friendly, slot-die coating, thick film}
}

@article{Wadsworth2018ProgressPerformance,
    title = {{Progress in Poly (3-Hexylthiophene) Organic Solar Cells and the Influence of Its Molecular Weight on Device Performance}},
    year = {2018},
    journal = {Advanced Energy Materials},
    author = {Wadsworth, Andrew and Hamid, Zeinab and Bidwell, Matthew and Ashraf, Raja S. and Khan, Jafar I. and Anjum, Dalaver H. and Cendra, Camila and Yan, Jun and Rezasoltani, Elham and Guilbert, Anne A.Y. and Azzouzi, Mohammed and Gasparini, Nicola and Bannock, James H. and Baran, Derya and Wu, Hongbin and de Mello, John C. and Brabec, Christoph J. and Salleo, Alberto and Nelson, Jenny and Laquai, Frédéric and McCulloch, Iain},
    number = {28},
    pages = {1--15},
    volume = {8},
    doi = {10.1002/aenm.201801001},
    issn = {16146840},
    keywords = {IDTBR, molecular weight, nonfullerene, organic photovoltaics, poly (3-hexylthiophene)}
}

@article{Baker2010QuantificationDetector,
    title = {{Quantification of Thin Film Crystallographic Orientation Using X-ray Diffraction with an Area Detector}},
    year = {2010},
    journal = {Langmuir},
    author = {Baker, Jessy L and Jimison, Leslie H and Mannsfeld, Stefan and Volkman, Steven and Yin, Shong and Subramanian, Vivek and Salleo, Alberto and Alivisatos, ) A Paul and Toney, Michael F},
    number = {11},
    pages = {9146--9151},
    volume = {26},
    url = {https://pubs.acs.org/sharingguidelines},
    doi = {10.1021/la904840q}
}

@article{RevenantQuantitativeGrowth,
    title = {{Quantitative analysis of grazing incidence small-angle x-ray scattering: PdÕMgO"001{\ldots} growth}},
    author = {Revenant, C and Leroy, F and Lazzari, R and Renaud, G and Henry, C R},
    doi = {10.1103/PhysRevB.69.035411},
    keywords = {0705Tp, 6110Eq, 6146w, numbers: 6837d}
}

@article{Liao2011QuantitativeCell,
    title = {{Quantitative Nanoorganized Structural Evolution for a High Efficiency Bulk Heterojunction Polymer Solar Cell}},
    year = {2011},
    journal = {J. Am. Chem. Soc},
    author = {Liao, Hsueh-Chung and Tsao, Cheng-Si and Lin, Tsung-Han and Chuang, Chih-Min and Chen, Charn-Ying and Jeng, U-Ser and Su, Chiu-Hun and Chen, Yang-Fang and Su, Wei-Fang},
    volume = {133},
    url = {https://pubs.acs.org/sharingguidelines},
    doi = {10.1021/ja202977r}
}

@article{Ye2018QuantitativeCells,
    title = {{Quantitative relations between interaction parameter, miscibility and function in organic solar cells}},
    year = {2018},
    journal = {Nature Materials},
    author = {Ye, Long and Hu, Huawei and Ghasemi, Masoud and Wang, Tonghui and Collins, Brian A. and Kim, Joo Hyun and Jiang, Kui and Carpenter, Joshua H. and Li, Hong and Li, Zhengke and McAfee, Terry and Zhao, Jingbo and Chen, Xiankai and Lai, Joshua Lin Yuk and Ma, Tingxuan and Bredas, Jean Luc and Yan, He and Ade, Harald},
    number = {3},
    pages = {253--260},
    volume = {17},
    publisher = {Springer US},
    url = {http://dx.doi.org/10.1038/s41563-017-0005-1},
    doi = {10.1038/s41563-017-0005-1},
    issn = {14764660}
}

@article{SanishviliRadiationBeam,
    title = {{Radiation damage in protein crystals is reduced with a micron-sized X-ray beam}},
    author = {Sanishvili, Ruslan and Yoder, Derek W and Pothineni, Sudhir Babu and Rosenbaum, Gerd and Xu, Shenglan and Vogt, Stefan and Stepanov, Sergey and Makarov, Oleg A and Макаров, Олег and Corcoran, Stephen and Benn, Richard and Nagarajan, Venugopalan and Smith, Janet L and Fischetti, Robert F},
    url = {www.pnas.org/lookup/suppl/},
    doi = {10.1073/pnas.1017701108/-/DCSupplemental}
}

@article{Schwartzkopf2021Real-timePolymers,
    title = {{Real-time insight into nanostructure evolution during the rapid formation of ultra-thin gold layers on polymers}},
    year = {2021},
    journal = {Nanoscale Horizons},
    author = {Schwartzkopf, Matthias and W{\"{o}}hnert, Sven-Jannik and Waclawek, Vivian and Carstens, Niko and Rothkirch, André and Rubeck, Jan and Gensch, Marc and Drewes, Jonas and Polonskyi, Oleksandr and Strunskus, Thomas and Hinz, Alexander M. and Schaper, Simon J. and K{\"{o}}rstgens, Volker and M{\"{u}}ller-Buschbaum, Peter and Faupel, Franz and Roth, Stephan V.},
    publisher = {Royal Society of Chemistry (RSC)},
    url = {https://pubs.rsc.org/en/content/articlehtml/2021/nh/d0nh00538j https://pubs.rsc.org/en/content/articlelanding/2021/nh/d0nh00538j},
    doi = {10.1039/d0nh00538j},
    issn = {2055-6756}
}

@article{Kassar2016Real-TimeFilms,
    title = {{Real-Time Investigation of Intercalation and Structure Evolution in Printed Polymer:Fullerene Bulk Heterojunction Thin Films}},
    year = {2016},
    journal = {Advanced Energy Materials},
    author = {Kassar, Thaer and G{\"{u}}ldal, Nusret S. and Berlinghof, Marvin and Ameri, Tayebeh and Kratzer, Andreas and Schroeder, Bob C. and Destri, Giovanni Li and Hirsch, Andreas and Heeney, Martin and McCulloch, Iain and Brabec, Christoph J. and Unruh, Tobias},
    number = {5},
    pages = {1--8},
    volume = {6},
    doi = {10.1002/aenm.201502025},
    issn = {16146840},
    keywords = {fullerenes, grazing incidence diffraction, intercalation dynamics, organic solar cells, thin films}
}

@article{Kowarik2006Real-timeFilms,
    title = {{Real-time observation of structural and orientational transitions during growth of organic thin films}},
    year = {2006},
    journal = {Physical Review Letters},
    author = {Kowarik, S. and Gerlach, A. and Sellner, S. and Schreiber, F. and Cavalcanti, L. and Konovalov, O.},
    number = {12},
    pages = {1--4},
    volume = {96},
    doi = {10.1103/PhysRevLett.96.125504},
    issn = {10797114}
}

@article{Eftaiha2014RecentCells,
    title = {{Recent advances of non-fullerene, small molecular acceptors for solution processed bulk heterojunction solar cells}},
    year = {2014},
    journal = {Journal of Materials Chemistry A},
    author = {Eftaiha, Ala'A F. and Sun, Jon Paul and Hill, Ian G. and Welch, Gregory C.},
    number = {5},
    pages = {1201--1213},
    volume = {2},
    doi = {10.1039/c3ta14236a},
    issn = {20507488}
}

@article{Gaspar2018RecentCells,
    title = {{Recent developments in the optimization of the bulk heterojunction morphology of polymer: Fullerene solar cells}},
    year = {2018},
    journal = {Materials},
    author = {Gaspar, Hugo and Figueira, Flávio and Pereira, Luiz and Mendes, Adélio and Viana, Júlio C. and Bernardo, Gabriel},
    number = {12},
    volume = {11},
    doi = {10.3390/ma11122560},
    issn = {19961944},
    keywords = {Fullerenes, Organic photovoltaics}
}

@article{Wang2020RecentCells,
    title = {{Recent Progress and Challenges toward Highly Stable Nonfullerene Acceptor‐Based Organic Solar Cells}},
    year = {2020},
    journal = {Advanced Energy Materials},
    author = {Wang, Yiwen and Lee, Jinho and Hou, Xueyan and Labanti, Chiara and Yan, Jun and Mazzolini, Eva and Parhar, Amber and Nelson, Jenny and Kim, Ji‐Seon and Li, Zhe},
    month = {12},
    pages = {2003002},
    publisher = {Wiley-VCH Verlag},
    url = {https://onlinelibrary.wiley.com/doi/10.1002/aenm.202003002},
    doi = {10.1002/aenm.202003002},
    issn = {1614-6832},
    keywords = {ISOS standards, device engineering, molecular design, nonfullerene solar cells, organic photovoltaics, stability}
}

@article{Chen2017RecentOSCs,
    title = {{Recent progress in non-fullerene small molecule acceptors in organic solar cells (OSCs)}},
    year = {2017},
    journal = {Journal of Materials Chemistry C},
    author = {Chen, Wangqiao and Zhang, Qichun},
    number = {6},
    pages = {1275--1302},
    volume = {5},
    publisher = {Royal Society of Chemistry},
    url = {http://dx.doi.org/10.1039/C6TC05066B},
    doi = {10.1039/c6tc05066b},
    issn = {20507526}
}

@article{Sun2019RecentPhotovoltaics,
    title = {{Recent progress on non-fullerene acceptors for organic photovoltaics}},
    year = {2019},
    journal = {Materials Today},
    author = {Sun, Hua and Chen, Fei and Chen, Zhi Kuan},
    number = {xx},
    pages = {94--118},
    volume = {24},
    url = {https://doi.org/10.1016/j.mattod.2018.09.004},
    doi = {10.1016/j.mattod.2018.09.004},
    issn = {18734103}
}

@article{Baran2016ReducedVoltages,
    title = {{Reduced voltage losses yield 10{\%} efficient fullerene free organic solar cells with >1 V open circuit voltages}},
    year = {2016},
    journal = {Energy and Environmental Science},
    author = {Baran, D. and Kirchartz, T. and Wheeler, S. and Dimitrov, S. and Abdelsamie, M. and Gorman, J. and Ashraf, R. S. and Holliday, S. and Wadsworth, A. and Gasparini, N. and Kaienburg, P. and Yan, H. and Amassian, A. and Brabec, C. J. and Durrant, J. R. and McCulloch, I.},
    number = {12},
    pages = {3783--3793},
    volume = {9},
    publisher = {Royal Society of Chemistry},
    doi = {10.1039/c6ee02598f},
    issn = {17545706}
}

@article{OkudaRelatedEdge,
    title = {{Related content Anomalous Grazing Incidence Small-Angle Scattering of Capped Ge Nanodots at the Si K Absorption Edge}},
    journal = {Journal of Physics: Conference Series OPEN ACCESS},
    author = {Okuda, Hiroshi and Kato, Masayuki and Ochiai, Shojiro},
    doi = {10.1088/1742-6596/184/1/012005}
}

@article{Vaudin2017RelatedSpectrum,
    title = {{Related content Precise silicon die curvature measurements using the NIST lattice comparator High-precision measurement of the x-ray Cu K{$\alpha$} spectrum}},
    year = {2017},
    journal = {Journal of Physics B: Atomic, Molecular and Optical Physics},
    author = {Vaudin, M D and Kessler, E G and Owen, D M and Mendenhall, Marcus H and Henins, Albert and Hudson, Lawrence T and Szabo, Csilla I and Windover, Donald and Cline, James P},
    url = {https://doi.org/10.1088/1361-6455/aa6c4a},
    doi = {10.1088/1361-6455/aa6c4a},
    keywords = {copper, wavelength standard, x-ray diffraction, x-ray spectroscopy}
}

@article{Freychet2016RemovalScattering,
    title = {{Removal of poly(methyl methacrylate) in diblock copolymers films studied by grazing incidence small-angle X-ray scattering}},
    year = {2016},
    journal = {Journal of Polymer Science, Part B: Polymer Physics},
    author = {Freychet, Guillaume and Maret, Mireille and Tiron, Raluca and Chevalier, Xavier and Gharbi, Ahmed and Fernandez-Regulez, Marta and Gergaud, Patrice},
    number = {12},
    pages = {1137--1144},
    volume = {54},
    doi = {10.1002/polb.24017},
    issn = {10990488},
    keywords = {GISAXS, copolymers, scanning electron microscopy, self-assembly, thin films, x-ray reflectivity}
}

@article{Hammouda2010ResearchPapers,
    title = {{research papers A new Guinier – Porod model research papers}},
    year = {2010},
    author = {Hammouda, Boualem},
    pages = {716--719},
    doi = {10.1107/S0021889810015773}
}

@article{Fevola2020ResonantCells,
    title = {{Resonant x-ray ptychographic nanotomography of kesterite solar cells}},
    year = {2020},
    journal = {Physical Review Research},
    author = {Fevola, Giovanni and J{\o}rgensen, Peter S and Verezhak, Mariana and Slyamov, Azat and Crovetto, Andrea and Balogh, Zoltan I and Rein, Christian and Canulescu, Stela and Andreasen, Jens W},
    pages = {1--12},
    volume = {013378},
    publisher = {American Physical Society},
    doi = {10.1103/PhysRevResearch.2.013378},
    keywords = {doi:10.1103/PhysRevResearch.2.013378 url:https://d}
}

@article{MagedAbdelsamie2022RevealingScattering,
    title = {{Revealing temperature-dependent polymer aggregation in solution with small-angle X-ray scattering}},
    year = {2022},
    journal = {Journal of Materials Chemistry A},
    author = {{Maged Abdelsamie} and P. Chaney, Thomas and {Hongping Yan} and A. Schneider, Sebastian and Alperen Ayhan, I. and D. Gomez, Enrique and R. Reynolds, John and F. Toney, Michael},
    publisher = {Royal Society of Chemistry},
    url = {https://pubs.rsc.org/en/content/articlehtml/2022/ta/d1ta09086k https://pubs.rsc.org/en/content/articlelanding/2022/ta/d1ta09086k},
    doi = {10.1039/D1TA09086K},
    issn = {2050-7488}
}

@article{Boldon2015ReviewApplication,
    title = {{Review of the fundamental theories behind small angle X-ray scattering, molecular dynamics simulations, and relevant integrated application}},
    year = {2015},
    journal = {Nano Reviews},
    author = {Boldon, Lauren and Laliberte, Fallon and Liu, Li},
    number = {1},
    pages = {25661},
    volume = {6},
    doi = {10.3402/nano.v6.25661},
    keywords = {ab initio, atomistic simulation, md-saxs, molecular dynamics, nanoparticles, newtonian, pair distribution function, protein folding, radius of gyration, small angle x-ray scattering}
}

@misc{Peng2013ReviewSystems,
    title = {{Review on life cycle assessment of energy payback and greenhouse gas emission of solar photovoltaic systems}},
    year = {2013},
    booktitle = {Renewable and Sustainable Energy Reviews},
    author = {Peng, Jinqing and Lu, Lin and Yang, Hongxing},
    pages = {255--274},
    volume = {19},
    publisher = {Elsevier Ltd},
    doi = {10.1016/j.rser.2012.11.035},
    issn = {13640321},
    keywords = {Energy payback time, Energy requirement, GHG emission rate, Life cycle assessment, Photovoltaic system}
}

@article{PolmanREVIEWChallenges,
    title = {{REVIEW SUMMARY Photovoltaic materials: Present efficiencies and future challenges}},
    author = {Polman, Albert and Knight, Mark and Garnett, Erik C and Ehrler, Bruno and Sinke, Wim C},
    url = {http://science.sciencemag.org/},
    doi = {10.1126/science.aad4424}
}

@article{Farouil2018RevisitingStudy,
    title = {{Revisiting the Vibrational and Optical Properties of P3HT: A Combined Experimental and Theoretical Study}},
    year = {2018},
    journal = {J. Phys. Chem. A},
    author = {Farouil, Leá and Alary, Fabienne and Eléna Bedel-Pereira, Eléna and Heully, Jean-Louis},
    pages = {46},
    volume = {122},
    publisher = {UTC},
    url = {https://pubs.acs.org/sharingguidelines},
    doi = {10.1021/acs.jpca.8b03814}
}

@article{Baran2015RoleCells,
    title = {{Role of Polymer Fractionation in Energetic Losses and Charge Carrier Lifetimes of Polymer: Fullerene Solar Cells}},
    year = {2015},
    journal = {Journal of Physical Chemistry C},
    author = {Baran, Derya and Vezie, Michelle S. and Gasparini, Nicola and Deledalle, Florent and Yao, Jizhong and Schroeder, Bob C. and Bronstein, Hugo and Ameri, Tayebeh and Kirchartz, Thomas and McCulloch, Iain and Nelson, Jenny and Brabec, Christoph J.},
    number = {34},
    pages = {19668--19673},
    volume = {119},
    doi = {10.1021/acs.jpcc.5b05709},
    issn = {19327455}
}

@article{Cheng2015Roll-CoatedStability,
    title = {{Roll-Coated Fabrication of Fullerene-Free Organic Solar Cells with Improved Stability}},
    year = {2015},
    journal = {Advanced Science},
    author = {Cheng, Pei and Bai, Huitao and Zawacka, Natalia K. and Andersen, Thomas R. and Liu, Wenqing and Bundgaard, Eva and J{\o}rgensen, Mikkel and Chen, Hongzheng and Krebs, Frederik C. and Zhan, Xiaowei},
    number = {6},
    month = {6},
    pages = {1500096},
    volume = {2},
    url = {http://doi.wiley.com/10.1002/advs.201500096},
    doi = {10.1002/advs.201500096},
    issn = {21983844}
}

@article{Liu2016Roll-coating,
    title = {{Roll-coating fabrication of flexible organic solar cells: comparison of fullerene and fullerene-free systems †}},
    year = {2016},
    author = {Liu, Kuan and Thue, Ab and Larsen-Olsen, Trofod and Lin, Yuze and Beliatis, Michail and Bundgaard, Eva and J{\o}rgensen, Mikkel and Krebs, Frederik C and Zhan, Xiaowei},
    url = {www.rsc.org/MaterialsA},
    doi = {10.1039/c5ta07357j}
}

@article{Sndergaard2012Roll-to-rollCells,
    title = {{Roll-to-roll fabrication of polymer solar cells}},
    year = {2012},
    journal = {Materials Today},
    author = {S{\o}ndergaard, Roar and H{\"{o}}sel, Markus and Angmo, Dechan and Larsen-Olsen, Thue T. and Krebs, Frederik C.},
    number = {1-2},
    month = {1},
    pages = {36--49},
    volume = {15},
    publisher = {Elsevier Ltd},
    url = {http://dx.doi.org/10.1016/S1369-7021(12)70019-6},
    doi = {10.1016/S1369-7021(12)70019-6},
    issn = {13697021}
}

@article{Gu2017Roll-to-RollBlend,
    title = {{Roll-to-Roll Printed Large-Area All-Polymer Solar Cells with 5{\%} Efficiency Based on a Low Crystallinity Conjugated Polymer Blend}},
    year = {2017},
    journal = {Advanced Energy Materials},
    author = {Gu, Xiaodan and Zhou, Yan and Gu, Kevin and Kurosawa, Tadanori and Guo, Yikun and Li, Yunke and Lin, Haoran and Schroeder, Bob C. and Yan, He Hongping and Molina-Lopez, Francisco and Tassone, Christopher J. and Wang, Cheng and Mannsfeld, Stefan C. B. and Yan, He Hongping and Zhao, Dahui and Toney, Michael F. and Bao, Zhenan},
    number = {14},
    month = {7},
    pages = {1602742},
    volume = {7},
    url = {http://doi.wiley.com/10.1002/aenm.201602742},
    doi = {10.1002/aenm.201602742},
    issn = {16146832},
    keywords = {X-ray diffraction, all-polymer solar cells, in situ X-ray scattering, organic solar cells, roll-to-roll processing}
}

@article{Weller2019Roll-to-RollCopolymers,
    title = {{Roll-to-Roll Scalable Production of Ordered Microdomains through Nonvolatile Additive Solvent Annealing of Block Copolymers}},
    year = {2019},
    author = {Weller, Daniel W and Galuska, Luke and Wang, Weiyu and Ehlenburg, Dakota and Hong, Kunlun and Gu, Xiaodan},
    url = {https://pubs.acs.org/sharingguidelines},
    doi = {10.1021/acs.macromol.9b00772}
}

@article{Yang2018Roll-to-RollSelf-Assembly,
    title = {{Roll-to-Roll Slot-Die-Printed Polymer Solar Cells by Self-Assembly}},
    year = {2018},
    author = {Yang, Junyu and Lin, Yuanbao and Zheng, Wenhao and Liu, Alei and Cai, Wanzhu and Yu, Xiaomin and Zhang, Fengling and Liang, Quanbin and Wu, Hongbin and Qin, Donghuan and Hou, Lintao},
    url = {www.acsami.org},
    doi = {10.1021/acsami.8b05673},
    keywords = {ITO-free, flexible, one-step slot-die, polymer solar cell, self-assembly}
}

@article{Ingham2011SAXSMorph:Data,
    title = {{SAXSMorph: A program for generating representative morphologies for two-phase materials from small-angle X-ray and neutron scattering data}},
    year = {2011},
    journal = {Journal of Applied Crystallography},
    author = {Ingham, Bridget and Li, Haiyong and Allen, Emily L. and Toney, Michael F.},
    number = {1},
    pages = {221--224},
    volume = {44},
    doi = {10.1107/S0021889810048557},
    issn = {00218898},
    keywords = {SAXSMorph, computer programs, small-angle X-ray scattering, small-angle neutron scattering}
}

@article{Andersen2014ScalableModules,
    title = {{Scalable, ambient atmosphere roll-to-roll manufacture of encapsulated large area, flexible organic tandem solar cell modules}},
    year = {2014},
    journal = {Energy and Environmental Science},
    author = {Andersen, Thomas R. and Dam, Henrik F. and H{\"{o}}sel, Markus and Helgesen, Martin and Carl{\'{e}}, Jon E. and Larsen-Olsen, Thue T. and Gevorgyan, Suren A. and Andreasen, Jens W. and Adams, Jens and Li, Ning and Machui, Florian and Spyropoulos, George D. and Ameri, Tayebeh and Lema{\^{i}}tre, Noëlla and Legros, Mathilde and Scheel, Arnulf and Gaiser, Detlef and Kreul, Kilian and Berny, Stephane and Lozman, Owen R. and Nordman, Sirpa and V{\"{a}}lim{\"{a}}ki, Marja and Vilkman, Marja and S{\o}ndergaard, Roar R. and J{\o}rgensen, Mikkel and Brabec, Christoph J. and Krebs, Frederik C.},
    number = {9},
    pages = {2925--2933},
    volume = {7},
    doi = {10.1039/c4ee01223b},
    issn = {17545706}
}

@article{Debye1949ScatteringSolid,
    title = {{Scattering by an inhomogeneous solid}},
    year = {1949},
    journal = {Journal of Applied Physics},
    author = {Debye, P. and Bueche, A. M.},
    number = {6},
    pages = {518--525},
    volume = {20},
    doi = {10.1063/1.1698419},
    issn = {00218979}
}

@article{Chae2016SelectiveLaser,
    title = {{Selective Chain Alignment of Conducting Polymer Blend Films by an Ultrafast Laser}},
    year = {2016},
    journal = {Macromolecular Chemistry and Physics},
    author = {Chae, Sangmin and Jo, Kuk Hyun and Lee, Si Woo and Keum, Hee-Sung and Kim, Hyo Jung and Choi, Jiyeon and Lee, Hyun Hwi},
    number = {4},
    month = {2},
    pages = {537--542},
    volume = {217},
    url = {http://doi.wiley.com/10.1002/macp.201500354},
    doi = {10.1002/macp.201500354},
    issn = {10221352}
}

@article{Peak2006SeleniteStudy,
    title = {{Selenite Adsorption Mechanisms on Pure and Coated Montmorillonite: An EXAFS and XANES Spectroscopic Study}},
    year = {2006},
    journal = {Soil Science Society of America Journal},
    author = {Peak, Derek and Saha, U. K. and Huang, P. M.},
    number = {1},
    month = {1},
    pages = {192--203},
    volume = {70},
    publisher = {Wiley},
    doi = {10.2136/sssaj2005.0054},
    issn = {0361-5995}
}

@article{Gao2012Selenophene-thiopheneNanostructures,
    title = {{Selenophene-thiophene block copolymer solar cells with thermostable nanostructures}},
    year = {2012},
    journal = {ACS Nano},
    author = {Gao, Dong and Hollinger, Jon and Seferos, Dwight S.},
    number = {8},
    month = {8},
    pages = {7114--7121},
    volume = {6},
    doi = {10.1021/nn3021844},
    issn = {19360851},
    keywords = {conjugated polymer, nanofiber, nanostructure, solar cell, thermal stability}
}

@misc{Carrera2015SemiconductingMaterials,
    title = {{Semiconducting polymers containing tellurium: Perspectives toward obtaining high-performance materials}},
    year = {2015},
    booktitle = {Macromolecules},
    author = {Carrera, Elisa I. and Seferos, Dwight S.},
    number = {2},
    month = {1},
    pages = {297--308},
    volume = {48},
    publisher = {American Chemical Society},
    doi = {10.1021/ma502307b},
    issn = {15205835}
}

@article{Liang2019SeparatingSeparation,
    title = {{Separating Crystallization Process of P3HT and O‐IDTBR to Construct Highly Crystalline Interpenetrating Network with Optimized Vertical Phase Separation}},
    year = {2019},
    journal = {Advanced Functional Materials},
    author = {Liang, Qiuju and Jiao, Xuechen and Yan, Ye and Xie, Zhiyuan and Lu, Guanghao and Liu, Jiangang and Han, Yanchun},
    number = {47},
    month = {11},
    pages = {1807591},
    volume = {29},
    publisher = {Wiley-VCH Verlag},
    url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/adfm.201807591},
    doi = {10.1002/adfm.201807591},
    issn = {1616-301X},
    keywords = {crystallinity, film-forming kinetics, morphology, nonfullerene solar cells, vertical phase separation}
}

@article{Lehmkuhler2015SequentialLaser,
    title = {{Sequential Single Shot X-ray Photon Correlation Spectroscopy at the SACLA Free Electron Laser}},
    year = {2015},
    journal = {Scientific Reports},
    author = {Lehmk{\"{u}}hler, Felix and Kwasniewski, Pawel and Roseker, Wojciech and Fischer, Birgit and Schroer, Martin A. and Tono, Kensuke and Katayama, Tetsuo and Sprung, Michael and Sikorski, Marcin and Song, Sanghoon and Glownia, James and Chollet, Matthieu and Nelson, Silke and Robert, Aymeric and Gutt, Christian and Yabashi, Makina and Ishikawa, Tetsuya and Gr{\"{u}}bel, Gerhard},
    pages = {1--9},
    volume = {5},
    publisher = {Nature Publishing Group},
    url = {http://dx.doi.org/10.1038/srep17193},
    doi = {10.1038/srep17193},
    issn = {20452322}
}

@article{Henry2017SimplifiedPolymers,
    title = {{Simplified Models for Accelerated Structural Prediction of Conjugated Semiconducting Polymers}},
    year = {2017},
    journal = {Journal of Physical Chemistry C},
    author = {Henry, Michael M. and Jones, Matthew L. and Oosterhout, Stefan D. and Braunecker, Wade A. and Kemper, Travis W. and Larsen, Ross E. and Kopidakis, Nikos and Toney, Michael F. and Olson, Dana C. and Jankowski, Eric},
    number = {47},
    pages = {26528--26538},
    volume = {121},
    doi = {10.1021/acs.jpcc.7b09701},
    issn = {19327455}
}

@article{Yuan2019Single-JunctionCore,
    title = {{Single-Junction Organic Solar Cell with over 15{\%} Efficiency Using Fused-Ring Acceptor with Electron-Deficient Core}},
    year = {2019},
    journal = {Joule},
    author = {Yuan, Jun and Zhang, Yunqiang and Zhou, Liuyang and Zhang, Guichuan and Yip, Hin Lap and Lau, Tsz Ki and Lu, Xinhui and Zhu, Can and Peng, Hongjian and Johnson, Paul A. and Leclerc, Mario and Cao, Yong and Ulanski, Jacek and Li, Yongfang and Zou, Yingping},
    number = {4},
    month = {4},
    pages = {1140--1151},
    volume = {3},
    publisher = {Cell Press},
    doi = {10.1016/j.joule.2019.01.004},
    issn = {25424351}
}

@article{Schubert1994SmallMicroemulsions,
    title = {{Small angle neutron scattering near Lifshitz lines: Transition from weakly structured mixtures to microemulsions}},
    year = {1994},
    journal = {The Journal of Chemical Physics},
    author = {Schubert, K. V. and Strey, R. and Kline, S. R. and Kaler, E. W.},
    number = {6},
    pages = {5343--5355},
    volume = {101},
    doi = {10.1063/1.467387},
    issn = {00219606},
    keywords = {EMULSIONS, MIXTURES, NEUTRON SPECTROSCOPY, PHASE TRANSFORMATIONS, SMALL ANGLE SCATTERING, SURFACE STATES, SURFACTANTS, WETTING}
}

@misc{SmallTopics,
    title = {{Small Angle Scattering - an overview | ScienceDirect Topics}},
    url = {https://www.sciencedirect.com/topics/chemistry/small-angle-scattering}
}

@article{Prevost2016Small-angle1,
    title = {{Small-angle scattering and morphologies of ultra-flexible microemulsions 1}},
    year = {2016},
    journal = {J. Appl. Cryst},
    author = {Prevost, Sylvain and Lopian, Tobias and Pleines, Maximilian and Diat, Olivier and Zemb, Thomas},
    pages = {2063--2072},
    volume = {49},
    url = {http://dx.doi.org/10.1107/S16005767160161502063},
    doi = {10.1107/S1600576716016150},
    keywords = {mesoscale solubilization, small-angle scattering (SAS), surfactant-free microemulsions, ultra-flexible microemulsions}
}

@article{Prevost2016Small-angleSAS2015.,
    title = {{Small-angle scattering and morphologies of ultra-flexible microemulsionsThis article will form part of a virtual special issue of the journal, presenting some highlights of the 16th International Conference on Small-Angle Scattering (SAS2015).}},
    year = {2016},
    journal = {Journal of Applied Crystallography, In-ternational Union of Crystallography},
    author = {Prevost, Sylvain and Lopian, Tobias and Pleines, Maximilian and Diat, Olivier and Zemb, Thomas and Small, Thomas Zemb},
    pages = {2063--2072},
    volume = {49},
    url = {http://dx.doi.org/10.1107/S16005767160161502063},
    doi = {10.1107/S1600576716016150{\"{i}}},
    keywords = {MESOSCALE SOLUBILIZATION, SMALL-ANGLE SCATTERING (SAS), SURFACTANT-FREE MICROEMULSIONS, TERNARY PHASE DIAGRAMS, ULTRA-FLEXIBLE MICROEMULSIONS}
}

@article{WelbornAb2020Small-angleMaterials,
    title = {{Small-angle X-ray scattering of nanoporous materials}},
    year = {2020},
    author = {Welborn Ab, Samuel S and Detsi, Eric},
    pages = {12},
    volume = {5},
    doi = {10.1039/c9nh00347a}
}

@article{WelbornAb2020Small-angleMaterialsb,
    title = {{Small-angle X-ray scattering of nanoporous materials}},
    year = {2020},
    author = {Welborn Ab, Samuel S and Detsi, Eric},
    pages = {12},
    volume = {5},
    doi = {10.1039/c9nh00347a}
}

@techreport{Bale1984Small-AngleProperties,
    title = {{Small-Angle X-Ray-Scattering Investigation of Submicroscopic Porosity with Fractal Properties}},
    year = {1984},
    author = {Bale, Harold D and Schmidt, Paul},
    number = {6},
    volume = {3}
}

@article{Guo2017Solvent-morphology-propertyCells,
    title = {{Solvent-morphology-property relationship of PTB7: PC71BM polymer solar cells}},
    year = {2017},
    journal = {ACS Applied Materials and Interfaces},
    author = {Guo, Shuai and Wang, Weijia and Herzig, Eva M. and Naumann, Anna and Tainter, Gregory and Perlich, Jan and M{\"{u}}ller-Buschbaum, Peter},
    number = {4},
    month = {2},
    pages = {3740--3748},
    volume = {9},
    publisher = {American Chemical Society},
    url = {www.acsami.org},
    doi = {10.1021/acsami.6b14926},
    issn = {19448252},
    pmid = {28075549},
    keywords = {Crystallinity, Morphology, Organic solar cells, PTB7, Solvent}
}

@article{Kim2014SpecialMicroelectronics,
    title = {{Special Issue : Polymers for Microelectronics Polymers for Microelectronics Special Issue : Polymers for Microelectronics}},
    year = {2014},
    journal = {Journal of Applied Polymer Science},
    author = {Kim, Bong Jun and Kim, Do Heung and Kang, Seung Youl and Ahn, Seong Deok and Im, Sung Gap},
    volume = {1},
    doi = {10.1002/app.41233}
}

@incollection{Allen2001SpinodalDecomposition,
    title = {{Spinodal Decomposition}},
    year = {2001},
    booktitle = {Encyclopedia of Materials: Science and Technology},
    author = {Allen, S.M.},
    pages = {8761--8764},
    publisher = {Elsevier},
    url = {https://linkinghub.elsevier.com/retrieve/pii/B0080431526015692},
    doi = {10.1016/B0-08-043152-6/01569-2}
}

@article{Steyn-Ross2019SpinodalPatterns,
    title = {{Spinodal decomposition in a mean-field model of the cortex: Emergence of hexagonally symmetric activation patterns}},
    year = {2019},
    journal = {PHYSICAL REVIEW E},
    author = {Steyn-Ross, Moira L and Steyn-Ross, D A and Voss, L J and Sleigh, J W},
    pages = {12318},
    volume = {99},
    doi = {10.1103/PhysRevE.99.012318},
    keywords = {doi:10.1103/PhysRevE.99.012318 url:https://doi.org/10.1103/PhysRevE.99.012318}
}

@article{Ding2016SprayApplications,
    title = {{Spray coated silver nanowires as transparent electrodes in OPVs for Building Integrated Photovoltaics applications}},
    year = {2016},
    journal = {Solar Energy Materials and Solar Cells},
    author = {Ding, Z. and Stoichkov, V. and Horie, M. and Brousseau, E. and Kettle, J.},
    month = {12},
    pages = {305--311},
    volume = {157},
    publisher = {Elsevier B.V.},
    doi = {10.1016/j.solmat.2016.05.053},
    issn = {09270248},
    keywords = {Building Integrated PVS, Intermediate layer, Organic solar cells, Silver nanowires}
}

@article{Jrgensen2008Stability/degradationCells,
    title = {{Stability/degradation of polymer solar cells}},
    year = {2008},
    journal = {Solar Energy Materials and Solar Cells},
    author = {J{\o}rgensen, Mikkel and Norrman, Kion and Krebs, Frederik C.},
    number = {7},
    pages = {686--714},
    volume = {92},
    doi = {10.1016/j.solmat.2008.01.005},
    issn = {09270248},
    keywords = {Degradation, Mechanisms, Organic solar cells, Polymer photovoltaic, Stability}
}

@article{Morkved2001StaticAmphiphilicity,
    title = {{Static and dynamic scattering from ternary polymer blends: Bicontinuous microemulsions, Lifshitz lines, and amphiphilicity}},
    year = {2001},
    journal = {Journal of Chemical Physics},
    author = {Morkved, Terry L. and Stepanek, Petr and Krishnan, Kasiraman and Bates, Frank S. and Lodge, Timothy P.},
    number = {16},
    pages = {7247--7259},
    volume = {114},
    url = {https://doi.org/10.1063/1.1357800},
    isbn = {10.1063/1.453006},
    doi = {10.1063/1.1357800},
    issn = {00219606}
}

@book{Gould2010StatisticalApplications,
    title = {{Statistical and thermal physics : with computer applications}},
    year = {2010},
    author = {Gould, Harvey and Tobochnik, Jan},
    pages = {511},
    publisher = {Princeton University Press},
    isbn = {9780691137445}
}

@article{Anitas2018StructuralAutomata,
    title = {{Structural Properties of Additive Nano/Microcellular Automata}},
    year = {2018},
    journal = {Annalen der Physik},
    author = {Anitas, Eugen Mircea and Slyamov, Azat},
    number = {6},
    month = {6},
    pages = {1800004},
    volume = {530},
    url = {http://doi.wiley.com/10.1002/andp.201800004},
    doi = {10.1002/andp.201800004},
    issn = {00033804}
}

@article{Cerar2020StructuralAlcohol,
    title = {{Structural, rheological and dynamic aspects of hydrogen-bonding molecular liquids: Aqueous solutions of hydrotropic tert-butyl alcohol}},
    year = {2020},
    journal = {Journal of Colloid and Interface Science},
    author = {Cerar, Jure and Jamnik, Andrej and Pethes, Ildikó and Temleitner, László and Pusztai, László and Tom{\v{s}}i{\v{c}}, Matija},
    month = {2},
    pages = {730--742},
    volume = {560},
    publisher = {Academic Press Inc.},
    doi = {10.1016/j.jcis.2019.10.094},
    issn = {10957103},
    keywords = {Alcohol, Aqueous binary system, Complemented-system method, Hydrotrope, Molecular dynamics simulation, SWAXS, Self-assembly, Self-diffusion coefficients, T-butanol, Viscosity}
}

@article{Pedersen2015StructureCells,
    title = {{Structure and crystallinity of water dispersible photoactive nanoparticles for organic solar cells}},
    year = {2015},
    journal = {Journal of Materials Chemistry A},
    author = {Pedersen, E. B.L. and Pedersen, M. C. and Simonsen, S. B. and Brandt, R. G. and B{\"{o}}ttiger, A. P.L. and Andersen, T. R. and Jiang, W. and Xie, Z. Y. and Krebs, F. C. and Arleth, L. and Andreasen, J. W.},
    number = {33},
    month = {7},
    pages = {17022--17031},
    volume = {3},
    publisher = {Royal Society of Chemistry},
    doi = {10.1039/c5ta04980f},
    issn = {20507496}
}

@article{Hayes2015StructureLiquids,
    title = {{Structure and Nanostructure in Ionic Liquids}},
    year = {2015},
    author = {Hayes, Robert and Warr, Gregory G and Atkin, Rob},
    url = {https://pubs.acs.org/sharingguidelines},
    doi = {10.1021/cr500411q}
}

@article{Bockmann2015StructureAnalysis,
    title = {{Structure of P3HT crystals, thin films, and solutions by UV/Vis spectral analysis}},
    year = {2015},
    journal = {Physical Chemistry Chemical Physics},
    author = {B{\"{o}}ckmann, Marcus and Schemme, Thomas and De Jong, Djurre H. and Denz, Cornelia and Heuer, Andreas and Doltsinis, Nikos L.},
    number = {43},
    month = {10},
    pages = {28616--28625},
    volume = {17},
    publisher = {Royal Society of Chemistry},
    doi = {10.1039/c5cp03665h},
    issn = {14639076}
}

@article{Irwin2016Structure-conductivityBlends,
    title = {{Structure-conductivity relationships in ordered and disordered salt-doped diblock copolymer/homopolymer blends}},
    year = {2016},
    journal = {Macromolecules},
    author = {Irwin, Matthew T. and Hickey, Robert J. and Xie, Shuyi and So, Soonyong and Bates, Frank S. and Lodge, Timothy P.},
    number = {18},
    month = {9},
    pages = {6928--6939},
    volume = {49},
    publisher = {American Chemical Society},
    doi = {10.1021/acs.macromol.6b01553},
    issn = {15205835}
}

@article{Gazzano2015Structure-morphologySAXS-WAXD,
    title = {{Structure-morphology correlation in electrospun fibers of semicrystalline polymers by simultaneous synchrotron SAXS-WAXD}},
    year = {2015},
    journal = {Polymer},
    author = {Gazzano, M. and Gualandi, C. and Zucchelli, A. and Sui, T. and Korsunsky, A. M. and Reinhard, C. and Focarete, M. L.},
    pages = {154--163},
    volume = {63},
    publisher = {Elsevier Ltd},
    url = {http://dx.doi.org/10.1016/j.polymer.2015.03.002},
    doi = {10.1016/j.polymer.2015.03.002},
    issn = {00323861},
    keywords = {Crystal phase, Electrospinning, Synchrotron SAXS-WAXD}
}

@article{Yuan2015StudyTechniques,
    title = {{Study on {$\pi$}−{$\pi$} Interaction in H-and J-Aggregates of Poly(3-hexylthiophene) Nanowires by Multiple Techniques}},
    year = {2015},
    author = {Yuan, Yuan and Shu, Jie and Liu, Ping and Zhang, Yinping and Duan, Yongxin and Zhang, Jianming},
    url = {https://pubs.acs.org/sharingguidelines},
    doi = {10.1021/acs.jpcb.5b02805}
}

@book{KomiteenforSundhedsoplysning2019SundeAr,
    title = {{Sunde b{\o}rn : til for{\ae}ldre med b{\o}rn i alderen 0-2 år}},
    year = {2019},
    author = {{Komiteen for Sundhedsoplysning} and {Danmark. Sundhedsstyrelsen} and {Heidi Maxmilling} and {Thomas Tolstrup} and {Dina Gellert}},
    isbn = {9788770140911}
}

@article{Ye2018SurpassingSolvent,
    title = {{Surpassing 10{\%} Efficiency Benchmark for Nonfullerene Organic Solar Cells by Scalable Coating in Air from Single Nonhalogenated Solvent}},
    year = {2018},
    journal = {Advanced Materials},
    author = {Ye, Long and Xiong, Yuan and Zhang, Qianqian and Li, Sunsun and Wang, Cheng and Jiang, Zhang and Hou, Jianhui and You, Wei and Ade, Harald},
    number = {8},
    pages = {1--9},
    volume = {30},
    doi = {10.1002/adma.201705485},
    issn = {15214095},
    keywords = {blade coating, film morphology, nonfullerene acceptors, nonhalogenated solvents, organic solar cells}
}

@article{Smith2013SynthesisChemistry,
    title = {{Synthesis and crystallinity of conjugated block copolymers prepared by click chemistry}},
    year = {2013},
    journal = {Macromolecules},
    author = {Smith, Kendall A. and Lin, Yen Hao and Dement, Dana B. and Strzalka, Joseph and Darling, Seth B. and Pickel, Deanna L. and Verduzco, Rafael},
    number = {7},
    pages = {2636--2645},
    volume = {46},
    doi = {10.1021/ma3026223},
    issn = {00249297}
}

@article{PortoneTailoringPolythiophene,
    title = {{tailoring optical properties and stimulated emission in nanostructured polythiophene}},
    author = {Portone, Alberto and Ganzer, Lucia and Branchi, Federico and Ramos, Rodrigo and Caldas, Marília J and Pisignano, Dario and Molinari, Elisa and Cerullo, Giulio and Persano, Luana and Prezzi, Deborah and Tersilla Virgili, &},
    url = {www.nature.com/scientificreports},
    doi = {10.1038/s41598-019-43719-0}
}

@techreport{Dectris2018TechnicalSystems,
    title = {{Technical Specifications EIGER R 4M Detector Systems}},
    year = {2018},
    author = {{Dectris}},
    pages = {27},
    url = {www.dectris.com}
}

@article{Lee2016Temperature-DependentFilm,
    title = {{Temperature-Dependent Evolution of Poly(3-Hexylthiophene) Type-II Phase in a Blended Thin Film}},
    year = {2016},
    journal = {Macromolecular Rapid Communications},
    author = {Lee, Si Woo and Keum, Hee Sung and Kim, Han Seong and Kim, Hyo Jung and Ahn, Kwangseok and Lee, Dong Ryeol and Kim, Je Han and Lee, Hyun Hwi},
    number = {3},
    month = {2},
    pages = {203--208},
    volume = {37},
    publisher = {John Wiley {\&} Sons, Ltd},
    url = {https://onlinelibrary.wiley.com/doi/full/10.1002/marc.201500527 https://onlinelibrary.wiley.com/doi/abs/10.1002/marc.201500527 https://onlinelibrary.wiley.com/doi/10.1002/marc.201500527},
    doi = {10.1002/MARC.201500527},
    issn = {1521-3927},
    pmid = {26605504},
    keywords = {II phase, P3HT, alignment, polymorph, solvent mixture, type}
}

@article{Haegel2017Terawatt-scaleChallenges,
    title = {{Terawatt-scale photovoltaics: Trajectories and challenges}},
    year = {2017},
    journal = {Science},
    author = {Haegel, Nancy M. and Margolis, Robert and Buonassisi, Tonio and Feldman, David and Froitzheim, Armin and Garabedian, Raffi and Green, Martin and Glunz, Stefan and Henning, Hans-Martin and Holder, Burkhard and Kaizuka, Izumi and Kroposki, Benjamin and Matsubara, Koji and Niki, Shigeru and Sakurai, Keiichiro and Schindler, Roland A. and Tumas, William and Weber, Eicke R. and Wilson, Gregory and Woodhouse, Michael and Kurtz, Sarah},
    number = {6334},
    month = {4},
    pages = {141--143},
    volume = {356},
    publisher = {American Association for the Advancement of Science},
    url = {http://www.sciencemag.org/lookup/doi/10.1126/science.aal1288},
    doi = {10.1126/science.aal1288},
    issn = {0036-8075}
}

@article{HeydariGharahcheshmeh2020TexturePolymers,
    title = {{Texture and nanostructural engineering of conjugated conducting and semiconducting polymers}},
    year = {2020},
    journal = {Materials Today Advances},
    author = {Heydari Gharahcheshmeh, M. and Gleason, K. K.},
    pages = {100086},
    volume = {8},
    publisher = {Elsevier Ltd},
    url = {https://doi.org/10.1016/j.mtadv.2020.100086 https://reader.elsevier.com/reader/sd/pii/S2590049820300333?token=75B6E7D5F9326B6AA8D9DA0794D754A023CDC033B1A9EECAF78F096CF3E215C5177131B675C0890DCE87247F7930AC50},
    doi = {10.1016/j.mtadv.2020.100086},
    issn = {25900498},
    keywords = {Electrical conductivity, Optoelectronic, P3HT, PEDOT, {$\pi$}–{$\pi$} stacking distance}
}

@misc{TheDiagram,
    title = {{The AFM and TEM images of films prepared without A,B) TCB, films... | Download Scientific Diagram}},
    url = {https://www.researchgate.net/figure/The-AFM-and-TEM-images-of-films-prepared-without-A-B-TCB-films-prepared-with-C-D-TCB_fig2_330518334}
}

@article{Hollamby2017The,
    title = {{The aggregation of an alkyl-C 60 derivative as a function of concentration, temperature and solvent type †}},
    year = {2017},
    author = {Hollamby, Martin J and Smith, Catherine F and Britton, Melanie M and Danks, Ashleigh E and Schnepp, Zoe and Grillo, Isabelle and Pauw, Brian R and Kishimura, Akihiro and Nakanishi, Takashi},
    doi = {10.1039/c7cp06348b}
}

@article{Wang2021ThePerformances,
    title = {{The coupling and competition of crystallization and phase separation, correlating thermodynamics and kinetics in OPV morphology and performances}},
    year = {2021},
    journal = {Nature Communications},
    author = {Wang, Zaiyu and Gao, Ke and Kan, Yuanyuan and Zhang, Ming and Qiu, Chaoqun and Zhu, Lei and Zhao, Zhe and Peng, Xiaobin and Feng, Wei and Qian, Zhiyuan and Gu, Xiaodan and Jen, Alex K.Y. and Tang, Ben Zhong and Cao, Yong and Zhang, Yongming and Liu, Feng},
    number = {1},
    month = {12},
    pages = {1--14},
    volume = {12},
    publisher = {Nature Research},
    url = {https://doi.org/10.1038/s41467-020-20515-3},
    doi = {10.1038/s41467-020-20515-3},
    issn = {20411723},
    keywords = {Organic molecules in materials science, Solar cells, Surfaces, interfaces and thin films}
}

@article{Lenz2010THEStructures,
    title = {{THE EUROPEAN PHYSICAL JOURNAL APPLIED PHYSICS Global scattering functions: a tool for grazing incidence small angle X-ray scattering (GISAXS) data analysis of low correlated lateral structures}},
    year = {2010},
    journal = {Eur. Phys. J. Appl. Phys},
    author = {Lenz, S and Bonini, M and Nett, S K and Lechmann, M C and Emmerling, S G J and Kappes, R S and Memesa, M and Timmann, A and Roth, S V and Gutmann, J S},
    pages = {10601},
    volume = {51},
    url = {https://doi.org/10.1051/epjap/2010064},
    doi = {10.1051/epjap/2010064}
}

@article{Gambhir2016TheAnalysis,
    title = {{The future costs of OPV – A bottom-up model of material and manufacturing costs with uncertainty analysis}},
    year = {2016},
    journal = {Solar Energy Materials and Solar Cells},
    author = {Gambhir, Ajay and Sandwell, Philip and Nelson, Jenny},
    month = {11},
    pages = {49--58},
    volume = {156},
    publisher = {Elsevier B.V.},
    doi = {10.1016/j.solmat.2016.05.056},
    issn = {09270248},
    keywords = {Cost reduction, Economies of scale, Innovation, Manufacturing costs, Organic photovoltaics, Solar photovolataic costs, Uncertainty analysis}
}

@article{Mirsafaei2017TheElectrodes,
    title = {{The influence of electrical effects on device performance of organic solar cells with nano-structured electrodes}},
    year = {2017},
    journal = {Scientific Reports},
    author = {Mirsafaei, Mina and Fallahpour, Amir Hossein and Lugli, Paolo and Rubahn, Horst Günter and Adam, Jost and Madsen, Morten},
    number = {1},
    month = {12},
    volume = {7},
    publisher = {Nature Publishing Group},
    doi = {10.1038/s41598-017-05591-8},
    issn = {20452322}
}

@article{Tumbleston2014TheCells,
    title = {{The influence of molecular orientation on organic bulk heterojunction solar cells}},
    year = {2014},
    journal = {Nature Photonics},
    author = {Tumbleston, John R and Collins, Brian A and Yang, Liqiang and Stuart, Andrew C and Gann, Eliot and Ma, Wei and You, Wei and Ade, Harald},
    number = {5},
    pages = {385--391},
    volume = {8},
    url = {www.nature.com/naturephotonics},
    doi = {10.1038/nphoton.2014.55},
    issn = {17494893}
}

@article{Beye2010TheElectrons,
    title = {{The liquid-liquid phase transition in silicon revealed by snapshots of valence electrons}},
    year = {2010},
    journal = {Proceedings of the National Academy of Sciences of the United States of America},
    author = {Beye, Martin and Sorgenfrei, Florian and Schlotter, William F. and Wurth, Wilfried and F{\"{o}}hlisch, Alexander},
    number = {39},
    pages = {16772--16776},
    volume = {107},
    doi = {10.1073/pnas.1006499107},
    issn = {00278424},
    keywords = {Liquid-liquid hypothesis, Silicon phases, Ultrafast spectroscopy, X-ray spectroscopy}
}

@misc{Curfman2009The2009,
    title = {{The medical device safety act of 2009}},
    year = {2009},
    booktitle = {New England Journal of Medicine},
    author = {Curfman, Gregory D. and Morrissey, Stephen and Drazen, Jeffrey M.},
    number = {15},
    pages = {1550--1551},
    volume = {360},
    doi = {10.1056/NEJMe0902377},
    issn = {15334406}
}

@article{GuThePolymers,
    title = {{The meniscus-guided deposition of semiconducting polymers}},
    author = {Gu, Xiaodan and Shaw, Leo and Gu, Kevin and Toney, Michael F and Bao, Zhenan},
    url = {www.nature.com/naturecommunications},
    doi = {10.1038/s41467-018-02833-9}
}

@article{Jiang2014TheoryGISAXS,
    title = {{Theory of GISAXS}},
    year = {2014},
    journal = {American Crystallographic Association Meeting},
    author = {Jiang, Zhang}
}

@article{Hegedus2004Thin-filmAnalysis,
    title = {{Thin-film solar cells: device measurements and analysis}},
    year = {2004},
    journal = {Progress in Photovoltaics: Research and Applications},
    author = {Hegedus, Steven S. and Shafarman, William N.},
    number = {23},
    month = {3},
    pages = {155--176},
    volume = {12},
    isbn = {1099-159X},
    doi = {10.1002/pip.518},
    issn = {1062-7995}
}

@article{ThisScattering,
    title = {{This is a repository copy of Exploring the bulk-phase structure of ionic liquid mixtures using small-angle neutron scattering}},
    url = {http://eprints.whiterose.ac.uk/118285/},
    doi = {10.1039/C7FD00167C},
    issn = {1364-5498}
}

@article{2019ThreeLimit,
    title = {{Three dimensional polarimetric neutron tomography-beyond the phase-wrapping limit}},
    year = {2019},
    url = {https://doi.org/10.1088/1361-6463/ab0aba},
    isbn = {192.38.90.123},
    doi = {10.1088/1361-6463/ab0aba}
}

@article{Sun2012Three-dimensionalReflection,
    title = {{Three-dimensional coherent X-ray surface scattering imaging near total external reflection}},
    year = {2012},
    journal = {Nature Photonics},
    author = {Sun, Tao and Jiang, Zhang and Strzalka, Joseph and Ocola, Leonidas and Wang, Jin},
    number = {9},
    pages = {586--590},
    volume = {6},
    publisher = {Nature Publishing Group},
    url = {http://dx.doi.org/10.1038/nphoton.2012.178},
    doi = {10.1038/nphoton.2012.178},
    issn = {17494885}
}

@article{Godard2011Three-dimensionalCrystals,
    title = {{Three-dimensional high-resolution quantitative microscopy of extended crystals}},
    year = {2011},
    journal = {Nature Communications},
    author = {Godard, P. and Carbone, G. and Allain, M. and Mastropietro, F. and Chen, G. and Capello, L. and Diaz, A. and Metzger, T. H. and Stangl, J. and Chamard, V.},
    number = {1},
    pages = {566--568},
    volume = {2},
    publisher = {Nature Publishing Group},
    url = {http://dx.doi.org/10.1038/ncomms1569},
    doi = {10.1038/ncomms1569},
    issn = {20411723}
}

@article{Holler2019Three-dimensionalZoom,
    title = {{Three-dimensional imaging of integrated circuits with macro- to nanoscale zoom}},
    year = {2019},
    journal = {Nature Electronics},
    author = {Holler, Mirko and Odstrcil, Michal and Guizar-Sicairos, Manuel and Lebugle, Maxime and M{\"{u}}ller, Elisabeth and Finizio, Simone and Tinti, Gemma and David, Christian and Zusman, Joshua and Unglaub, Walter and Bunk, Oliver and Raabe, Jörg and Levi, A. F. J. and Aeppli, Gabriel},
    month = {10},
    publisher = {Springer Science and Business Media LLC},
    doi = {10.1038/s41928-019-0309-z}
}

@article{Donnelly2017Three-dimensionalNanotomography,
    title = {{Three-dimensional magnetization structures revealed with X-ray vector nanotomography}},
    year = {2017},
    journal = {Nature},
    author = {Donnelly, Claire and Guizar-Sicairos, Manuel and Scagnoli, Valerio and Gliga, Sebastian and Holler, Mirko and Raabe, Jörg and Heyderman, Laura J.},
    number = {7663},
    month = {7},
    pages = {328--331},
    volume = {547},
    publisher = {Nature Publishing Group},
    doi = {10.1038/nature23006},
    issn = {14764687},
    keywords = {Characterization and analytical techniques, Ferromagnetism, Imaging techniques, Magnetic properties and materials}
}

@article{Rogers2012Time-ResolvedBM,
    title = {{Time-Resolved Structural Evolution of Additive-Processed Bulk Heterojunction Solar Cells Scheme 1. Molecular Structures of (a) PCPDTBT and (b) PC 70 BM}},
    year = {2012},
    journal = {J. Am. Chem.Soc},
    author = {Rogers, James T and Schmidt, Kristin and Toney, Michael F and Bazan, Guillermo C and Kramer, Edward J},
    pages = {26},
    volume = {134},
    publisher = {UTC},
    url = {https://pubs.acs.org/sharingguidelines},
    doi = {10.1021/ja2104747}
}

@article{Pearson2015ToAl,
    title = {{To cite this article: Xing Fan et al}},
    year = {2015},
    journal = {Chinese Phys. B},
    author = {Pearson, Andrew J and Wang, Tao and Lidzey -, David G},
    pages = {78401},
    volume = {24},
    url = {http://cpb.iphy.ac.cn},
    doi = {10.1088/1674-1056/24/7/078401}
}

@article{Yang2021TowardAir,
    title = {{Toward all aerosol printing of high-efficiency organic solar cells using environmentally friendly solvents in ambient air}},
    year = {2021},
    journal = {Journal of Materials Chemistry A},
    author = {Yang, Ping and Zhai, Tianqi and Yu, Boyang and Du, Gengxin and Mi, Baoxiu and Zhao, Xinyan and Deng, Weiwei},
    number = {32},
    month = {8},
    pages = {17198--17210},
    volume = {9},
    publisher = {The Royal Society of Chemistry},
    url = {https://pubs.rsc.org/en/content/articlehtml/2021/ta/d1ta02890a https://pubs.rsc.org/en/content/articlelanding/2021/ta/d1ta02890a},
    doi = {10.1039/D1TA02890A},
    issn = {2050-7496}
}

@article{Sepe2016TowardStudy,
    title = {{Toward an equilibrium structure in lamellar diblock copolymer thin films using solvent vapor annealing – An in-situ time-resolved GISAXS study}},
    year = {2016},
    journal = {European Polymer Journal},
    author = {Sepe, Alessandro and Zhang, Jianqi and Perlich, Jan and Smilgies, Detlef M. and Posselt, Dorthe and Papadakis, Christine M.},
    pages = {607--620},
    volume = {81},
    publisher = {Elsevier Ltd},
    url = {http://dx.doi.org/10.1016/j.eurpolymj.2015.12.013},
    doi = {10.1016/j.eurpolymj.2015.12.013},
    issn = {00143057},
    keywords = {Block copolymers, Grazing-incidence small-angle X-ray scattering, Nanostructured thin films, Solvent vapor annealing}
}

@article{Blakesley2014TowardsSemiconductors,
    title = {{Towards reliable charge-mobility benchmark measurements for organic semiconductors}},
    year = {2014},
    journal = {Organic Electronics},
    author = {Blakesley, James C. and Castro, Fernando A. and Kylberg, William and Dibb, George F.A. and Arantes, Caroline and Valaski, Rogério and Cremona, Marco and Kim, Jong Soo and Kim, Ji-Seon},
    number = {6},
    month = {6},
    pages = {1263--1272},
    volume = {15},
    publisher = {Elsevier},
    url = {https://linkinghub.elsevier.com/retrieve/pii/S1566119914000469},
    doi = {10.1016/j.orgel.2014.02.008},
    issn = {15661199},
    keywords = {Charge-carrier mobility, Injection-limited current, Mobility, Mobility benchmark, Space-charge limited current}
}

@article{Luke2019TwistBlends,
    title = {{Twist and Degrade—Impact of Molecular Structure on the Photostability of Nonfullerene Acceptors and Their Photovoltaic Blends}},
    year = {2019},
    journal = {Advanced Energy Materials},
    author = {Luke, Joel and Speller, Emily M. and Wadsworth, Andrew and Wyatt, Mark F. and Dimitrov, Stoichko and Lee, Harrison K. H. and Li, Zhe and Tsoi, Wing C. and McCulloch, Iain and Bagnis, Diego and Durrant, James R. and Kim, Ji‐Seon},
    number = {15},
    month = {4},
    pages = {1803755},
    volume = {9},
    publisher = {Wiley-VCH Verlag},
    url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/aenm.201803755},
    doi = {10.1002/aenm.201803755},
    issn = {1614-6832},
    keywords = {conformational change, nonfullerene acceptor molecular structures, nonfullerene acceptors, organic solar cells, photostability}
}

@article{Pfau2012UltrafastWalls,
    title = {{Ultrafast optical demagnetization manipulates nanoscale spin structure in domain walls}},
    year = {2012},
    journal = {Nature Communications},
    author = {Pfau, B. and Schaffert, S. and M{\"{u}}ller, L. and Gutt, C. and Al-Shemmary, A. and B{\"{u}}ttner, F. and Delaunay, R. and D{\"{u}}sterer, S. and Flewett, S. and Fr{\"{o}}mter, R. and Geilhufe, J. and Guehrs, E. and G{\"{u}}nther, C. M. Cm and Hawaldar, R. and Hille, M. and Jaouen, N. and Kobs, A. and Li, K. and Mohanty, J. and Redlin, H. and Schlotter, W. F. WF and Stickler, D. and Treusch, R. and Vodungbo, B. and Kl{\"{a}}ui, M. and Oepen, HP P. and L{\"{u}}ning, J. and Gr{\"{u}}bel, G. and Eisebitt, S.},
    number = {1},
    month = {10},
    pages = {1--6},
    volume = {3},
    publisher = {Nature Publishing Group},
    url = {www.nature.com/naturecommunications},
    doi = {10.1038/ncomms2108},
    issn = {20411723},
    keywords = {Optical physics, Spintronics}
}

@article{Kajiya2018UltrapureFlow,
    title = {{Ultrapure Films of Polythiophene Derivatives are Born on a Substrate by Liquid Flow}},
    year = {2018},
    journal = {Cite This: ACS Appl. Energy Mater},
    author = {Kajiya, Daisuke and Saitow, Ken-Ichi},
    pages = {6881--6889},
    volume = {1},
    url = {www.acsaem.org},
    doi = {10.1021/acsaem.8b01260},
    keywords = {aggregate, coffee ring, contact angle, soft electronics, {$\pi$}-conjugated polymer}
}

@article{Zhang2017UnderstandingDevices,
    title = {{Understanding and controlling morphology evolution via DIO plasticization in PffBT4T-2OD/PC 71 BM devices}},
    year = {2017},
    journal = {Scientific Reports},
    author = {Zhang, Yiwei and Parnell, Andrew J. and Pontecchiani, Fabio and Cooper, Joshaniel F.K. K and Thompson, Richard L. and Jones, Richard A.L. L and King, Stephen M. and Lidzey, David G. and Bernardo, Gabriel},
    number = {July 2016},
    month = {3},
    pages = {1--12},
    volume = {7},
    publisher = {Nature Publishing Group},
    url = {www.nature.com/scientificreports http://dx.doi.org/10.1038/srep44269},
    doi = {10.1038/srep44269},
    issn = {20452322}
}

@article{Mai2016UnderstandingCells,
    title = {{Understanding Morphology Compatibility for High-Performance Ternary Organic Solar Cells}},
    year = {2016},
    journal = {Chemistry of Materials},
    author = {Mai, Jiangquan and Lau, Tsz Ki and Li, Jun and Peng, Shih Hao and Hsu, Chain Shu and Jeng, U. Ser and Zeng, Jianrong and Zhao, Ni and Xiao, Xudong and Lu, Xinhui},
    number = {17},
    pages = {6186--6195},
    volume = {28},
    doi = {10.1021/acs.chemmater.6b02264},
    issn = {15205002}
}

@article{Singh2018UnravelingCells,
    title = {{Unraveling the efficiency-limiting morphological issues of the perylene diimide-based non-fullerene organic solar cells}},
    year = {2018},
    journal = {Scientific Reports},
    author = {Singh, Ranbir and Suranagi, Sanjaykumar R. and Lee, Jaewon and Lee, Hansol and Kim, Min and Cho, Kilwon},
    number = {1},
    month = {12},
    pages = {1--9},
    volume = {8},
    publisher = {Springer US},
    url = {http://dx.doi.org/10.1038/s41598-018-21162-x},
    doi = {10.1038/s41598-018-21162-x},
    issn = {20452322}
}

@article{Holmes2019UnravellingFormulations,
    title = {{Unravelling donor–acceptor film morphology formation for environmentally-friendly OPV ink formulations}},
    year = {2019},
    journal = {Green Chemistry},
    author = {Holmes, Natalie P. and Munday, Holly and Barr, Matthew G. and Thomsen, Lars and Marcus, Matthew A. and Kilcoyne, A. L.David David and Fahy, Adam and Van Stam, Jan and Dastoor, Paul C. and Moons, Ellen},
    number = {18},
    pages = {5090--5103},
    volume = {21},
    publisher = {Royal Society of Chemistry},
    url = {http://xlink.rsc.org/?DOI=C9GC02288K},
    doi = {10.1039/C9GC02288K},
    issn = {1463-9262}
}

@article{Zhang2018UnveilingCells,
    title = {{Unveiling the important role of non-fullerene acceptors crystallinity on optimizing nanomorphology and charge transfer in ternary organic solar cells}},
    year = {2018},
    journal = {Organic Electronics: physics, materials, applications},
    author = {Zhang, Kang Ning and Bi, Peng Qing and Wen, Zhen Chuan and Niu, Meng Si and Chen, Zhi Hao and Wang, Tong and Feng, Lin and Yang, Jun Liang and Hao, Xiao Tao},
    number = {June},
    month = {11},
    pages = {643--652},
    volume = {62},
    publisher = {Elsevier},
    url = {https://doi.org/10.1016/j.orgel.2018.07.001},
    doi = {10.1016/j.orgel.2018.07.001},
    issn = {15661199},
    keywords = {Charge transfer, Non-fullerene acceptors, Organic solar cells}
}

@article{Liu2018UnwarpingData,
    title = {{Unwarping GISAXS data}},
    year = {2018},
    journal = {IUCrJ},
    author = {Liu, Jiliang and Yager, Kevin G.},
    pages = {737--752},
    volume = {5},
    publisher = {International Union of Crystallography},
    doi = {10.1107/S2052252518012058},
    issn = {20522525},
    keywords = {GISAXS, GTSAXS, X-ray scattering, distorted-wave Born approximation, image healing, reconstruction}
}

@article{Carle2014UpscalingLifetime,
    title = {{Upscaling from single cells to modules-fabrication of vacuum- and ITO-free polymer solar cells on flexible substrates with long lifetime}},
    year = {2014},
    journal = {Journal of Materials Chemistry C},
    author = {Carl{\'{e}}, Jon E. and Helgesen, Martin and Madsen, Morten V. and Bundgaard, Eva and Krebs, Frederik C.},
    number = {7},
    pages = {1290--1297},
    volume = {2},
    doi = {10.1039/c3tc31859a},
    issn = {20507534}
}

@article{Maplesoft2015VejledningPakken,
    title = {{Vejledning til Gym pakken}},
    year = {2015},
    author = {Maplesoft, Copyright}
}

@article{Pfannmoller2011VisualizingMicroscopy,
    title = {{Visualizing a homogeneous blend in bulk heterojunction polymer solar cells by analytical electron microscopy}},
    year = {2011},
    journal = {Nano Letters},
    author = {Pfannm{\"{o}}ller, Martin and Fl{\"{u}}gge, Harald and Benner, Gerd and Wacker, Irene and Sommer, Christoph and Hanselmann, Michael and Schmale, Stephan and Schmidt, Hans and Hamprecht, Fred A. and Rabe, Torsten and Kowalsky, Wolfgang and Schr{\"{o}}der, Rasmus R.},
    number = {8},
    month = {8},
    pages = {3099--3107},
    volume = {11},
    publisher = {American Chemical Society},
    url = {https://pubs.acs.org/sharingguidelines},
    doi = {10.1021/nl201078t},
    issn = {15306984},
    keywords = {Organic photovoltaics, bulk heterojunction, low-energy-loss electron spectroscopic imaging, multivariate statistical analysis, transmission electron microscopy}
}

@article{Jakowetz2017VisualizingBlends,
    title = {{Visualizing excitations at buried heterojunctions in organic semiconductor blends}},
    year = {2017},
    journal = {Nature Materials},
    author = {Jakowetz, Andreas C. and B{\"{o}}hm, Marcus L. and Sadhanala, Aditya and Huettner, Sven and Rao, Akshay and Friend, Richard H.},
    number = {5},
    pages = {551--557},
    volume = {16},
    doi = {10.1038/nmat4865},
    issn = {14764660}
}

@article{Kontges2020VisualizingBlends,
    title = {{Visualizing morphological principles for efficient photocurrent generation in organic non-fullerene acceptor blends}},
    year = {2020},
    journal = {Energy {\&} Environmental Science},
    author = {K{\"{o}}ntges, Wolfgang and Perkhun, Pavlo and Kammerer, Jochen and Alkarsifi, Riva and W{\"{u}}rfel, Uli and Margeat, Olivier and Videlot-Ackermann, Christine and Simon, Jean-Jacques and Schr{\"{o}}der, Rasmus R. and Ackermann, Jörg and Pfannm{\"{o}}ller, Martin},
    pages = {1259--1268},
    doi = {10.1039/c9ee03535d},
    issn = {1754-5692}
}

@article{Cui2019Wide-gapApplications,
    title = {{Wide-gap non-fullerene acceptor enabling high-performance organic photovoltaic cells for indoor applications}},
    year = {2019},
    journal = {Nature Energy},
    author = {Cui, Yong and Wang, Yuming and Bergqvist, Jonas and Yao, Huifeng and Xu, Ye and Gao, Bowei and Yang, Chenyi and Zhang, Shaoqing and Ingan{\"{a}}s, Olle and Gao, Feng and Hou, Jianhui},
    number = {9},
    month = {9},
    pages = {768--775},
    volume = {4},
    publisher = {Nature Publishing Group},
    url = {https://doi.org/10.1038/s41560-019-0448-5},
    doi = {10.1038/s41560-019-0448-5},
    issn = {20587546},
    keywords = {Energy, Energy harvesting, Renewable energy, Solar cells}
}

@article{Pfeiffer2018X-rayPtychography,
    title = {{X-ray ptychography}},
    year = {2018},
    journal = {Nature Photonics},
    author = {Pfeiffer, Franz},
    number = {1},
    month = {1},
    pages = {9--17},
    volume = {12},
    url = {http://www.nature.com/articles/s41566-017-0072-5},
    doi = {10.1038/s41566-017-0072-5},
    issn = {1749-4885}
}

@article{Pandolfi2018Xi-cam:Analysis,
    title = {{Xi-cam: a versatile interface for data visualization and analysis}},
    year = {2018},
    journal = {Journal of Synchrotron Radiation},
    author = {Pandolfi, Ronald J. and Allan, Daniel B. and Arenholz, Elke and Barroso-Luque, Luis and Campbell, Stuart I. and Caswell, Thomas A. and Blair, Austin and De Carlo, Francesco and Fackler, Sean and Fournier, Amanda P. and Freychet, Guillaume and Fukuto, Masafumi and G{\"{u}}rsoy, Dogˇa and Jiang, Zhang and Krishnan, Harinarayan and Kumar, Dinesh and Kline, R. Joseph and Li, Ruipeng and Liman, Christopher and Marchesini, Stefano and Mehta, Apurva and N'Diaye, Alpha T. and Parkinson, Dilworth Y. and Parks, Holden and Pellouchoud, Lenson A. and Perciano, Talita and Ren, Fang and Sahoo, Shreya and Strzalka, Joseph and Sunday, Daniel and Tassone, Christopher J. and Ushizima, Daniela and Venkatakrishnan, Singanallur and Yager, Kevin G. and Zwart, Peter and Sethian, James A. and Hexemer, Alexander},
    number = {4},
    month = {7},
    pages = {1261--1270},
    volume = {25},
    publisher = {Wiley-Blackwell},
    doi = {10.1107/S1600577518005787},
    issn = {16005775},
    keywords = {GISAXS, GIWAXS, NEXAFS, SAXS, WAXS, XAS, scattering, software, spectroscopy, tomography}
}

@misc{YuangboaLin.pdf,
    title = {{Yuangboa Lin.pdf}}
}

@article{Ye2016___.1--m-MATERIALS,
    title = {{{\_}{\_}{\_}.1--m-• MATERIALS}},
    year = {2016},
    author = {Ye, Long and Xiong, Yuan and Yao, Huifeng and Gadisa, Abay and Zhang, Hao and Li, Sunsun and Ghasemi, Masoud and Balar, Nrup and Hunt, Adrian and Connor, Brendan T O and Hou, Jianhui and Ade, Harald},
    pages = {7451--7458}
}

@article{Bruce2013NoTitle,
    title = {{済無No Title No Title}},
    year = {2013},
    journal = {Journal of Chemical Information and Modeling},
    author = {Bruce, 2011},
    number = {9},
    pages = {1689--1699},
    volume = {53},
    isbn = {9788578110796},
    doi = {10.1017/CBO9781107415324.004},
    issn = {1098-6596},
    pmid = {25246403},
    arxivId = {arXiv:1011.1669v3},
    keywords = {icle}
}
